A scalable exponential-DG approach for nonlinear conservation laws: with application to Burger and Euler equations

We propose an Exponential DG approach for numerically solving partial differential equations (PDEs). The idea is to decompose the governing PDE operators into linear (fast dynamics extracted by linearization) and nonlinear (the remaining after removing the former) parts, on which we apply the discontinuous Galerkin (DG) spatial discretization. The resulting semi-discrete system is then integrated using exponential time-integrators: exact for the former and approximate for the latter. By construction, our approach i) is stable with a large Courant number (Cr > 1); ii) supports high-order solutions both in time and space; iii) is computationally favorable compared to IMEX DG methods with no preconditioner; iv) requires comparable computational time compared to explicit RKDG methods, while having time stepsizes orders magnitude larger than maximal stable time stepsizes for explicit RKDG methods; v) is scalable in a modern massively parallel computing architecture by exploiting Krylov-subspace matrix-free exponential time integrators and compact communication stencil of DG methods. Various numerical results for both Burgers and Euler equations are presented to showcase these expected properties. For Burgers equation, we present detailed stability and convergence analyses for the exponential Euler DG scheme.

==> ExponentialDG_long.tex <==
\section{Exponential DG framework}
\seclab{ExponentialDG}

In this section, we present the key idea behind Exponential DG framework. We first split a given PDE into a linear and a nonlinear parts, to which DG discretization and exponential time integrators are applied. We begin with notations and conventions used in the paper. 

\subsection{Finite element definitions and notations}
Let $\Omega$ % be a line, a plane or a volume. 
be an open and bounded subset of $\R^d$, where $d = \LRc{1,2,3}$ is
the spatial dimention.
%% a spherical manifold is embedded in $R^3$. 
% \tanbui{$d =\LRc{2,3}$}{Do we actually have d = 3 in this paper?},
%Let $\pOmega$ be the physical boundary of the plane.
We denote by
$\Omega_h := \cup_{i=1}^\Nel \K_i$ the mesh containing a finite
collection of non-overlapping elements, $\K_i$, that partition
$\Omega$.  Here, $h$ is defined as $h := \max_{j\in
  \LRc{1,\hdots,\Nel}}diam\LRp{\Kj}$. Let $\pOmega_h := \LRc{\pK:\K
  \in \Omega_h}$ be the collection of the faces of all elements. 
Let us define $\Gh$
%$\Gh:= \LRc{\e: \e \in \Gho \cup \Ghb }$ 
as the skeleton
of the mesh which consists of the set of all uniquely defined faces.
%\tanbui{do we actually need $\Gho$ and $\Ghb$ later? if not there is no need to introduce them here.}
%where $\Ghb$ is the set of all boundary faces on $\pOmega$, and
%$\Gho:=\Gh \setminus \Ghb$ is the set of all interior interfaces. 
For
two neighboring elements $\Kp$ and $\Km$ that share an interior
interface $\e = \Kp \cap \Km$, we denote by $q^\pm$ the trace of their
solutions on $\e$. 
We define $\nm$ as the unit outward normal vector on
the boundary $\pK^-$ of element $\Km$, and $\np = -\nm$ the unit outward
normal of a neighboring element $\Kp$.  On the interior interfaces $\e
\in \Gho$, we define the mean/average operator $\average{\bf v}$, where $\bf v$ is
either a scalar or a vector quantify, as
$\average{{\bf v}}:=\LRp{{\bf v}^- + {\bf v}^+}/2$, 
%\begin{align*}
%\average{{\bf b}}:=\LRp{{\bf b}^- + {\bf b}^+}/2,
% \average{{\bf v}}:=\LRp{{\bf v}^- + {\bf v}^+}/2,
%% ,& \quad \jump{c\n} :=c^-\n^- + c^+\n^+,\\
%% \average{{\bf v}}:=\LRp{ {\bf v}^- + {\bf v}^+ }/2,& \quad \jump{{\bf v}\cdot\n} :={\bf v}^-\cdot \n^- + {\bf v}^+\cdot\n^+.
%\end{align*}
and the jump operator $\jump{\bf v} := 2\average{\bf v \cdot \nb}$.
 On the boundary faces $\e \in \Ghb$, we define the mean and jump operators as 
$\average{{\bf v}}:={\bf v}, \quad \jump{{\bf v}} :={\bf v}\cdot\nb$.
%\begin{align*}
%\average{c}:= c,& \quad \jump{c\n} :=c\n,\\
%\average{{\bf v}}:={\bf v}, \quad \jump{{\bf v}} :={\bf v}.
%\end{align*}

Let $\Poly^{k}\LRp{D}$ denote the space of polynomials of degree at
most $k$ on a domain $D$. Next, we introduce discontinuous
piecewise polynomial spaces for scalars and vectors as
\begin{align*}
\Vh\LRp{\Omega_h} &:= \LRc{v \in L^2\LRp{\Omega_h}:
  \eval{v}_{\K} \in \Poly^k\LRp{\K}, \forall \K \in \Omega_h}, \\
\Lamh\LRp{\Gh} &:= \LRc{\lambda \in \Lte:
  \eval{\lambda}_{\e} \in \Poly^k\LRp{\e}, \forall \e \in \Gh},\\
\Vbh\LRp{\Omega_h} &:= \LRc{{\bf v} \in \LRs{L^2\LRp{\Omega_h}}^m:
  \eval{{\bf v}}_{\K} \in \LRs{\Poly^k\LRp{\K}}^m, \forall \K \in \Omega_h},\\
\Lambh\LRp{\Gh} &:= \LRc{\lambdab \in \LRs{\Lte}^m:
  \eval{\lambdab}_{\e} \in \LRs{\Poly^k\LRp{\e}}^m, \forall \e \in \Gh}.
\end{align*}
and similar spaces $\VhK$, $\Lamhe$, $\VbhK$, and $\Lambhe$ by
replacing $\Omega_h$ with $\K$ and $\Gh$ with $\e$. Here, $m$ is the
number of components of the vector under consideration.

We define $\LRp{\cdot,\cdot}_\K$ as the $L^2$-inner product on an
element $\K \in \R^d$, and $\LRa{\cdot,\cdot}_{\pK}$ as the
$L^2$-inner product on the element boundary $\pK \in
\R^{d-1}$.  We also define the broken inner products as
$\LRp{\cdot,\cdot}_\Omega := \LRp{\cdot,\cdot}_{\Omega_h} :=
\sum_{\K\in \Omega_h}\LRp{\cdot,\cdot}_\K$ and
$\LRa{\cdot,\cdot}_{\pOmega} := \LRa{\cdot,\cdot}_{\pOmega_h} :=
\sum_{\pK\in \pOmega_h}\LRa{\cdot,\cdot}_\pK$, and on the mesh
skeleton as $\LRa{\cdot,\cdot}_\Gh := \sum_{\e\in
  \Gh}\LRa{\cdot,\cdot}_\e$.
%We also define the weighted norms as
%$\norm{\cdot}_{\Omegah,\gamma}:= \LRp{ \sum_{K\in \Omegah} \norm{\cdot}_{K,\gamma}^2 }^\half$ and
%$\norm{\cdot}_{\pOmegah,\gamma}:= \LRp{ \sum_{K\in \Omegah} \norm{\cdot}_{\pK,\gamma}^2 }^\half$,  
%where 
%$\norm{\cdot}_{\K,\gamma}=\LRp{|\gamma|\cdot,\cdot}_{\K}^\half$ and 
%$\norm{\cdot}_{\pK,\gamma} = \LRa{|\gamma|\cdot,\cdot}_{\pK}^\half$. % = \LRp{\int_{\pK} |\tau| (\cdot)^2 dx}^\half$.
%We denote $\norm{\cdot}_\K=\norm{\cdot}_{\K,1}$ and $\norm{\cdot}_\pK=\norm{\cdot}_{\pK,1}$. 

%We shall use boldface lowercase letters, e.g. $\mb{v}$  for vector-valued functions
% and employ boldface uppercase letters, e.g. $\mb{L}$ for tensors or matrices.




\subsection{Constructing a linear and a nonlinear operator in DG  }

We consider a partial differential equation (PDE), 
\begin{align}
  \eqnlab{pde}
   \dd{\qb}{t} + \Div \Fcal = \sb, \quad \text{ in } \Omega,
\end{align}
where $\qb$ is the conservative variable, $\Fcal=\Fcal(\qb)$ is 
the flux tensor, and $\sb$ is the source vector. 
We seek a stiff linear flux $\Fcal_L$ %in \eqnref{split-goveq-continuous} 
that, we assume, captures the rapidly changing dynamics in the system.
Inspired by the works in \cite{tokman2006efficient, giraldo2010high}, we use a flux Jacobian to define the linear flux, i.e., 
\begin{align}
  \eqnlab{linearflux}
  \Fcal_L := \dd{\Fcal}{\qb} \Bigg\vert_{\tilde{\qb}} \qb,
\end{align}
where $\tilde{\qb}$ is a reference state.
%By introducing the linear flux $\Fcal_L$ in \eqnref{linearflux}, 
By adding and subtracting the linear flux $\Fcal_L$ in \eqnref{pde},
 we split the divergence term into a linear (stiff) part $\Div{\Fcal_L}$ and a nonlinear (non-stiff)
part $\Div{\LRp{\Fcal - \Fcal_L}}$.
Similarly, we decompose the source term $\sb$ into a linear term $\sb_L$,
\begin{align}
  \eqnlab{linearsource}
  \sb_L := \dd{\sb}{\qb} \Bigg\vert_{\tilde{\qb}} \qb,
\end{align}
 and a nonlinear term $\sb - \sb_L$.
% \footnote{
% This approach avoids taking a partial derivative of the stabilization parameter in a numerical flux.}, 
Thus \eqnref{pde} becomes %is decomposed into a linear and a nonlinear parts,
\begin{align}
  \eqnlab{split-goveq-continuous}
   \dd{\qb}{t} + \Div \Fcal_L + \Div \Fcal_{\mc{N}} = \sb_L + \sb_{\mc{N}}
\end{align}
at the continuous level, 
where $\Fcal_{\mc{N}} = \Fcal - \Fcal_L$ and $\sb_{\mc{N}} = \sb - \sb_L$. 
The decomposition at continuous level avoids complicated derivatives
of the stabilization parameter coming from a numerical flux in DG
methods when applying exponential time integrators.
% The weak formulation of the DG methods in
A semi-discrete form of \eqnref{split-goveq-continuous}  using DG
discretization for spatial derivatives
 reads: 
find $\qb \in \Vbh(\Omegah)$ such that
  % \begin{subequations}
    \begin{align}
    \eqnlab{EXPO-SemiDiscretizedForm_ode}
      \LRp{\pp{\qb}{t},\vtest}_\Omegah %= \LRp{\dd{\qb}{t}, \vtest}_\Omegah
       &= L\qb + \mc{N}(\qb),
    \end{align}
  % \end{subequations}
 for all ${\bf v}\in \Vbh(\Omegah)$, 
  where 
%   \begin{align*}
%     \mc{N}(\qb) &=  \LRp{\Fcal_{\mc{N}}\LRp{\qb}, \Grad{\vtest}}_\Omegah
%                   + \LRp{\sb_{\mc{N}}(\qb),\vtest}_\Omegah
%                   - \LRa{\Fcals_{\mc{N}}\LRp{\qb^\pm} \cdot \n,\vtest}_\pOmegah,\\
%     L\qb  &= \LRp{\Fcal_L\LRp{\qb}, \Grad{\vtest}}_\Omegah
%                   + \LRp{\sb_L(\qb),\vtest}_\Omegah
%                   - \LRa{\Fcals_L\LRp{\qb^\pm} \cdot \n,\vtest}_\pOmegah
%   \end{align*} 
  % for the weak form, and
  
  \begin{align*}
    \mc{N}(\qb) &= - \LRp{\Div \Fcal_{\mc{N}}\LRp{\qb}, \vtest }_\Omegah
                  + \LRp{\sb_{\mc{N}}(\qb),\vtest}_\Omegah
                  - \LRa{ \LRp{ \Fcals_{\mc{N}}\LRp{\qb^\pm}
                              - \Fcal_{\mc{N}}\LRp{\qb} } \cdot \n,\vtest}_\pOmegah,\\
    L\qb  &= - \LRp{\Div \Fcal_L\LRp{\qb}, \vtest }_\Omegah
                  + \LRp{\sb_L(\qb),\vtest}_\Omegah
                  - \LRa{ \LRp{ \Fcals_L\LRp{\qb^\pm}
                              - \Fcal_L\LRp{\qb} } \cdot \n,\vtest}_\pOmegah.
  \end{align*} 
  
%   which, after an elementwise integration by parts, are equivalent to
%   \tanbui{do you use both forms in the codes? If not, describe only
%     the form that you implemented for the simplicity of the exposition.}
%  for the strong form with a periodic boundary condition. 
Here, %$\Fcal_{\mc{N}}:=\Fcal - \Fcal_L$ is a nonlinear flux; 
$\Fcal_L^*$ and $\Fcal_{\mc{N}}^*:=\Fcal^* - \Fcal_L^*$ 
are a linear and a nonlinear DG numerical flux, respectively, 
such that
%\begin{subequations}
\begin{align*}
  \LRa{\jump{ \Fcals_{\mc{N}}\LRp{\qb^\pm} \cdot \n},\vhtest}_\Gh = 0
\text{ and } 
  \LRa{\jump{ \Fcals_{L}\LRp{\qb^\pm} \cdot \n},\vhtest}_\Gh = 0,
\end{align*}
%\end{subequations}
for all $\vhtest \in \Lamh\LRp{\Gh}$. At this point both spatial linear and the nonlinear operators are discretized with DG, and  %in \eqnref{EXPO-SemiDiscretizedForm_ode}, 
we discuss exponential time integrators for temporal derivative next.
% The numerical flux \cite{LeVeque02} can be Lax-Friedrichs 
% (also known as Rusanov) \cite{rusanov1962calculation} or
% Roe\cite{roe1981approximate} flux, for example.
% \tanbui{If you use only one of them in your codes, say it here. If you
% specify it later in the numerical results, then remove this comment}

% Indeed, this choice increase accuray and stabilitytransforms the first-order ETD1 in \eqnref{etd1} 
% to the second-order EPI2 \cite{tokman2006efficient}, 
% \begin{align*}
%     q^{n+1} 
% %    &= q^n + (e^{L\dt} - I)L^{-1} L q^n 
% %    + \dt \varphi_1(L\dt) \mc{N}^n \\
%     &= q^n + \dt \varphi_1(L\triangle t) R^n
% \end{align*}
% where $q^{n+1} = q(t^{n+1})$, $q^n = q(t^n)$, $\mc{N}^n:=\mc{N}(q^n)$ and $R^n:=R(q^n)$.
% We will numerically demonstrate the benefit of using Jacobian as the linear operator in Section \secref{EXPO-numericalResults-ODE}. 





% \subsection{Model problems}


% \subsection{Bugers equation}

% Burgers equations appear often as a toy model, a simplification of a more complex model. It is used to understand some of the basic behavior of the sophisticated problem. 
% \begin{align}
% \eqnlab{pde-bugers-eq}
%  \dd{u}{t} + \half\dd{u^2}{x} 
%  = \dd{}{x} \LRp{\kappa \dd{u}{x} } \text{ in } \Omega
% \end{align}
% where $u$ is a scalar quantity, $\kappa >0 $ constant viscosity and $\Omega$ is a domain.

% Now the question is how to construct a Jacobian from the nonlinear right-hand side. 
% Inspired from IMEX methods, we linearize the full nonlinear equation in continuous level, and construct linear and nonlinear parts by adding and subtracting linear operator, i.e., 
% \begin{align}
% \eqnlab{pde-bugers-eq-split}
%  \dd{u}{t} 
%  = \underbrace{ 
%   \dd{}{x} \LRp{\kappa \dd{u}{x} - \tilde{u} u }
%   }_{Lu}
%    + \underbrace{
%    \dd{}{x}\LRp{ \tilde{u}u - \frac{u^2}{2}} 
%    }_{\mc{N}(u)}
%   \text{ in } \Omega
% \end{align}
% where $\tilde{u}$ is linearized $u$ evaluated at a base state, e.g., $\tilde{u} = u^n$. Note that the linear part $Lu$ is nothing but a linear convection-diffusion equation. 
% The DG weak formulation of \eqnref{pde-bugers-eq} reads: seek $q,u \in \Vh\LRp{\Omegah}$ such that 
% \begin{subequations}
% \eqnlab{gov-burgers1d}
% \begin{align}
%  \eqnlab{gov-burgers1d-gradu}
%  \LRp{q,p}_\Omegah &= 
%    \LRp{\dd{u}{x},p}_\Omegah + \LRa{n(u^* - u),p}_\pOmegah, \\
%    \eqnlab{gov-burgers1d-u}
%  \LRp{\dd{u}{t},v}_\Omegah 
%    &= \LRp{\dd{}{x} \LRp{\kappa q - \half u^2  },v}_\Omegah \nonumber \\
%    & + \LRa{ n\LRp{ \LRp{\kappa q - \half u^2}^* 
%                    -\LRp{\kappa q - \half u^2}   } ,v }_\pOmegah \nonumber \\
%    &- \LRp{\dd{ \tilde{u}u }{x},v}_\Omegah
%     - \LRa{ n\LRp{ \tilde{u}u^* - \tilde{u}u } ,v }_\pOmegah \nonumber \\
%    &+ \LRp{\dd{ \tilde{u}u }{x},v}_\Omegah
%     + \LRa{ n\LRp{ \tilde{u}u^* - \tilde{u}u } ,v }_\pOmegah
% \end{align}
% \end{subequations}
% for all $p,v \in \Vh\LRp{\Omega_h}$. 
% Here, we use central flux for $u^*$ and $q^*$ for diffusion operator, i.e.,
% $q^* = \half(q^+ + q^-)$ and $u^* = \half(u^+ + u^-)$, 
% and local Lax-Friedrich flux for inviscid Burgers part and the linear Jacobian part, i.e., 
% $ \half {u^*}^2 := \average{\half u^2} + \half \max(|u^\pm|)\jump{u}$ and
% $ \tilde{u}u^* := \average{u} + \half \max(|\tilde{u}^\pm|)\jump{u}$.
% %For Dirichlet boundary condition, we take $\uh = u_D$ and $\qh=q^-$. 
% We notice that \eqnref{gov-burgers1d-gradu} is a local operation,
% which means after $q$ is comptued from \eqnref{gov-burgers1d-gradu},
% we can plug $q$ in \eqnref{gov-burgers1d-u} element-by-element.
% By rearranging \eqnref{gov-burgers1d-u}, we define a linear and a nonlinear parts as
% \begin{align}
% \eqnlab{gov-burgers1d-dg-split}
%  L u &:= \LRp{\dd{}{x} \LRp{\kappa q - \tilde{u} u  },v}_\Omegah
%        + \LRa{ n\LRp{ 
%                       \LRp{ \kappa q - \tilde{u}u }^*
%                     - \LRp{ \kappa q - \tilde{u}u }  } ,v }_\pOmegah,\nonumber \\
%  \mc{N}(u) &:= \LRp{\dd{}{x} \LRp{\tilde{u} u - \half u^2 },v}_\Omegah \nonumber \\
%        &+ \LRa{ n\LRp{ 
%                       \LRp{ \tilde{u}u - \half u^2 }^*
%                     - \LRp{ \tilde{u}u - \half u^2 } } ,v }_\pOmegah.
% \end{align}










% \subsection{Euler equations}


% We consider Euler equations 
% \begin{subequations}
% \eqnlab{euler-gov}
% \begin{align}
%   \dd{\rho}{t}    + \Div\LRp{\rho\ub} &= s_\rho,\\
%   \dd{\rho\ub}{t} + \Div\LRp{\rho\ub\otimes\ub + \pres\Ical} &= s_{\rho \ub},\\
%   \dd{\rho E}{t} + \Div\LRp{\rho \ub H} &= s_{\rho E},
% \end{align}
% \end{subequations}
% where $\rho$ is the density;
%  $\ub$ is the velocity;
%  $\pres$ is the pressure;
%  $\rho E = \rho e + \half \rho \norm{\ub}^2$ is the total energy; $e=\frac{\pres}{\gamma -1}$ is the internal energy;
%  $H = E + \frac{\pres}{\rho} = \frac{a^2}{\gamma -1} + \frac{1}{2}\norm{\ub}^2$ is the total specific enthalpy;
%  $a = \sqrt{\frac{\pres}{\rho}}$ is the sound speed; 
%  $\gamma$ is the ratio of the specific heat;
%  $\Ical$ is the rank-1,2 or 3 identity matrix;
%  and $\sb$ is a source term. 
% % $g$ is the gravitational constant,

% For simplicity, we focus on one-dimensional Euler equations. 
% The core of the linearization is to introduce a flux Jacobian.
% In a compact form, \eqnref{euler-gov} can be written as
% \begin{align}
% \eqnlab{euler1d-gov}
%     \dd{\qb}{t}  = - \dd{\Fb(\qb)}{x} + \sb
% \end{align}
% with $\qb = (\rho, \rho u, \rho E)^T$, $\sb=(s_\rho, s_{\rho u}, s_{\rho E})^T$ and 
% $\Fb(\qb) = (\rho u, \rho u u + \pres, \rho u H)^T$. 
% We define the flux Jacobian $A:=\dd{\Fb}{\qb}$ by
% \begin{align}
% \eqnlab{euler1d-fluxJacobian}
%   A= 
%   \begin{pmatrix}
%     0 & 1 & 0\\
%     \half (\gamma-3) u^2 & (3-\gamma) u  & \gamma -1 \\
%     u\LRp{\half (\gamma-1) u^2 - H} & H + (1-\gamma) u^2 & \gamma u
%   \end{pmatrix},
% \end{align}
% evaluate $A$ at a reference state $\tilde{\qb}$, 
% and construct the following linear flux, 
% $\Fb_L:= A(\tilde{\qb}) \qb = \tilde{A} \qb$.
% By adding and subtracting the linear flux,
% we decompose \eqnref{euler1d-gov} into the following form, 
% \begin{align}
%   \eqnlab{euler-split-1d}
%   \dd{\qb}{t} = \underbrace{  \LRp{  - \dd{\Fb(\qb)}{x} +  \dd{\tilde{A}\qb}{x} }  }_{\mc{N}(\qb)}
%               + \underbrace{  \LRp{  - \dd{\tilde{A}\qb}{x} + \sb               }  }_{L\qb}.
% \end{align}
% By multiplying a test function $\vtest$ to \eqnref{euler-split-1d},
% integrating by parts twice for each element 
% and summing all the elements, we arrive at the strong formulation: seek $\qb \in \Vbh(\Omegah)$ such that 
% \begin{align}
%   \eqnlab{euler-strong-1d}
%   \LRp{\dd{\qb}{t},\vtest}_\Omegah
%     &= \LRp{ - \dd{\Fb(\qb)}{x} +  \dd{\tilde{A}\qb}{x} , \vtest}_\Omegah \nonumber \\
%     & + \LRa{ n \LRp{ -\LRp{\Fb(\qb^\pm)}^* + \LRp{\tilde{A}\qb^\pm}^*  }  , \vtest}_\pOmegah \nonumber\\
%     & - \LRa{ n \LRp{ -\Fb(\qb) + \LRp{\tilde{A}\qb}  }  , \vtest}_\pOmegah \nonumber \\
%     & + \LRp{\sb , \vtest}_\Omegah 
%       - \LRp{ \dd{\tilde{A}\qb}{x}, \vtest}_\Omegah \nonumber \\
%     & - \LRp{ n \LRp{ \LRp{\tilde{A}\qb^\pm }^* - \tilde{A}\qb }, \vtest}_\pOmegah
% \end{align}
% for all $\vtest \in \Vbh(\Omegah)$. 
% As for the numerical flux, we use Roe flux \cite{Roe81} 
% for both $\Fb^* (\qb^\pm)$ and $(\tilde{A}\qb^\pm)^*$, i.e.,
% \begin{subequations}
% \begin{align}
% \eqnlab{euler1d-roe-flux}
%   \Fb^* (\qb^\pm) & = \average{\Fb(\qb)} + \half |A(\qb)| \jump{\qb},\\
%   \LRp{\tilde{A}\qb^\pm}^* & = \average{\tilde{A}\qb} + \half |\tilde{A}| \jump{\qb},
% \end{align}
% \end{subequations}
% where $|A|:= R |\Lambda| R^{-1}$, 
% $|\Lambda| = diag(|u-a|,|u|,|u+a|)$ absolute eigenvalues, 
% \begin{align*}
%     \tilde{R} = \begin{pmatrix}
%     1 & 1 & 1 \\
%     u-a & u & u + a \\
%     H - au & \frac{u^2}{2} & H + au
%     \end{pmatrix}
% \end{align*}
% right eigenvectors and its inverse
% \begin{align*}
%     R^{-1} = \begin{pmatrix}
%     \LRp{\frac{\gamma-1}{4}}\frac{u^2}{a^2} + \frac{u}{2a} 
%     & -\LRp{\frac{\gamma-1}{a}}\frac{u}{a^2} - \frac{1}{2a} 
%     & \frac{\gamma-1}{2a^2} \\
%     1-\LRp{\frac{\gamma-1}{2}} \frac{u^2}{a^2} 
%     & (\gamma-1)\frac{u}{a^2} 
%     & \frac{1-\gamma}{a^2} \\
%     \LRp{\frac{\gamma-1}{4}}\frac{u^2}{a^2} - \frac{u}{2a} 
%     & -\LRp{\frac{\gamma-1}{a}}\frac{u}{a^2} + \frac{1}{2a} 
%     & \frac{\gamma-1}{2a^2} 
%     \end{pmatrix}
% \end{align*}
% whose rows are left eigenvectors. 
% The readers can refer Appendix \ref{appendix:EulerFluxJacobian} 
% for the flux Jacobian of two- or three-dimensional Euler equations. 
%Once we construct 



\subsection{Exponential time integrators}

For the clarity of the exposition, let us rewrite \eqnref{EXPO-SemiDiscretizedForm_ode} as\footnote{Note that we have absorbed the "mass matrix" into the definition of $L$ and $\mc{N}$.}
%In particular, we consider a nonlinear initial value problem, 
  % \begin{align}
  %   \eqnlab{nonlinear_ivp}
  %   \DD{\qb}{t} = R(\qb), \quad t\in\LRp{0,T},
  % \end{align}
\begin{align*}
    % \eqnlab{nonlinear_ivp_split}
    \DD{\qb}{t} = L\qb + \mc{N}(\qb), \quad t\in\LRp{0,T},
  \end{align*}  
with an initial condition $\qb_0 = \qb(0)$. % \in \R^\ell$.
% By splitting the right-hand side into a linear and a nonlinear parts, i.e.,
%   \begin{align}
%     \eqnlab{nonlinear_ivp_split}
%     \DD{q}{t} = Lq + \mc{N}(q), \quad t\in\LRp{0,T},
%   \end{align}
% and 
By multiplying an integrating factor $e^{-\dt L}$, we arrive at 
\begin{align}
\eqnlab{nonlinear_ivp_sol}
  \qb(t^{n+1}) = e^{\dt L} \qb(t^n) 
    + \int_0^\dt e^{(\dt - \sigma) L} \mc{N}(\qb(t^n+\sigma) ) d\sigma
\end{align}
by a simple application of the method of variation of constants. 
%This formula 
At this point, \eqnref{nonlinear_ivp_sol} is exact.
The first term $e^{\dt L}\qb(t^n)$ is the homogeneous solution, 
whereas the second term is the particular solution that involves a convolution integral with the matrix exponential.
Various exponential integrators have been proposed to approximate %by approximating 
\eqnref{nonlinear_ivp_sol} in different ways. 
In particular, % Taylor expansions \cite{cox2002exponential} or
 a $p$th-order time polynomial approximation to the nonlinear map $\mc{N}$ can be written as
 \begin{align*}
% \eqnlab{nonlinear_ivp_polynomial}
  % \mc{N}(q(t^n+\sigma)) \approx \sum_{j=0}^{p-1} \frac{t^j}{j!}N_j.
  % \mc{N}(q(t))
  \mc{N}(\qb(t^n+\sigma))
   = \sum_{j=0}^{p-1} \frac{\LRp{t^n+\sigma}^j}{j!}\vb_{j+1} + \mc{O}\LRp{\dt^p}, 
\end{align*}
with appropriate choice \cite{skaflestad2009scaling} for  $\vb_j$.
 This allows us to express an approximation of $\qb(t^{n+1})$ in \eqnref{nonlinear_ivp_sol}, 
 %again denoted as $\qb(t^{n+1})$,
 denoted as $\qb^{n+1}$,
as a linear combination of $\varphi$-functions \cite{niesen2012algorithm}, i.e., %acting on some vectors \cite{niesen2012algorithm}, i.e., 
\begin{align}
  \eqnlab{linear_combination_of_phifunctions}
  \qb^{n+1} = \sum_{i=0}^p (\dt)^i \varphi_i (\dt L) {\bf b}_i,
\end{align}
where we have defined ${\bf b}_0:=\qb(t^n)$ and 
${\bf b}_i:=\sum_{j=0}^{p-i}\frac{(t^n)^j}{j!} \vb_{i+j}$.
% Note that  \tanbui{We need to define what $v_i$ are here. Can $v_i$ be arbitrary?}. 
Here, $\varphi_i$-functions for a scalar $\tau$ are defined by
% \footnote{
% $\varphi_k$-function for a scalar $\tau$ argument is defined as
\begin{align*}
% \eqnlab{phi-functions}
  \varphi_i(\tau) := \int_0^1 e^{(1-z)\tau} \frac{z^{i-1} }{(i-1)!} dz
\end{align*}
with 
$\varphi_0(\tau):= e^{\tau}$. It is easy to see the recurrence relation
 $\LRs{\varphi_i(\tau) - \varphi_i(0)} \tau^{-1} = \varphi_{i+1} (\tau)$ and $\varphi_i(0) = \frac{1}{i!}$ hold true. The definition of $\varphi_i$-functions for matrices is straightforward, e.g., based on Jordan canonical form \cite{horn1994topics}.
 %The extended definition with matrices instead of scalars can be found in \cite{horn1994topics}, which is based on Jordan canonical form.

 % That means $(p+1)$ $\varphi$-function evaluations are needed.

 % \tanbui{{\bf Plan for proving the convergence of the scheme}: 1) Look at
 %   the EPI literature to see what assumptions on $L$ and $\mc{N}$ for
 %   the method to converge to which order. 2) Make a similar
 %   assumptions and state a general convergent results. Then 3) for
 %   each example in the numerical section, verify the assumptions as a
 %   lemma. The convergence of the Krylov subspace projection approximation is a
 %   separate issue, and we can point the readers to the literature on
 %   the convergence results.}
 % \shinhoo{I have searched several papers regarding the subject,
 % but I don't fine useful resources to tackle the problem. 
 % Tokman does not mentioned about the assumptions of $A$ and $\mc{N}$. 
 % Hochbruck explains the condition of $A$ and $\mc{N}$, 
 % but it does not seem to fit our problem. 
 % I think we should skip the convergence part. 
 % }

% We notice that \eqnref{linear_combination_of_phifunctions} requires $(p+1)$ $\varphi$-function evaluations, 
% which are known to be expensive. 
% To address the issue, 
For efficient computation of \eqnref{linear_combination_of_phifunctions},
Krylov subspace methods \cite{friesner1989method,
gallopoulos1992efficient,
hochbruck1998exponential} with the exponential of the augmented matrix can be used \cite{sidje1998expokit,al2009new,niesen2012algorithm,gaudreault2018kiops}. As will be seen in sections \secref{augmentedMatrix} and \secref{KrylovProjection}, the idea is to construct an augmented matrix and to project the large matrix onto a small Krylov subspace so that matrix exponential is amenable to compute. %.economical.


\subsection{Augmented matrix}
\seclab{augmentedMatrix}
%\tanbui{I am bit confused on the logic here. We are in a general setting where $L$ is a matrix, and then go to scalar case in section 2.3, and then now come back to matrix in this section.}
% Now, we need to addresss how to efficiently evaluate the action of $\varphi$-functions on a vector.
Suppose $L \in \R^{\ell\times\ell}$. Let 
$\Ical_p$ be the $p\times p$ identity matrix,
$\eb_i \in \R^p$ the $i$th canonical unit vector, 
$\bb$ an arbitrary vector in $\R^\ell$, 
 and 
$J:=\begin{pmatrix} 
  0 & \Ical_{p-1} \\ 
  0 & 0 
\end{pmatrix} \in \R^{p\times p} $. 
Following \cite{sidje1998expokit} we introduce 
the following augmented matrix, %$\tilde{L} \in \R^{(\ell+p)\times(\ell+p)}$
\begin{align*}
% \eqnlab{augmented_matrix_original}
  \tilde{L}\LRp{\bb} := \begin{pmatrix}
    L &  \bb \otimes \eb_1 \\
    0 &  J  
  \end{pmatrix}
  \in \R^{(\ell+p)\times(\ell+p)}.
\end{align*}
% To reduce the computational burden on the evaluations, 
% the authors 
% \cite{niesen2012algorithm} have proposed the alternative form based on the recurrence relation \eqnref{phi-functions}, 
% \begin{align}
% \eqnlab{nonlinear_ivp_polynomial_sol3}
%   q(t^{n+1}) = \sum_{m=0}^{p-1} \frac{(\dt)^m}{m!}w_m + (\dt)^p \varphi_p (\dt L) w_p
% \end{align}
% with $w_0=q(t^n)$ and $w_i = L w_{i-1} + \sum_{l=0}^{p-i} \frac{(t^n)^l}{l!} v_{l+i} \text{ for } i=1,2,\cdots,p$. 
% Only the action of $\varphi_p(\dt L)$ on a vector $w_p$ is required. 
% To compute $\varphi_p(\dt L) w_p$, 
% we let $L \in \R^{\ell\times\ell}$,
% $w_p,e_1 \in \R^\ell$ and 
% $J=\begin{pmatrix} 
%   0 & \Ical_{p-1} \\ 
%   0 & 0 
% \end{pmatrix}$, and introduce 
% an augmented matrix $\tilde{L} \in \R^{(\ell+p)\times(\ell+p)}$, 
% \begin{align}
% \eqnlab{augmented_matrix_original}
%   \tilde{L} = \begin{pmatrix}
%     L &  w_p e_1^T \\
%     0 &  J  
%   \end{pmatrix}.
% \end{align}
From \cite[Theorem 1]{sidje1998expokit}, the exponential of the augmented matrix is given by 
%we can compute the vector $\varphi_p(\dt L) w_p$ as follows,
% \tanbui{Please remove numbers on equations, everywhere, that you don't refer to. You can simply add * achieve the goal as I do here.}
\begin{align*}
  e^{\dt \tilde{L}\LRp{\bb}} =
    \begin{pmatrix}
      e^{\dt L} & \dt \varphi_1 (\dt L) \bb 
                & (\dt)^2 \varphi_2 (\dt L) \bb 
                & \cdots 
                & (\dt)^p \varphi_p (\dt L) \bb \\
      0 &  1 & \frac{\dt}{1 !} & \cdots & \frac{(\dt)^{p-1} }{(p-1)!} \\
      0 &  0 & 1  & \cdots & \frac{(\dt)^{p-2} }{(p-2)!} \\
      \vdots & \vdots & \vdots & \ddots & \vdots \\
      0 & 0 & 0 & 1 & \frac{\dt}{1!} \\
      0 & 0 & 0 & 0 & 1
    \end{pmatrix}.
\end{align*}
Note that
%We can obtain the evaluation of $(\dt)^{k}\varphi_k(\dt L) \bb$ by taking a matrix 
\begin{align*}
  (\dt)^{k}\varphi_k(\dt L) \bb 
  = \mc{S} 
  e^{\dt \tilde{L}\LRp{\bb_i}} \tilde{\eb}_{\ell+k},
\end{align*}
where $\mc{S} := \begin{pmatrix}
  \Ical_{\ell} & 0_{\ell\times p}
  \end{pmatrix}\in \R^{\ell\times(\ell+p)}$
  and $\tilde{\eb}_{\ell+k}$ is the $(\ell+k)$th canonical unit vector 
  in $\R^{\ell+p}$. Thus, \eqnref{linear_combination_of_phifunctions} can be written as
  \[
  \qb^{n+1} = \sum_{i=0}^p \mc{S} 
  e^{\dt \tilde{L}\LRp{\bb_i}} \tilde{\eb}_{\ell+k},
  \]
  which requires $(p+1)$ evaluations for each $\varphi$-function.
  
%Now, we can compute the linear combination in \eqnref{linear_combination_of_phifunctions},
% but this approach demands $(p+1)$ $\varphi$-function evaluations.
% That is, the first $\ell$ entries of the last column of $e^{\dt \tilde{L}}$ gives 
% the vector $(\dt)^p e^{\dt L} w_p$, i.e., 
% \begin{align}
%   \underbrace{
%   \begin{pmatrix}
%     (\dt)^p \varphi_p(\dt L) w_p\\
%   \tilde{w}
%   \end{pmatrix}
%   }_{\in \R^{(\ell+p)}} 
%   = 
%   \underbrace{
%   e^{\dt \tilde{L}} 
%   }_{\in \R^{(\ell+p)\times (\ell+p)} }
%   \underbrace{
%   \begin{pmatrix}
%     0\\
%     e_p
%   \end{pmatrix}
%   }_{\in \R^{(\ell+p)}}
% \end{align}
% where 
% $e_p=(0,0,\cdots,1)^T\in \R^{p}$ and 
% $\tilde{w}= \LRp{\frac{(\dt)^{p-1}}{(p-1)!},\cdots,\dt,1 }^T$. 
% However, the procedure in \eqnref{nonlinear_ivp_polynomial_sol3} may become sensitive to rounding errors when a large coefficient of $\varphi$-function is involved \cite{gaudreault2018kiops}. 
Recently, the work in \cite{gaudreault2018kiops} has suggested to compute
$(\dt)^{k}\varphi_k(\dt L) \bb_k$ in 
\eqnref{linear_combination_of_phifunctions}
simultaneously using the generalized augmented matrix:
\begin{align}
\eqnlab{augmented_matrix_general}
  \tilde{L} := \begin{pmatrix}
    L & B \\
    0 & J
  \end{pmatrix},
\end{align}
where $B:=(\bb_1,\bb_2,\cdots,\bb_p) 
= \bb_1 \otimes \eb_1 
+ \bb_2 \otimes \eb_{2} 
+ \cdots 
+ \bb_p \otimes \eb_p \in \R^{\ell\times p}$. 
The matrix exponential of the augmented matrix \eqnref{augmented_matrix_general} can be written as
\begin{align}
  \eqnlab{matrix_exponential_augmented_matrix}
  e^{\dt \tilde{L}} =
    \begin{pmatrix}
      e^{\dt L} & \dt \varphi_1 (\dt L) \bb_1 
              & \sum_{i=1}^2 (\dt)^i \varphi_i (\dt L) \bb_i 
          & \cdots 
          & \sum_{i=1}^p (\dt)^i \varphi_i (\dt L) \bb_i \\
      0 &  1 & \frac{\dt}{1 !} & \cdots & \frac{(\dt)^{p-1} }{(p-1)!} \\
      0 &  0 & 1  & \cdots & \frac{(\dt)^{p-2} }{(p-2)!} \\
      \vdots & \vdots & \vdots & \ddots & \vdots \\
      0 & 0 & 0 & 1 & \frac{\dt}{1!} \\
      0 & 0 & 0 & 0 & 1
    \end{pmatrix}.
\end{align}
We can then evaluate $\qb^{n+1}$ in \eqnref{linear_combination_of_phifunctions}
by taking the top $\ell$ elements from the matrix exponential \eqnref{matrix_exponential_augmented_matrix}, i.e., 
\begin{align}
\eqnlab{ExpFinal}
  \qb^{n+1} = \mc{S} 
  e^{\dt \tilde{L}} 
  \begin{pmatrix}
    \bb_0 \\
    \eb_p
  \end{pmatrix}.
\end{align}
%where $\bb_0\in \R^{\ell}$. 
What remains is to compute the matrix exponential acting on a vector on the right hand side \eqnref{ExpFinal}. %and we approximate it using a Krylov 
%subspace approach. 

\subsection{Krylov subspace projection-based methods}
\seclab{KrylovProjection}
% Since $\varphi$-functions can be solved simultaneously using the augmented matrix 
% \eqnref{augmented_matrix_general}, we focus on how $e^{A}b$ is approximated in Krylov subspace projection-based methods \cite{saad1992analysis}. 
The goal of this section is describe a Krylov subspace approach to approximate the right hand side of \eqnref{ExpFinal}. Let us begin with a given a matrix $A\in \R^{n\times n}$ and a vector $\bb \in \R^n$,
%we seek an approximation of $e^{A} \bb \in \Kcal_m$,
%$$\Kcal_m:= \text{span}\LRc{\bb,A\bb,A^2\bb, \cdots, A^{m-1} \bb }$$
%in $m$ dimensional Krylov subspace whose dimension is  $m <\!\!< n$. 
%To that end, we generate an orthonormal basis set 
%$$ V_m := \LRp{\vb_1,\vb_2,\cdots,\vb_m} $$
%through Arnoldi iterations \cite{arnoldi1951principle} in Algorithm \algref{arnoldi}, 
%	\begin{algorithm}[H]
%    		\begin{algorithmic}[1]
%			\STATE $\vb_1 = \bb/\norm{\bb}$
 %   			\FOR{$j=1$ to $m$}
 %   			  \STATE ${\wb = A \vb_j}$
 %   			  \FOR{$i=1$ to $j$}
 %   			    \STATE $\wb = \wb - {(\vb_i \cdot \wb)} \vb_i$
 %   			  \ENDFOR
 %   			  \STATE $h_{j+1,j} = {\norm{\wb}}$
 %   			  \STATE $\vb_{j+1} = \wb/h_{j+1,j}$
 %   			\ENDFOR
 %   		\end{algorithmic}
 %   		\caption{Arnoldi iterations}
 %   		\alglab{arnoldi}
 %   	\end{algorithm}
%%nd project the action of $A$ to the Krylov subspace,
and recall the Arnoldi iterations \cite{arnoldi1951principle} to generate an orthonormal basis $V_m$ of the $m$-th dimensional Krylov subpsace
\[
\Kcal_m:= \text{span}\LRc{\bb,A\bb,A^2\bb, \cdots, A^{m-1} \bb },
\]
so that
\begin{align*}
% \eqnlab{arnoldi-decomposition}
A V_m = V_m H_m + h_{m+1,m} \vb_{m+1} \otimes \eb_m,
\end{align*}
where $H_m = V_m^T A V_m \in \R^{m\times m}$ is the Hessenberg matrix,
%$h_{i,j}$ 
% \footnote{
%   $h_{m+1,m}$ can be considered as a residual of the projection 
%   of $A$ onto the Krylov subspace $\mc{K}_m$\cite{gaudreault2018kiops}.} 
%is the element of $H_m$; 
and $\eb_m \in \R^m$ is the $m$th canonical unit vector. 
The action of $e^{A}$ on $\bb$ 
can be approximated using the small matrix $H_m$ via
\begin{align}
\eqnlab{evaluation-phifunction-krylov}
  e^{A} \bb \simeq V_m e^{H_m} V_m^T \bb = \norm{\bb}_2 V_m e^{H_m} \eb_1,
\end{align}
with $\vb_1:=\bb/\norm{\bb}_2$ and $V_m^T \vb_1 = \eb_1$.
%Note that the size of $H_m$ is $m$-by-$m$.
Note that the evaluation of $e^{H_m} $ is less expensive than that of $e^{A}$ since $m \le n$.
Next, we evaluate the matrix exponential $e^{H_m}$ 
using Pad{\'e} approximation via the scaling and squaring method \cite{al2009new}.
%(we use EXPOKIT \cite{sidje1998expokit}). 

The accuracy of the approximation \eqnref{evaluation-phifunction-krylov} relies on the size of the Krylov subspace $m$ and the distribution of the eigenvalues of $A$. 
By  \cite[Theorem 2]{sidje1998expokit},
% \footnote
% {
% We obtain \eqnref{error-phifunction} when $p=0$ 
% from 
% Theorem 2 in \cite{sidje1998expokit}, which states that
% \begin{align}
%   \varphi_p(\tau A) b - \norm{b}_2 V_m \varphi_p(\tau H_m) e_1
%    = \norm{b}_2 \tau h_{m+1,m} \sum_{j=p+1}^\infty e_m^T \varphi_j (\tau H_m) e_1 \LRp{\tau A}^{j-p-1} v_{m+1}. 
% \end{align}
%   }
the error in the approximation 
\eqnref{evaluation-phifunction-krylov} satisfies 
\begin{align*}
  % \eqnlab{error-phifunction}
  \underbrace{ e^{A}\bb - \norm{\bb}_2 V_m e^{H_m} \eb_1}_{=: \varepsilon}
   = \norm{\bb}_2 h_{m+1,m} \sum_{j=1}^\infty \eb_m \otimes \varphi_j (H_m) \eb_1 A^{j-1} \vb_{m+1}. 
\end{align*}
This suggests {\it a posteriori} error estimate \cite{sidje1998expokit,niesen2012algorithm}:
\begin{align}
  \eqnlab{error-phifunction-posteriori}
  \norm{ \varepsilon }_2
   \simeq \norm{\bb}_2 \norm{  h_{m+1,m} \eb_m \otimes \varphi_1 (H_m) \eb_1 \vb_{m+1}}_2, 
\end{align}
under the assumption that the magnitude of $\varphi_1$ dominates the error for small $\norm{A}$ \cite{hochbruck1998exponential}.
% \tanbui{It is a good idea to state under which condition this is true.}.
Note that the error can be computed at no additional cost because the Arnoldi iteration already computes vector $\vb_{m+1}$ and the multiplication with the matrix $A$ is not required \cite{niesen2012algorithm}. 
The {\it a posteriori} error estimate \eqnref{error-phifunction-posteriori} is easily computed by 
introducing an augmented matrix $\tilde{H}_m \in \R^{(m+1) \times (m+1)}$
\begin{align*}
% \eqnlab{augmented-matrix-hessenberg}
\tilde{H}_m = 
  \begin{pmatrix}
    H_m & \eb_1 \\
    0 & 0
  \end{pmatrix}, 
\end{align*} 
and using the top right element of the
 matrix exponential 
\begin{align}
  \eqnlab{augmented-matrix-hessenberg-exponential}
  e^{\tilde{H}_m} = 
  \begin{pmatrix}
    e^{H_m} & \varphi_1(H_m) \eb_1 \\
    0 & 1 
  \end{pmatrix}.
\end{align}
Once the error estimate is computed, we can control the accuracy of 
the approximation \eqnref{evaluation-phifunction-krylov}. 
For example, if the spectrum of $A$ is broad, we can either increase the size $m$ of the Krylov subspace or downsize the eigenvalues of $A$. 

%As can be seen from \eqnref{nonlinear_ivp_polynomial_sol2},  
%As can be seen from \eqnref{linear_combination_of_phifunctions},
%of interest is $A = \dt L$. 
When $A=\dt \tilde{L}$, which is what needed in \eqnref{matrix_exponential_augmented_matrix}, 
we can also control the accuracy of \eqnref{evaluation-phifunction-krylov} by splitting $\dt$ into a sum of smaller intervals, i.e., 
$\dt = \tau_1 + \tau_2 + \cdots + \tau_k$, 
and then computing the matrix exponential iteratively\footnote{This is equivalent to a time-stepping method with small sub-step sizes.}, i.e.,
% \tanbui{$L$ should be replaced by $\tilde{L}$?}
\begin{align*}
  e^{\dt \tilde{L}} \bb 
  = e^{\tau_k \tilde{L} }\LRp{ \cdots \LRp{ e^{\tau_2 \tilde{L}} \LRp{e^{\tau_1 \tilde{L}} \bb} }  }.
\end{align*}

Based on {\it a posteriori} error in \eqnref{error-phifunction-posteriori}, 
the work in \cite{niesen2012algorithm} develops {\texttt {phim}} algorithm
to carry out the matrix exponential efficiently 
by adaptively adjusting the size of the Krylov subspace and the number of sub-steps\footnote{We define the total number of Krylov steps, $N_{Krylov}$, by accumulating the size of the Krylov subspace at each sub-step.}.
Along this line, \texttt{KIOPS} \cite{gaudreault2018kiops} and \texttt{phipm/IOM2} \cite{luan2019further} have been developed to
improve the adaptive Krylov algorithm {\texttt{phim}} by replacing the Arnoldi iteration with 
the incomplete orthogonalization procedure (IOP)
\cite{koskela2015approximating}. % in Algorithm \algref{iop}.
Within IOP,
a Krylov basis is not necessarily orthogonal to all the bases. 
In particular, each Krylov vector $\vb_j$ in $V_m$ is set to be orthogonal to only
$\ell$ ($< m$) bases, i.e., 
$\vb_{\max(1,j-\ell)},\cdots,\vb_{j-1}$. 
This reduces the orthgonalization cost from $\mc{O}(m^2 n)$ to $\mc{O}(\ell m n)$ in Arnoldi iterations. 
%\tanbui{what is ``the $o$ number of bases''?}

%	\begin{algorithm}[H]
%    		\begin{algorithmic}[1]
%			\STATE Set orthogonal length $\ell$ %\tanbui{quite
%            %            a weird notation $o$?}
%			%\STATE $v_1 = b/\myblue{\norm{b}}$
%			\STATE $\vb_1 = \bb/\norm{\bb}$
%    			\FOR{$j=1$ to $m$}
%    			  %\STATE $\myred{w = A (v_j)}$
%    			  \STATE $\wb = A (\vb_j)$
%    			  \FOR{$i=\max(1,(j-\ell)+1)$ to $j$}
%    			    %\STATE $w = w - \myblue{(v_i^Tw)} v_i$
%    			    \STATE $\wb = \wb - (\vb_i \cdot \wb) \vb_i$
%    			  \ENDFOR
%    			  %\STATE $h_{j+1,j} = \myblue{\norm{w}}$
%    			  \STATE $h_{j+1,j} = \norm{\wb}$
%    			  \STATE $\vb_{j+1} = \wb/h_{j+1,j}$
%    			\ENDFOR
%    		\end{algorithmic}
%    		\caption{Incomplete orthogonal procedure}
%    		\alglab{iop}
%    	\end{algorithm}

In this paper, we use \texttt{KIOPS} algorithm for serial computations.
For parallel computation, we have implemented an exponential time integrator based on the \texttt{KIOPS} algorithm for our C\texttt{++} DG finite element library
%on top of the DG finite element library written in C\texttt{++}, 
(a spin-off from \texttt{mangll}
\cite{wilcox2010high}).
% \tanbui{If your library is easier to understand with comments, we
%   should make it open-source. This improves your visibility and
%   track-record of releasing open-source codes for the community.}
% \shinhoo{
% I would like to make it open-source, but postpone it at this moment.
% Its quality is not ready yet for publishing. 
% }
For computing the matrix exponential in \eqnref{augmented-matrix-hessenberg-exponential},
we use \texttt{EIGEN}\cite{guennebaud2014eigen}. %C\texttt{++} library.
Parallel implementations mainly focus on vector-vector and matrix-vector multiplication in IOP. %in incomplete orthogonal procedure in Algorithm \algref{iop}.
The matrix-vector multiplication, e.g. $A\vb_j$, is carried out in a matrix-free manner 
by acting the linear operator $A$ on the vector $\vb_j$. % in Algorithm \algref{iop}.
Thanks to DG discretization, the action $A\vb_j$ is
highly 
parallel as the communication cost can be  effectively overlapped by computation. 
% \tanbui{vector-vector multiplication is standard, unless you do
%   something different and more effective and there is no need
% to talk about it here}
Clearly, vector-vector multiplication %, e.g. $\norm{\bb}$, $\norm{\wb}$ and $\vb_i \cdot \wb$ in Algorithm \algref{iop},
% % we scatter a global vector to each processor,
% %  perform the dot product with the scatted local vector, 
% % and call \texttt{MPI ALLreduce} function. 
% %This 
requires a global communication, but its cost is relatively small compared to the overall computational cost.



==> NumericalResults2.tex <==
\section{Numerical Results}
\seclab{NumericalResults}

% \tanbui{
% Our main point to show for exponential DG is: 1) its stability is similar to
% implicit method, 2) its cost is similar to explicit RK DG method (and thus
% more efficient than implicit DG method), 3) its paralell
% scalability is similar to explicit DG methods, 3) it is high-order in
% both space and time; 4) it can deal with stiff problems robustly and
% efficiently (large Courant numbers without stability compared to
% explicit methods, and much less cost compared to fully implicit
% method, and 5) it is more efficient, e.g. scalability, than IMEX methods.
% If you can show all these points, the method (and hence the paper) is
% very convincing and appealing. Otherwise, we will run into the
% problems with the reviewers later and it will be very hard to publish
% the work. We have already had similar experinece with the IMEX HDG-DG
% paper, and we don't want to run in to the same problems again if we
% like to publish the work in SISC, or JCP, or CMAME.
% }
% \shinhoo{
%   We show the main point through numerical examples.
%   Exponential DG 
%   1) is stable with a large Courant number ($Cr>1$) similar to IMEX DG;
%   2) becomes comparable to RKDG on uniform grid, and beneficial on nonuniform grid;
%   3) shows similar parallel performance to RKDG; 
%   4) supports high-order solutions in space and time in isentropic vortext case;
%   5) is more efficient than IMEX DG in terms of computational cost. 
% }
  
In this section, we conduct several numerical experiments 
to evaluate the performance of the proposed framework.
In particular, we examine the numerical stability for a wide range of Courant numbers $(Cr>1)$;
the high-order convergence; the accuracy and the efficiency; its weak and strong scalability.
For numerical simulations, 
we consider a system of ordinary differential equations
(ODE), Allen-Cahn equation, viscous Burgers
equation, and Euler equations. 



% differential equations (ODE) with different linearized forms. Then, we
%  deal with
% the one-dimensional Allen-Cahn equation and viscous Burgers
% equation. Finally, we solve Euler equations in two- and
% % three-dimensional domains.
% Of interest are the high-order convergence in both time and space, the
% strong and weak
% scalability, and the ability to use large Courant number ($Cr > 1$) of
% the proposed approach.

%\tanbui{We need to present the convergence in space as
%  well to justify the proposed exponential DG.}

\subsection{A system of two ordinary differential equations (ODE)}
\seclab{EXPO-numericalResults-ODE}

%Exponential time integrators require the decomposed system in \eqnref{nonlinear_ivp_split}, i.e., the linear and the nonlinear terms.
% In Exponential DG framework, we construct the linear term in \eqnref{linearflux} and \eqnref{linearsource}, based on linearization.
% This is because linearized operators typically  capture the rapidly varying physics. 
% %This is one way to build the linear term in \eqnref{nonlinear_ivp_split}.
% We will illustrate the benefit of using Jacobian in the following example.
%The question is how we build the linear operator?

We consider the autonomous system of two ODEs
 proposed by \cite{cox2002exponential}
\begin{subequations}
\begin{align}
  \DD{u(t)}{t} &= c u - v + (\lambda v - c u)  r^2, \\
  \DD{v(t)}{t} &= u + c v - (\lambda u + c v)  r^2,
\end{align}
 \eqnlab{ode-system-ex-goveq}
\end{subequations}
where $r^2 = u^2 + v^2$, $c>0$ constant, 
$u=r\cos \theta$, $v = r\sin\theta$. 
The exact solution is given by 
% \begin{subequations}
\begin{align*}
  r^2(t) &= r_0^{2}
  \LRp{r_0^2 \LRp{1-e^{-2 c t }} + e^{-2 c t} }^{-1},\\
  \theta(t) &= \theta_0 + (1-\lambda)t 
             - \frac{\lambda}{2 c} 
             \log\LRp{r_0^2 \LRp{1-e^{-2 c t}} + e^{-2c t} }.
\end{align*}
 % \eqnlab{ode-system-ex-exactsolution}
% \end{subequations}
For a numerical simulation, we take $c=100$,
$\lambda=\half$, $u_0 = u(0)=2$ and $v_0= v(0)=1$. 
The exact solution with the parameters is shown in Figure \figref{system-ode-ex-sol}.
The magnitude and the phase of the solution rapidly change within a
short period of time. 

%---------------------
% EXACT SOLUTION PLOT
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Magnitude]{
      \includegraphics[trim=1.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.45\textwidth]{./figures/EXPO-SystemODE-exact-magnitude}
      \figlab{system-ode-ex-exact-magnitude}
    }
    \subfigure[Phase]{
      \includegraphics[trim=1.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.45\textwidth]{./figures/EXPO-SystemODE-exact-phase} 
      \figlab{system-ode-exact-phase}
    }
    \caption{System of two ODEs: (a) magnitude and (b) phase of the exact solution.}
     % of 
     %  \eqnref{ode-system-ex-exactsolution}. }
    \figlab{system-ode-ex-sol}
  \end{figure}


Let $\qb=(u,v)^T$ and $\Rb(\qb)$ be the right hand-side of \eqnref{ode-system-ex-goveq}. We define two linear operators:
one is the constant linear operator \cite{cox2002exponential}
\begin{align}
\eqnlab{linearop-const}
L_{c}:=\begin{pmatrix}
c & -1\\
1 & c
\end{pmatrix}
\end{align} 
and the other is Jacobian 
%\tanbui{Please recheck. I could be wrong,
%  but a quick check on the second row does not give the same results
%  as yours. Also the Jacobian is a function of $\qb$, we should
%  make it clear in the definition of $L_d$, e.g. $L_q\LRp{\qb}$. To be consistent with
%  \eqnref{linearflux}, we should also use $\tilde{\qb}$ here.}
%How do we choose a linear operator to capture the characteristics of a rapidly changing system?
%To address the question, we consider the two linear operators: 
%the dynamic Jacobian operator
\begin{align}
\eqnlab{linearop-dynamic}
L_{d}\LRp{\qbtilde}:=\dd{\Rb}{\qb}\bigg|_\qbtilde
=\begin{pmatrix}
    c(1-\rtilde^2) + 2 \utilde (\lambda \vtilde - c \utilde) 
  & -1 + \lambda \rtilde^2 + 2 \vtilde (\lambda \vtilde - c \utilde) \\
    1 - \lambda \rtilde^2 - 2 \utilde (\lambda \utilde + c \vtilde)
  & c(1-\rtilde^2) - 2 \vtilde (\lambda \utilde + c \vtilde) 
\end{pmatrix}.
\end{align}
% evaluated at each timestep $t^n$, 
%Since $L_d$ is a function of $(u,v)$, we can dynamically update $L_d(u^n,v^n)$ at each time $t^n$,
%whereas $L_c$ is a constant matrix, which may not capture the fast characteristics of the system.

The first-order exponential time differencing (ETD1) method \cite{cox2002exponential} 
reads
\begin{align}
  \eqnlab{etd1}
  \qb^{n+1}
  = e^{\dt L} \qb^n
  + \dt \varphi_1 (\dt L) \mc{N}^{(0)},
\end{align}
where
$\qb^n:=\qb(t^n)$, $L=L_d \text{ or } L_c$,
$ \mc{N}^{(0)} := \Rb^n - L \qb^n$ and 
$\Rb^n:=\Rb(\qb^n)$. 
We denote ETD1 method with the constant linear operator \eqnref{linearop-const} by ETD1-L, 
and the one with the Jacobian \eqnref{linearop-dynamic} by ETD1-J 
in which the Jacobian is evaluated at each timestep. 
We also let the ETD1 method with the fixed Jacobian \eqnref{linearop-dynamic} 
evaluated at $\qbtilde_0=(u_0,v_0)^T$ by ETD1-J0.
Indeed, ETD1-J is equivalent to the second-order EPI2 \cite{tokman2006efficient},
\begin{align*}
  \qb^{n+1}
  &= \qb^n + \dt \varphi_1(L_d\triangle t) \Rb^n.
\end{align*}
This form is computationally attractive because it needs only one matrix exponential instead of two in \eqnref{etd1} \cite{hochbruck2010exponential}. 

\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-ode-tconv}
  \caption{System of two ODEs: time convergence study of ETD1-L, ETD1-J, and EPI2.
  We observe the first-order convergence rate for ETD1-L and the second-order convergence rate for ETD1-J and EPI2.
  The use of Jacobian improves not only the accuracy but also the stability of ETD1. }
  \figlab{expo-ode-tconv}
\end{figure}


Figure \figref{expo-ode-tconv} demonstrates the benefit of using the Jacobian in terms of accuracy and stability. 
We measure the errors of magnitude $r$ and phase $\theta$ at $T=1$ for ETD1-L, ETD1-J, and EPI2 methods. 
The error levels of ETD1-J0 for $r$ and $\theta$ are three orders of magnitude and four times larger than ETD1-L counterparts, respectively.
However, ETD1-J0 shows better stability than ETD1-L.
The errors of ETD1-L and ETD1-J0 show the first-order convergence rate in both the magnitude and the phase errors,
whereas the ETD1-J counterpart shows the second-order convergence rate.
Not only that, ETD1-J allows a larger timestep size without facing
instabilities.  %than ETD1-L.
This demonstrates the importance of using Jacobian.
%\tanbui{you didn't discuss the reference value $\tilde{u}$ here. Does
%  it change for each time step? We should compare the case with fixed
%  reference $\tilde{\qb}$ and varying (linearize around the solution of
%  the previous time step) $\tilde{\qb}$}


%% \begin{table}[t]
%% \caption{System of two ODEs: time convergence study of ARS111 and ETD1.
%% Using $L_d$ gives better stability and accuracy than using $L_c$. 
%% With the small timestep size ($dt < 10^{-3}$), 
%% ETD1 solutions are more accurate than ARS111 solutions. 
%% }
%%  \tablab{expo-ode-tconv}
%% \begin{center}
%% \begin{tabular}{*{1}{c}|c||cccc|cccc}
%% \hline
%% \multirow{2}{*}{ $L$ } 
%%   & \multirow{2}{*}{dt} 
%%   & \multicolumn{4}{c|}{$ETD1$}   
%%   & \multicolumn{4}{c}{$ARS1$}   \tabularnewline
%%     &    
%%     &   $\norm{r - r^e}$ & {\small rate} & $\norm{\theta-\theta^e}$ & {\small rate}
%%     &   $\norm{r - r^e}$ & {\small rate} & $\norm{\theta-\theta^e}$ & {\small rate}\tabularnewline
%% \hline\hline
%% \multirow { 6}{*}{    $ L_c$ }& 2.0E-5 & 1.3E-08 &        - & 5.2E-04 &        - & 3.8E-08 &        - & 1.0E-03 &        - \tabularnewline
%%                          & 5.0E-5 & 3.1E-08 &      1.0 & 1.3E-03 &      1.0 & 9.4E-08 &      1.0 & 2.6E-03 &      1.0 \tabularnewline
%%                          & 1.0E-4 & 6.2E-08 &      1.0 & 2.6E-03 &      1.0 & 1.9E-07 &      1.0 & 5.2E-03 &      1.0 \tabularnewline
%%                          & 2.0E-4 & 1.3E-07 &      1.0 & 5.2E-03 &      1.0 & 3.8E-07 &      1.0 & 1.1E-02 &      1.0 \tabularnewline
%%                          & 5.0E-4 & 3.1E-07 &      1.0 & 1.3E-02 &      1.0 & 9.9E-07 &      1.0 & 2.7E-02 &      1.0 \tabularnewline
%%                          & 1.0E-3 & 6.1E-07 &      1.0 & 2.6E-02 &      1.0 & 2.1E-06 &      1.1 & 5.6E-02 &      1.1 \tabularnewline
%% \multicolumn{6}{c}{} \tabularnewline
%% \multirow { 9}{*}{    $ L_d$ }& 2.0E-5 & 1.7E-11 &        - & 2.8E-08 &        - & 1.3E-08 &        - & 2.1E-06 &        - \tabularnewline
%%                          & 5.0E-5 & 1.0E-10 &      2.0 & 1.8E-07 &      2.0 & 3.1E-08 &      1.0 & 5.2E-06 &      1.0 \tabularnewline
%%                          & 1.0E-4 & 4.2E-10 &      2.0 & 7.5E-07 &      2.0 & 6.1E-08 &      1.0 & 1.0E-05 &      1.0 \tabularnewline
%%                          & 2.0E-4 & 1.7E-09 &      2.0 & 3.2E-06 &      2.1 & 1.2E-07 &      1.0 & 2.0E-05 &      1.0 \tabularnewline
%%                          & 5.0E-4 & 1.1E-08 &      2.0 & 2.3E-05 &      2.1 & 2.8E-07 &      0.9 & 5.4E-05 &      1.1 \tabularnewline
%%                          & 1.0E-3 & 4.4E-08 &      2.0 & 9.2E-05 &      2.0 & 5.0E-07 &      0.8 & 1.6E-04 &      1.5 \tabularnewline
%%                          & 1.0E-2 & 6.3E-06 &      2.2 & 4.8E-03 &      1.7 & 6.3E-06 &      1.1 & 9.0E-03 &      1.8 \tabularnewline
%%                          & 1.0E-1 & 1.1E-03 &      2.2 & 1.6E-01 &      1.5 & 1.1E-03 &      2.3 & 1.8E-01 &      1.3 \tabularnewline
%%                          & 1.0 & 6.0E-01 &      2.7 & 5.2E-01 &      0.5 & 6.0E-01 &      2.7 & 5.2E-01 &      0.5 \tabularnewline
%% \hline\hline
%% \end{tabular}
%% \end{center}
%% \end{table}
 

%% We also perform the time convergence study for ARS111 in Figure \figref{expo-ode-tconv-ars}.
%% ARS111-L and ARS111-J stand for ARS111 method with the constant linear operator \eqnref{linearop-const} 
%% and the dynamic Jacobian \eqnref{linearop-dynamic}, respectively.
%% ARS111-L shows the first-order convergence rate, 
%%     whereas ARS111-J shows the first-order convergence rate
%%   near $10^{-4}$ timestep size, but the second-order convergence rate 
%%   as loosen the timestep size.
%% This implies that the error associated with the fast modes starts to dominate as tighten the timestep size. 
%% We also notice that the difference of the phase error between ARS111-L and ARS111-J 
%% is relatively larger than that of the magnitude error. 
%% The same behavior is observed between ETD1-L and ETD1-J. 
%% The dynamic Jacobian $L_d$ significantly improves the phase error.
%% We tabulate the time convergence results in Table \tabref{expo-ode-tconv}.
%% We see that ETD1 solutions are more accurate than ARS111 solutions
%% with the small timestep sizes ($dt < 10^{-3}$).
%% This makes sense because the IMEX scheme is known to damp out the high-frequency modes in the system,
%% whereas exponential integrators exactly treat the fast modes. 
%% In particular, exponential integrators subdivide a timestep size $\triangle t$ into several sub-steps $\triangle t=\tau_1 + \tau_2  + \cdots$ and march the approximation step-by-step
%% similar to an explicit time integration method. 
%% Overall, exponential integrators are promising in the sense that it is not only accurate but also stable with a large timestep size. 


% \subsection{Allen-Cahn equation}

% In this section we consider the following Allen-Cahn equation:
% \begin{align*}
% % \eqnlab{pde-allen-eq}
%  \dd{u}{t} 
%   = \dd{}{x} \LRp{\kappa \dd{u}{x} } - \LRp{u^3 - u} \text{ in } \Omega,  
% \end{align*}
% with $\Omega=\LRc{x: x \in \LRp{-1,1} }$, the following smooth initial solution, 
% %We choose a smooth initial condition,
% \begin{align*}
%     u(x,t=0) = 0.53 x + 0.47 \sin(-1.5\pi x)
% \end{align*}
% and a constant viscosity $\kappa=0.001$.
% We impose Dirichlet boundary conditions, 
% $u(-1,t) = -1$ and $u(1,t) = 1$. 


% %-------------------------
% % EXAMPLES FOR ALLEN-CAHN EQ.
% %-------------------------
% \begin{figure}[h!t!b!]
%     \centering
% %    \subfigure[Gaussian]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
% %      \figlab{pde-burgers-ex-Gaussian}
% %    }
%   % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-Allen-smooth}
%   % \figlab{pde-allen-ex-smooth}
%     \subfigure[solutions]{
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Allen-smooth}
%       \figlab{pde-allen-ex-smooth}
%     }
%     \subfigure[differences]{
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Allen-smooth-difference}
%       \figlab{pde-allen-ex-smooth-difference}
%     }
% %    \subfigure[Tanh]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
% %      \figlab{pde-burgers-ex-Tanh}
% %    }    
%     %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
%     \caption{(a) Smooth solutions and (b) their differences with RK4 for Allen-Cahn equation at $t=1$.
% RK2 with $Cr_d=0.16$, EPI2 with $Cr_d=26.8$ and EPI2 with $Cr_d=56.7$ are simulated with
% $k=4$ solution order and $N_e=80$ elements.
% Dirichlet boundary conditions are imposed at $x=-1$ and $x=1$.}
%     \figlab{pde-allen-smooth}
%   \end{figure}
  
% We perform the simulation for $t \in [0, 1]$ with  $k = 4$ solution
% order and a uniform mesh with $N_e = 80$ elements.
% We define the diffusion Courant number $Cr_d=\frac{\kappa dt}{(dx)^2}$ where 
% $dx$ is the minimum distance between the interpolation nodes on $\Omega$. 
% %\tanbui{is the mesh uniform or not? Please state it.}
% The solution snapshots (at $t = 1$) for the second-order Runge-Kutta method (RK2)
% with $Cr_d=0.16$ and EPI2 ($Cr_d=26.8$ and $Cr_d=56.7$) are shown 
% in Figure \figref{pde-allen-smooth}.
% % \tanbui{I think we should put the curves on the same figure with
% %   different colors/symbols to clearly see the similarity of the
% %   solutions that we claim. Also, the plot at $t=0$ is not meaningful/necessary
% %   but makes the figures busy/confused. Please remove the initial
% %   condition plots, and do the same for the
% %   other numerical examples below.}
% Both the EPI2 solutions with $Cr_d=26.8$ and $Cr_d=56.7$ produce a similar result to the RK2 counterpart even with two orders of magnitude larger timestep size. 
% Compared to the EPI2 solution with $Cr_d=26.8$, we see that the EPI2 solution with $Cr_d=56.7$ has a larger difference from the RK4 due to the time truncation error. 
% We conduct a temporal convergence study for EPI2 and EXPRB32\footnote{
% EXPRB32  \cite{hochbruck2010exponential} is the third-order two-stage method,
% \begin{align*}
%   q^{(2)} &= q^n + \dt \varphi_1(L \dt) R^n,\\
%   q^{n+1} &= q^n + \dt \varphi_1(L \dt) R^n
%                  + \dt \varphi_3(L \dt) 2 D_{n,2},
%   %q^{n+1} = q^n  + \dt \varphi_1(L \dt) R^n + \frac{2}{3}\dt \varphi_2 (L \dt) D_{n,2},
% \end{align*}
% where $D_{n,2}:= \LRp{R(q^{(2)}) - L q^{(2)}} - \LRp{R(q^{n}) - L q^n}$.
% %Since this method requires both $q^0$ and $q^1$ solutions for advancing in time, 
% %we compute $q^1$ using EPI2 method, in which the local error is the third-order, 
% %so that the global error of EPI3 becomes the third-order. \tanbui{Is
% %  the statement true? I thought that global error is always one-order
% %  less than the local error?}
% } by taking 
% the RK4 solution (with $dt=2\times 10^{-5}$, $k=10$ and $N_e=80$)
% as ``the ground truth'' solution.
% As expected, the theoretical convergence rates (second and third orders) are observed for EPI2 and EXPRB32 
% in Table \tabref{expo-allen-tconv-smooth}.

% \begin{table}[t]
% \caption{A smooth function for Allen-Cahn equation:
% time convergence study is conducted with $k=4$ solution order and $N_e=80$ elements. 
% The expected second- and third-order convergence rates are
% observed for EPI2
% and EXPRB32, respectively.}
% \tablab{expo-allen-tconv-smooth}
% \begin{center}
% %\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
% \begin{tabular}{cc||cc|cc}
% \hline
% \multirow{2}{*}{$dt$} 
% & \multirow{2}{*}{$Cr$}
% & \multicolumn{2}{c|}{ EPI2 } 
% & \multicolumn{2}{c}{ EXPRB32 } \tabularnewline
%   &  &  error & order & error & order \tabularnewline
% \hline\hline
%   0.50 & 115.83 & 1.179E-02 &      $-$ &       1.636E-03 &      $-$ \tabularnewline 
%   0.10 & 23.17  & 2.993E-03 &    1.978 &       1.462E-04 &    3.485 \tabularnewline 
%   0.05 & 11.58  & 4.898E-04 &    1.975 &       7.593E-06 &    3.228 \tabularnewline 
%   0.01 & 2.32   & 1.237E-04 &    1.986 &       8.869E-07 &    3.098 \tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}




\subsection{Viscous Burgers equation}

We consider a steady-state manufactured solution,
$$ u(x,t) = \sin(x^2) x (x-1) $$ 
by adding a source term to \eqnref{pde-burgers-eq}. 
We perform 
a spatial convergence study with Lax-Friedrich (LF) flux and entropy flux (EF),
where we take $\sigma=0$ and $\sigma=3\times 10^{-4}$. 
We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
The error is measured at $t=0.01$ and the results are summarized in Table \tabref{expo-burgers-sconv-mms}.
% with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.
In general, the convergence results show similar behavior.
All the error levels are similar to each other.
We also see that the rates of convergence with LF and EF are not optimal for odd order,
e.g., both the rates for $k=3$ are $\mc{O}(h^3)$, but optimal for even order. 
This behavior is well-known for parabolic equations with a central flux \cite{cockburn1998local}.
However, for the case of EF $(\sigma=3\times 10^{-4})$,  
we observe that the rate of convergence tends to increase 
due to the presence of the non-zero jump term.  
These results support our theoretical results. 

In the following two examples: smooth solution and shock solution, 
we use EF flux for EPI2 and EXPRB32. 
% \begin{table}[t]
% \caption{A smooth solution for viscous Burgers equation:
% a spatial convergence study is conducted with Lax-Friedrich (LF) flux and entropy flux (EF). 
% We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
% The error is measured at $t=0.01$ with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.}
% \tablab{expo-burgers-sconv-smooth}
% \begin{center}
% \begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}}
% \hline
% \multirow{2}{*}{}%$k=16$} 
%   & \multirow{2}{*}{$h$}  
%   & \multicolumn{2}{c|}{$LF$}   
%   & \multicolumn{2}{c|}{$EF$}   
%   \tabularnewline
%   &    &  error & order &  error & order       \tabularnewline
% \hline\hline
% \multirow { 4}{*}{   k=1}&  0.050 & 7.047E-03 &      $-$ & 7.116E-03 &      $-$ \tabularnewline
%                          &  0.030 & 2.092E-03 &    1.752 & 2.272E-03 &    1.647 \tabularnewline
%                          &  0.010 & 6.967E-04 &    1.586 & 9.015E-04 &    1.334 \tabularnewline
%                          &  0.005 & 2.646E-04 &    1.397 & 4.175E-04 &    1.111 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=2}&  0.050 & 3.013E-04 &      $-$ & 3.038E-04 &      $-$ \tabularnewline
%                          &  0.030 & 3.373E-05 &    3.159 & 3.385E-05 &    3.166 \tabularnewline
%                          &  0.010 & 3.985E-06 &    3.082 & 3.992E-06 &    3.084 \tabularnewline
%                          &  0.005 & 4.907E-07 &    3.022 & 4.912E-07 &    3.023 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=3}&  0.050 & 3.252E-05 &      $-$ & 3.284E-05 &      $-$ \tabularnewline
%                          &  0.030 & 3.750E-06 &    3.116 & 3.876E-06 &    3.083 \tabularnewline
%                          &  0.010 & 4.629E-07 &    3.018 & 4.775E-07 &    3.021 \tabularnewline
%                          &  0.005 & 5.739E-08 &    3.012 & 5.944E-08 &    3.006 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=4}&  0.050 & 1.599E-06 &      $-$ & 1.602E-06 &      $-$ \tabularnewline
%                          &  0.030 & 5.413E-08 &    4.884 & 5.791E-08 &    4.790 \tabularnewline
%                          &  0.010 & 1.486E-09 &    5.187 & 1.691E-09 &    5.098 \tabularnewline
%                          &  0.005 & 4.362E-11 &    5.091 & 5.183E-11 &    5.028 \tabularnewline
% % \multicolumn{6}{c}{} %\tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}
\begin{table}[t]
\caption{A manufactured solution for viscous Burgers equation:
a spatial convergence study is conducted with Lax-Friedrich (LF) flux and
 entropy flux (EF). 
We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
% The error is measured at $t=0.01$ with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.}
}
\tablab{expo-burgers-sconv-mms}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
\hline
\multirow{2}{*}{ } 
  & \multirow{2}{*}{$h$}  
  & \multicolumn{2}{c|}{$LF$}   
  & \multicolumn{2}{c|}{$EF$ ($\sigma=3\times 10^{-4}$)}   
  & \multicolumn{2}{c|}{$EF$ ($\sigma=0$)}   
  \tabularnewline
  &    &  error & order &  error & order &  error & order       \tabularnewline
\hline\hline
\multirow { 4}{*}{   k=1 }&  0.05 & 4.093E-04 &      $-$ & 4.096E-04 &      $-$ & 4.097E-04 &      $-$ \tabularnewline
                         &  0.03 & 1.223E-04 &    1.743 & 1.225E-04 &    1.741 & 1.232E-04 &    1.734 \tabularnewline
                         &  0.01 & 4.494E-05 &    1.445 & 4.378E-05 &    1.484 & 4.620E-05 &    1.415 \tabularnewline
                         &  0.01 & 1.937E-05 &    1.214 & 1.562E-05 &    1.487 & 2.074E-05 &    1.155 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{   k=2 }&  0.05 & 2.630E-06 &      $-$ & 2.632E-06 &      $-$ & 2.632E-06 &      $-$ \tabularnewline
                         &  0.03 & 3.210E-07 &    3.034 & 3.213E-07 &    3.034 & 3.213E-07 &    3.034 \tabularnewline
                         &  0.01 & 3.966E-08 &    3.017 & 3.952E-08 &    3.023 & 3.952E-08 &    3.023 \tabularnewline
                         &  0.01 & 4.916E-09 &    3.012 & 4.833E-09 &    3.032 & 4.833E-09 &    3.032 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=3}&  0.05 & 1.431E-07 &      $-$ & 1.459E-07 &      $-$ & 1.471E-07 &      $-$ \tabularnewline
                         &  0.03 & 1.709E-08 &    3.066 & 1.742E-08 &    3.066 & 1.819E-08 &    3.015 \tabularnewline
                         &  0.01 & 2.003E-09 &    3.093 & 1.876E-09 &    3.215 & 2.268E-09 &    3.003 \tabularnewline
                         &  0.01 & 2.251E-10 &    3.154 & 1.441E-10 &    3.703 & 2.834E-10 &    3.001 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{   k=4}&  0.05 & 5.946E-10 &      $-$ & 5.991E-10 &      $-$ & 6.013E-10 &      $-$ \tabularnewline
                         &  0.03 & 1.827E-11 &    5.024 & 1.837E-11 &    5.027 & 1.860E-11 &    5.015 \tabularnewline
                         &  0.01 & 5.626E-13 &    5.021 & 5.590E-13 &    5.039 & 5.796E-13 &    5.004 \tabularnewline
                         &  0.01 & 1.730E-14 &    5.023 & 1.690E-14 &    5.048 & 1.810E-14 &    5.001 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}
%We test two examples to the viscous Burgers equation in Figure \figref{pde-burgers-ex}. 
%The first example, shown in Figure \figref{pde-burgers-ex}(a), is a smooth Gaussian profile develops sharp gradient as time goes on, $t\in[0,2]$. The initial condition is given as 
%\begin{align}
%    u(x,t) = e^{-2x^2},
%\end{align}
%where $x\in [-1,1]$, $\kappa=0.01$. Periodic boundary condition is imposed. 
We take the following smooth initial condition, 
\begin{align}
  \eqnlab{burgers-smooth}
    u(x,t=0) = \sin^3(2\pi x) (1-x)^{\frac{3}{2}}, %\quad x \in [0,1],
\end{align}
homogeneous boundary condition, and viscosity $\kappa=0.03$.
We perform the simulation for $t \in [0, 1]$ with $k = 4$ solution order and $N_e = 40$ elements.
The smooth initial profile is spread out due to the viscosity as time passes by.
Figure \figref{pde-burgers-smooth} shows the snapshots at $t=1$
for RK2 $(Cr_d=0.16)$ and EPI2 $(Cr_d=161.0, Cr_d=804.9)$. 
% and $t=1$ for RK4 integrator with $Cr=0.32$ and EPI2 integrator with $Cr=319.98$. 
% As can be seen, the smooth initial profile is spread out due to the viscosity.
%and the solutions from both methods  are in good agreement with each other.
Compared to RK2, EPI2 $(Cr_d=161.0)$ uses one-hundred times larger timestep size but
produces a comparable result.
Even with five-hundred times larger timestep size, 
EPI2 $(Cr_d=804.9)$ solution captures the general trend of the evolution.
% \tanbui{again, I think it is much more informative to plot them on the
% same figure. Also, in this kind of comparison, the stability is very
% important to point out for EI. Is $Cr=0.32$ the stability limit for RK4?}

%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[solutions ]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-all}
      \figlab{pde-burgers-ex-smooth-all}
    }
    \subfigure[differences ]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-difference}
      \figlab{pde-burgers-ex-smooth-difference}
    }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{(a) Smooth solutions and (b) their differences with RK4 for viscous Burgers equation at $t=1$.
RK2 with $Cr_d=0.16$, EPI2 with $Cr_d=161.0$ and EPI2 with $Cr_d=804.9$ are used with
$k=4$ solution order and $N_e=40$ elements.
Homogeneous boundary conditions are imposed at $x=0$ and $x=1$.}
%     \caption{A smooth solution to the viscous Burgers equation is simulated for $t \in [0,1]$: 
% (a) RK4 with $Cr=0.32$ and (b) EPI2 with $Cr=321.98$ are used on the grid of $k=4$ and $N_e=40$.
% Homogeneous boundary conditions are imposed at $x=0$ and $x=1$.}
    \figlab{pde-burgers-smooth}
  \end{figure}


To measure the temporal convergence of EPI2 and EXPRB32,
%\footnote{
%EPI3 \cite{tokman2006efficient} is the third-order multi-step method,
%\begin{align}
%  \qb^{n+1} = \qb^n  + \dt \varphi_1(L_d \dt) R^n + \frac{2}{3}\dt \varphi_2 (L_d \dt) D_{n,n-1},
%\end{align}
%where $D_{n,n-1}:= \LRp{R(\qb^{n-1}) - L_d \qb^{n-1}} - \LRp{R(\qb^{n}) - L_d \qb^n}$.
%Since this method requires both $\qb^0$ and $\qb^1$ solutions for advancing in time, 
%we compute $\qb^1$ using EPI2 method, in which the local error is the third-order, 
%so that the global error for EPI3 becomes the third-order accurate. 
%},
we take the RK4 solution (with $dt=5\times 10^{-6}$,  $k=10$, and
$N_e=40$) as a ground truth.
In Table \tabref{expo-burgers-tconv-smooth}, we again observe the second- and third-order convergence rates
for EPI2 and EXPRB32, respectively. 

\begin{table}[t]
\caption{A smooth solution for viscous Burgers equation:
a time convergence study is conducted with $k=4$ solution order and $N_e=40$ elements. 
We observe the second- and the third-order convergence rates for EPI2
and EXPRB32, respectively.}
\tablab{expo-burgers-tconv-smooth}
\begin{center}
%\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
\begin{tabular}{cc||cc|cc}
\hline
\multirow{2}{*}{$dt$} 
& \multirow{2}{*}{$Cr$} 
& \multicolumn{2}{c|}{ EPI2 } 
& \multicolumn{2}{c}{ EXPRB32 } \tabularnewline
  &  &  error & order & error & order \tabularnewline
\hline\hline
  % LF flux
  % 0.50 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  % 0.25 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  % 0.10 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  % 0.05 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.880 \tabularnewline
  % 0.01 &  16.1 &   4.944E-06 &    2.037 &       1.065E-07 &    2.986 \tabularnewline
  % entropy flux
  % 0.5000 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  % 0.2500 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  % 0.1000 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  % 0.0500 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.880 \tabularnewline
  % 0.0100 &  16.1 &   4.944E-06 &    2.037 &       1.068E-07 &    2.983 \tabularnewline  
  % entropy flux with sigma = kappa/100
  0.5000 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  0.2500 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  0.1000 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  0.0500 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.881 \tabularnewline
  0.0100 &  16.1 &   4.943E-06 &    2.037 &       1.042E-07 &    2.999 \tabularnewline  
\hline\hline
\end{tabular}
\end{center}
\end{table} 



%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[solutions]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-all}
      \figlab{pde-burgers-ex-stationary-shock-all}
    }
    \subfigure[differences]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-difference}
      \figlab{pde-burgers-ex-stationary-shock-difference}
    }
    % \subfigure[EPI2 with $Cr=6.71$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
    % }
    % \subfigure[EPI2 with $Cr=13.42$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
    % }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{
    (a) Shock solutions to the viscous Burgers equation at $t=1$, and 
    (b) their differences with RK4.
    EF ($\sigma=10^{-5}$) flux is used for EPI2 and EXPRB32 
    with solution order $k=4$ and $N_e=40$ elements.}
    \figlab{pde-burgers-stationary-shock}
  \end{figure} 

% We have seen that Exponential DG methods work well for the smooth
% solution in \eqnref{burgers-smooth}.
% \tanbui{DG is not useful here if we don't demonstrate correct order of
% convergence in both time and space. So please also show the
% convergence rate for space.}
% \shinhoo{we don't have exact solution for this problem. I will show the spatial convergence in 2D Euler equation}.
Next, we consider a solution with a steep gradient.
A stationary shock evolves in time 
due to the nonlinear convection term \eqnref{pde-burgers-eq}.
The initial condition is given as
\begin{align*}
  u(x,t=0) = \sin(2\pi x)
\end{align*}
for $x \in [0,1]$ with homogeneous boundary conditions.
We take $\kappa=0.001$ and 
 perform the simulation for $t \in [0, 1]$ with $k = 4$ and $N_e = 40$.
 In Figure \figref{pde-burgers-stationary-shock}, 
 we compare EPI2 and EXPRB32 solutions with the RK2 solution.
 We take the RK4 solution 
  (with $dt=1\times 10^{-4}$,  $k=10$, and
$N_e=40$) as a reference, and plot the difference. 
We use EF ($\sigma=10^{-5}$) flux for EPI2 and EXPRB32 and LF flux for RK2 and RK4
% \footnote{
% We numerically observe that the difference between the results with LF and EF fluxes for EPI2 and EXPRB32 is within $\mc{O}(10^{-3})$ in this example, hence omit the EPI2 and EXPRB32 results with LF flux in Figure \figref{pde-burgers-stationary-shock}.  
% }
.

We see that EPI2 $(Cr_d=10.73)$ has an overshoot
% slighly departs from the reference solution 
near the shock interface.
% compared to others.
This is due to the time truncation error associated with the nonlinear convection term. 
To amend this issue,
 we can either shrink a timestep size or employ a high-order time integrator. 
We see that EPI2 $(Cr_d=5.36)$ and EXPRB32 $(Cr_d=10.73)$ become closer to the reference solution near the interface. 
  

% We observe the overshoot near the shock interface for EPI2 $(Cr_d=13.42)$.  
% This is due to the time truncation error associated with the nonlinear convection term. 
% To amend this issue,
%  we can either shrink a timestep size or employ a high-order time integrator. 
% We see that the solutions of EPI2 $(Cr_d=6.71)$ and EXPRB32 $(Cr_d=13.42)$ do not suffer from the overshoot near the interface in Figure \figref{pde-burgers-shock}.

%  %-------------------------
% % EXAMPLES FOR BURGERS EQ.
% %-------------------------
% \begin{figure}[h!t!b!]
%     \centering
% %    \subfigure[Gaussian]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
% %      \figlab{pde-burgers-ex-Gaussian}
% %    }
%     \subfigure[solutions]{
%       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all2}      
%       \figlab{pde-burgers-ex-shock-all}
%     }
%     \subfigure[differences]{
%       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference2}
%       \figlab{pde-burgers-ex-shock-difference}
%     }
%     % \subfigure[EPI2 with $Cr=6.71$]{
%     %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
%     %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
%     % }
%     % \subfigure[EPI2 with $Cr=13.42$]{
%     %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
%     %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
%     % }
% %    \subfigure[Tanh]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
% %      \figlab{pde-burgers-ex-Tanh}
% %    }    
%     %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
%     \caption{
%     (a) Shock solutions to the viscous Burgers equation at $t=2$, and 
%     (b) their differences with RK4.
%     RK2 with $Cr_d=0.13$, EPI2 with $Cr_d=6.71$ and EPI2 with $Cr_d=13.42$
%  are used with solution order $k=4$ and $N_e=40$ elements.}
%     \figlab{pde-burgers-shock}
%   \end{figure} 

%  The initial condition is given as
% \begin{align*}
%   u(x,t=0) = e^{-2x^2}.
% \end{align*}
% We take $\kappa=0.01$ and $x \in [-1,1]$. 
% We perform the simulation for $t \in [0, 2]$ with $k = 4$ and $N_e = 40$.
% Periodic boundary condition is imposed at $x=-1$ and $x=1$. 
% This is a challenging problem because the nonlinear convection term in
% \eqnref{pde-burgers-eq} develops a shock, i.e., solution with a steep gradient.
% %
% %frequently update Jacobian,
% %which eventually prevents a large timestep size.
% %\tanbui{I thought the opposite: updating the Jacobian allows larger
% %  stepsize then keeping it fixed?}
% Figure \figref{pde-burgers-shock} shows the solutions at
%  $t=2$ for RK2 $(Cr_d=0.13)$, EPI2 ($Cr_d=6.71$ and $Cr_d=13.42$) and EXPRB32 ($Cr_d=13.42)$. 
%  %  A shock is developed as it travels with a small dissipation.
%  % \tanbui{putting the figures together in the same plot is
%  %  more informative. Can you get and use a result with RK4 as the
%  %  reference solution to compare with these two solutions?}
% We observe the overshoot near the shock interface for EPI2 $(Cr_d=13.42)$.  
% This is due to the time truncation error associated with the nonlinear convection term. 
% To amend this issue,
%  we can either shrink a timestep size or employ a high-order time integrator. 
% We see that the solutions of EPI2 $(Cr_d=6.71)$ and EXPRB32 $(Cr_d=13.42)$ do not suffer from the overshoot near the interface in Figure \figref{pde-burgers-shock}.
% % Compared to Figure \figref{pde-burgers-shock}a, 
% % Figure \figref{pde-burgers-shock}b shows the overshoot near the shock
% % interface. 
% % To amend this issue, we may employ various techniques such as strong-stability preserving (SSP) methods \cite{gottlieb2005high} and non-oscillatory schemes \cite{gottlieb2006recovering}. However, since it needs a comprehensive investigation, 
% % we will pose the issue in future work. 
% %However, it is not clear how to determine the update frequency for the Jacobian.
% %As an alternative, we may employ strong-stability preserving (SSP) type method \cite{gottlieb2005high} 
% %or reconstruction \cite{gottlieb2006recovering}, but thorough investigation is needed. 
% %We will tackle this issue in future work. 
% %

 
%EPI2 time integrators with 
%As shown in Figure \figref{pde-burgers-ex}(b),
%$\tanh$ shape is translated from left to right. 
%The exact solution is given as 
%\begin{align}
%    u(x,t) = 1 -\tanh \LRp{\frac{x+0.5-t}{2\kappa}}.
%\end{align}
%We impose exact boundary condition at both the ends. 

We also perform the same simulations above for EPI2 and EXPRB32 with Lax-Friedrich flux.
The results are summarized in Figure \figref{pde-burgers-fluxdifference}.
The differences between the results with Lax-Friedrich and entropy fluxes are 
orders of $\mc{O}(10^{-8})$ for the smooth solution case and $\mc{O}(10^{-3})$ for the shock solution case.
Considering these small differences between two fluxes %that these differences are not significant and 
and the simplicity of Lax-Friedrich flux, we use Lax-Friedrich flux for Euler equations 
in the following examples.

%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[smooth case]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-difference-flux-difference}      
      \figlab{pde-burgers-ex-smooth-fluxdiff}
    }
    \subfigure[shock case]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-flux-difference}
      \figlab{pde-burgers-ex-sShock-fluxdiff}
    }
    % \subfigure[EPI2 with $Cr=6.71$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
    % }
    % \subfigure[EPI2 with $Cr=13.42$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
    % }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{
    The differences between the results with Lax-Friedrich flux and with entropy flux are plotted: (a) the smooth solution case in Figure \figref{pde-burgers-smooth} and 
    (b) the shock solution case in Figure \figref{pde-burgers-stationary-shock}.
    }
    \figlab{pde-burgers-fluxdifference}
\end{figure} 






\subsection{Euler equations: Isentropic vortex translation}

We study the isentropic vortex example \cite{zhou2003high}, 
where small perturbations of a vortex are added to the uniform mean flow 
and translated without changing its shape. 
The superposed flow is given as 
\begin{align*}
u &= u_\infty - \frac{\lambda}{2\pi} \tilde{y} e^{\alpha \LRp{1-r^2}/2}, \\
v & = v_\infty + \frac{\lambda}{2\pi}\tilde{x} e^{\alpha\LRp{1-r^2}/2}, \\
T & = T_\infty - \LRp{\frac{1}{2\alpha c_p} } \LRp{\frac{\lambda}{2\pi}}^2 e^{\alpha\LRp{1-r^2}},
% T & = T_\infty - T_\infty\LRp{\frac{\gamma-1}{2\alpha a_\infty^2} } \LRp{\frac{\lambda}{2\pi}}^2 e^{\alpha\LRp{1-r^2}},
\end{align*}
where $r = \norm{\xb - \xb_c - \ub_\infty t}$,
$\tilde{x}=x - x_c - u_\infty t$,
$\tilde{y}=y - y_c - v_\infty t$,
$\ub_\infty=(u_\infty,v_\infty)$ the velocity of the mean flow,
$\xb_c=(5,0)$, $c_p$ specific heat ratio at constant pressure 
and $\lambda$ the vortex strength. 
The mean flows are set to be $(u_\infty,v_\infty,\rho_\infty,T_\infty,\pres_\infty) = (0.2,0,1,1,1)$.
We take $\alpha=2$, $\gamma=1.4$, $\lambda=0.05$ and 
$c_p=\frac{\gamma}{\gamma-1}$.
% and the perturbations are given as 
% \begin{align*}
% u^\prime & = - \frac{\lambda}{2\pi} e^{\LRp{1-r^2}}(y - y_c), \\
% v^\prime & = + \frac{\lambda}{2\pi} e^{\LRp{1-r^2}}(x - x_c), \\
% T^\prime & = - \frac{\LRp{\gamma - 1}\lambda^2}{16\gamma\pi^2} e^{2\LRp{1-r^2}}
% \end{align*}
The exact solutions are generated from the isentropic relation\footnote{
$$\frac{\rho}{\rho_\infty} = \LRp{\frac{T}{T_\infty}}^{\frac{1}{\gamma-1}}
=\LRp{\frac{\pres}{\pres_\infty}}^{\frac{1}{\gamma}}
$$
}. 
%$$ \rho = \LRp{T_\infty + T^\prime}^{1/(\gamma-1)}. $$
%We take $\gamma=1.4$ and 
The domain is $\Omega = \LRp{0,10} \times \LRp{-5,5}$ and 
periodic boundary conditions are applied to all directions. 
For a three-dimensional simulation, we take the zero vertical velocity, $w = 0$ and extrude domain vertically, $\Omega = \LRp{0,10} \times \LRp{-5,5} \times \LRp{0,1}$. 

We perform the simulation for $t\in [0,15]$ 
with $k=12$ and $N_e=256$ in Figure \figref{expo-pde-euler2d-vortex}.
We increase the timestep size of EPI2 until it shows a notable time truncation error. 
Compared to the EPI2 $(Cr=42.75)$ solution in the left panel, 
the EPI2 $(Cr=85.56)$ solution in the center panel 
shows the oscillatory solution in the mean flows,
 which starts from the edge of the vortex and propagates the entire domain.
 Due to the hyperbolic nature of the Euler system, 
 the oscillation remains throughout the simulation, 
 but the shape of the vortex and its movement are still comparable to 
 the one with EPI2 $(Cr=42.75)$.
To alleviate the oscillation, we can employ a high-order time integrator.
For example, the third-order EXPRB32 $(Cr=85.56)$ in the right panel significantly improves the solution accuracy in Figure \figref{expo-pde-euler2d-vortex}.
% This is 
% EPI2 and EXPRB42 can use one-hundred times larger timestep size than RK4, 
% and still capture the vortex movement. 
% However, the solution of EPI2 degrades
% \tanbui{perhaps we should make the statement more precise. I see that
%   the solution is osillatory, though the magnitude is similar. Is this
% what you meant by ``degrade''?}
% due to the time truncation error. % in Figure \figref{expo-pde-euler2d-vortex}(b). %The artificial 

% For time discretization, 
% RK4 with $Cr=0.86$, 
% %EPI2 with $Cr=8.56$ and 
% EPI2 with $Cr=85.56$ and 
% EXPRB42 \cite{hochbruck2010exponential} with $Cr=85.56$
% \tanbui{a few words, put it in parentheses or footnote,introducing EXPRB42 are necessary here}
% are chosen. 
% As can be seen in Figure \figref{expo-pde-euler2d-vortex}(b) 
% and Figure \figref{expo-pde-euler2d-vortex}(c), 
% EPI2 and EXPRB42 can use one-hundred times larger timestep size than RK4, 
% and still capture the vortex movement. 
% However, the solution of EPI2 degrades
% \tanbui{perhaps we should make the statement more precise. I see that
%   the solution is osillatory, though the magnitude is similar. Is this
% what you meant by ``degrade''?}
% due to the time truncation error. % in Figure \figref{expo-pde-euler2d-vortex}(b). %The artificial oscillation is caused by the time truncation error for EPI2.
%This is a consequence of the time trunction error. 
%Since Euler system is nonlinear, exponential integrators are not free from the time truncation error.  
%the 
%have the time truncation error. This is why we observe the oscillation in Figure \figref{expo-pde-euler2d-vortex}(b). However, the time truncation error is significantly reduced 
% To alleviate the error, we can use a high-order time integration method.
% For example, in Figure \figref{expo-pde-euler2d-vortex}(c), 
% the time truncation error of EXPRB42
% \tanbui{what is the order of EXPRB42? what if we use smaller Cr
%   (i.e. do we still see the similar degrade)? Perhaps providing
%   solution with different Cr's (similar to our IMEX paper) is
%   informative and provides a more complete picture of the behavior of
%   the EPI2 method. It is also weird that EXPRB42 comes out of
%   blue. You introduced EPI3 before, why not using it here? As a
%   reader/reviewer, I would raise a lot concerns about this
%   inconsistency of the manuscript.}
% is significantly reduced compared to the EPI2 counterpart. 


%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
\centering
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t5}
  % \figlab{pde-euler2d-epi2-Cr42-t5}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t5} 
  % \figlab{pde-euler2d-epi2-Cr85-t5}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t5}
   % \figlab{pde-euler2d-exprb32-Cr85-t5}
   \\
% }\\
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t10}
  % \figlab{pde-euler2d-epi2-Cr42-t10}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t10} 
  % \figlab{pde-euler2d-epi2-Cr85-t10}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t10}
   % \figlab{pde-euler2d-exprb32-Cr85-t10}
   \\
% }\\
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t15}
  % \figlab{pde-euler2d-epi2-Cr42-t15}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t15} 
  % \figlab{pde-euler2d-epi2-Cr85-t15}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t15}
   % \figlab{pde-euler2d-exprb32-Cr85-t15}
% }
% \subfigure[RK4 with $Cr=0.86$]{
%   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-rk4}
%   \figlab{pde-euler2d-rk4}
% }
% %\subfigure[EPI2 with $Cr=8.56$]{
% %  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-epi2-10x} 
% % % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-10x} 
% %  \figlab{pde-euler2d-epi2-10x}
% %}
% \subfigure[EPI2 with $Cr=85.56$]{
%   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-epi2-100x} 
%   %\includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-100x} 
%   \figlab{pde-euler2d-epi2-100x}
% }    
% \subfigure[{\tiny EXPRB42} with $Cr=85.56$]{
%    \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-100x}
%    \figlab{pde-euler2d-exprb42-100x}
% }
\caption{Isentropic vortex example to the two-dimensional Euler equations: 
translating density fields for EPI2 ($Cr=42.75$, left), EPI2 ($Cr=85.56$, center) and EXPRB32 ($Cr=85.56$, right) at times $t=5$ (top), $t=10$ (middle) and $t=15$ (bottom).}
\figlab{expo-pde-euler2d-vortex}
\end{figure}



%\begin{table}[t]
%\caption{Isentropic vortex in two-dimensions: 
%time convergence study is conducted with $k=16$ solution order and $N_e=256$ elements. We observe the second-order convergence rate for EPI2 as expected.}
%\tablab{expo-euler2d-tconv-isentropic}
%\begin{center}
%\begin{tabular}{*{1}{c}||c|cc|cc|cc|c}
%\hline
%    & $Cr$ 
%& {\small $ \norm{\rho - \rho^e}_2$} & rate
%& {\small $ \norm{\rho {\bf u} - \rho \ub^e}_2$} & rate 
%& {\small $\small \norm{\rho E - \rho E^e}_2 $} & rate &  wc $[s]$ \tabularnewline
%\hline\hline
%\multirow { 6}{*}{  {\small EPI2} }& 71.4 & 2.89E-07 &        - & 6.18E-07 &        - & 1.02E-06 &        - &     75.4 \tabularnewline
%                         & 35.7 & 8.75E-08 &    1.73 & 1.26E-07 &    2.30 & 3.08E-07 &    1.73 &     43.9 \tabularnewline
%                         & 14.3 & 1.52E-08 &    1.91 & 1.82E-08 &    2.11 & 5.34E-08 &    1.91 &     37.0 \tabularnewline
%                         &  7.1 & 3.88E-09 &    1.97 & 4.43E-09 &    2.04 & 1.37E-08 &    1.97 &     38.8 \tabularnewline
%                         &  1.4 & 1.58E-10 &    1.99 & 1.74E-10 &    2.01 & 5.57E-10 &    1.99 &    108.1 \tabularnewline
%                         &  0.7 & 3.96E-11 &    2.00 & 4.33E-11 &    2.00 & 1.40E-10 &    2.00 &    230.8 \tabularnewline
%\multicolumn{9}{c}{} \tabularnewline
%\multirow { 2}{*}{   { \small RK4} }&  0.7 & 1.44E-13 &        - & 1.24E-12 &        - & 6.26E-14 &        - &     35.5 \tabularnewline
%                         &  0.4 & 1.53E-13 &   -0.10 & 1.24E-12 &    0.00 & 7.77E-14 &   -0.31 &     78.1 \tabularnewline
%\hline\hline
%\end{tabular}
%\end{center}
%\end{table}



To examine the error growth rate, 
time convergence studies are conducted with $k=\LRc{8,16}$ for $t\in[0,1]$ on a uniform mesh and a non-uniform mesh in Figure \figref{expo-pde-euler2d-mesh}.
%Here, we take the Krylov subspace size $m$ from the previous time step as a first guess for the adaptive Krylov subspace method \cite{gaudreault2018kiops} at the current time step. 
To verify the high-order accuracy in time, 
we take the second, the third, and the fourth-order exponential integrators:
EPI2, EXPRB32, and EXPRB42
\footnote{
EXPRB42  \cite{luan2017fourth} is the fourth-order two-stage method,
\begin{align*}
  q^{(2)} &= q^n + \frac{3}{4} \dt \varphi_1 \LRp{ \frac{3}{4} L \dt } R^n,\\
  q^{n+1} &= q^n + \dt \varphi_1(L \dt) R^n
                 + \frac{32}{9} \dt \varphi_3 \LRp{ L \dt } D_{n,2},
  %q^{n+1} = q^n  + \dt \varphi_1(L \dt) R^n + \frac{2}{3}\dt \varphi_2 (L \dt) D_{n,2},
\end{align*}
where $D_{n,2}:= \LRp{R(q^{(2)}) - L q^{(2)}} - \LRp{R(q^{n}) - L q^n}$.
}
.
We compare Exponential DG methods with IMEX DG and RKDG \cite{shu1988total} methods. 
In particular, we take the second-order, ARS232 \cite{ascher1997implicit} and the third-order, ARS443 \cite{ascher1997implicit} schemes without any preconditioner. 
The results for $\rho$ on a uniform mesh are summarized in 
Figure \figref{expo-euler-isentropic-tconv-uni-p16} 
and Figure \figref{expo-euler-isentropic-tconv-uni-p8}.
% Also, we do not consider the fourth-order IMEX methods because 
% the second and the third order IMEX schemes  
% have already shown its relative performance 

In Figure \figref{expo-euler-isentropic-tconv-uni-p16}(a),
 we observe 
 that the RK2 solution converges to the true solution with the second-order accuracy, 
 and the high-order RK (RK3 and RK4) solutions have reached the saturated error level at 
 $\mc{O}(10^{-13})$, 
 where the spatial discretization error starts to dominate.
We also see that Exponential DG (EPI2, EXPRB32, EXPRB42) and IMEX DG (ARS232 and ARS443) methods show the theoretical convergence rates for a wide range of time stepsizes. %Courant number. % This is a very
                                %attractive feature compared to the
                                %IMEX scheme.
This is attractive because that Exponential DG and IMEX DG supports a high-order solution in time, 
and overcomes the timestep size restriction 
the explicit RKDG methods suffer from. 
% \tanbui{You put the RK4 results there and you have to explain why. You
% can not let the readers to read the figure by themselves. For example,
% you can talk about why you have only two points for RK4 in Figure
% \figref{expo-euler-isentropic-tconv-uni-p16}(a). You need to label the
% numbers (I think they are Courant numbers, on the top of the figure. Also, some mutual
% comparison among RK4, EPI2, and EXPRB42 need to be spelled out. In
% particular, you need to really tell one should do EPI instead of
% RK: if you were a reader, why should you care about EPI?}

In Figure \figref{expo-euler-isentropic-tconv-uni-p16}(b), 
we see that the high-order EXPRB32 and EXPRB42 schemes are beneficial compared to
the second-order EPI2 below $\mc{O}(10^{-10})$ error level,
 but the second-order EPI2 become two times faster than EXPRB32 and EXPRB42 
 above $\mc{O}(10^{-8})$ error level. 
 Both EXPRB32 and EXPRB42 require two-stage matrix exponential evaluations, 
 hence, their wallclock times are similar. 
 However, due to the high-order accuracy, EXPRB42 is slightly more efficient than EXPRB32.
 Compared to IMEX DG, EPI2 and EXPRB32 are more economical than ARS232 and ARS443. 
 EPI2 is four times faster than ARS232, and 
 EXPRB32 is ten times faster than ARS443 at $\mc{O}(10^{-8})$ error level.
 Compared to explicit RKDG, EXPRB42 becomes comparable to RK2 near $\mc{O}(10^{-11})$ error level but
 is slightly slower than RK3 and RK4 at $\mc{O}(10^{-13})$ error level.
 Note that we use a smooth solution for convergence study. 
 In practice, $\mc{O}(10^{-13})$ error level is hard to be attainable when involving a non-smooth solution, heterogeneous materials and so on. 
% tanbui{beneficial in which sense, even me I have to decode the figure
%   to see why EXPRB42 is more beneficial? You have to spell it out.}
% However, we
% still see that RK4 DG is more economical than Exponential DG methods
% at $\mc{O}(10^{-13})$ error level.
% \tanbui{Again, why are there only two points for RK4 at a very low
%   error levels? saying RK is more advantage at
%   $10^{-13}$ is not actually  useful because one typically does not go down that
% far. Can we compare the methods in terms of accuracy and wall-clock time, at the same time stepsizes?}
%This shows that an exponential time integrator captures the fast modes in the system more accurately 
%than the IMEX method. The wall clock time of EPI2 drops sharply until Courant number reaches 7 and grows after 7. There is a sweet spot near $Cr=1.43$, of which the wall clock time of EPI2 is comparable to that of RK4. In general, the computational cost is more expensive than RK4, but there are tune parameters in the algorithm \cite{gaudreault2018kiops}. Here, we use the parameters of \texttt{tol}=$10^{-10}$, \texttt{mmin}=10, \texttt{mmax}=128 and \texttt{orth$\_$len}=100.
%The results are tabulated in \tabref{expo-euler2d-tconv-isentropic}. 

%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
\centering
\subfigure[Uniform mesh]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-msh-uniform}
  \figlab{pde-euler2d-mesh-uniform}
}
\subfigure[Non-uniform mesh]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-msh-nonuniform} 
 % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-10x} 
  \figlab{pde-euler2d-mesh-nonuniform}
}
\caption{(a) Uniform mesh with $N_e=256$ elements and (b) non-uniform meshes with $N_e=250$ elements.}
\figlab{expo-pde-euler2d-mesh}
\end{figure}





% %---------------------
% % TIME CONVERGENCE - uniform - N16
% %---------------------
% \begin{figure}[h!t!b!]
%     \centering
%     \subfigure[Accuracy]{
%             \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N16-r}
%       \figlab{expo-euler-isentropic-tconv-uni-p16-accuracy}
%     }
%     \subfigure[Efficiency]{
%      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.413\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N16-wc}
%       \figlab{expo-euler-isentropic-tconv-uni-p16-efficiency}
%     }
%   \caption{Isentropic vortex translation in two dimensions:
%     time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
%         The computational domain is discretized with $N_e = 256$ and $k=16$. }
%   \figlab{expo-euler-isentropic-tconv-uni-p16}
% \end{figure}


%---------------------
% TIME CONVERGENCE - uniform - N16
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N16-r}
      \figlab{expo-euler-isentropic-tconv-uni-p16-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.413\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N16-wc}
      \figlab{expo-euler-isentropic-tconv-uni-p16-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=16$. }
  \figlab{expo-euler-isentropic-tconv-uni-p16}
\end{figure}


% %---------------------
% % TIME CONVERGENCE - uniform, N8
% %---------------------
% \begin{figure}[h!t!b!]
%     \centering
%     \subfigure[Accuracy]{
%             \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N8-r}
%       \figlab{expo-euler-isentropic-tconv-uni-p8-accuracy}
%     }
%     \subfigure[Efficiency]{
%      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N8-wc}
%       \figlab{expo-euler-isentropic-tconv-uni-p8-efficiency}
%     }
%   \caption{Isentropic vortex translation in two dimensions:
%     time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
%         The computational domain is discretized with $N_e = 256$ and $k=8$. }
%   \figlab{expo-euler-isentropic-tconv-uni-p8}
% \end{figure}


%---------------------
% TIME CONVERGENCE - Uniform, N8
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N8-r}
      \figlab{expo-euler-isentropic-tconv-uni-p8-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N8-wc}
      \figlab{expo-euler-isentropic-tconv-uni-p8-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=8$. }
  \figlab{expo-euler-isentropic-tconv-uni-p8}
\end{figure}

To mimic such a situation, we increase a spatial discretization error by lowering the polynomial order from $k=16$ to $k=8$ so that the saturation error level rises in Figure \figref{expo-euler-isentropic-tconv-uni-p8}. 
We omit the results of RK2 and RK3 in Figure \figref{expo-euler-isentropic-tconv-uni-p8}
because the errors of RK2, RK3, and RK4 are almost the same, 
but the wallclock time of RK4 is faster than those of RK2 and RK3
in Table \tabref{expo-euler-isentropic-tconv-uni-p8}.
%the errors are saturated at $\mc{O}(10^{-8})$ error level, 
In this case, the wallclock time of EPI2 becomes comparable to that of RK4
and slightly shorter than RK2.
At $\mc{O}(10^{-8})$ error level, EPI2 is two times faster than EXPRB32 and EXPRB42, 
five times faster than ARS232, and seventeen times faster than ARS443. 

% \tanbui{I don't know why we have EPI2 there because it is not
%   fourth-order accuracy as RK4. I think we should focus on EXPRB4
%   verus RK4 because they are compatible. You can do EPI2 verus RK2. I
%   think the appealing messages from these two figures are: 1) EXPRB4
% is more robust (not stability issues) with time steps, 2) EXPRB4 can
% attain the same accuracy with higher CFL numbers compared to RK4, 3)
% EXPRB4 has similar/same wall-clock time as RK4 at the same accuracy
% level. You can add more positive points here.}
% \shinhoo{In this case for $k=8$ on uniform mesh, 
% the saturation error level is at $\mc{O}(10^{-8})$. 
% The best performed methods for RKDG, Exponential DG and IMEX DG are
% RK4, EPI2 and ARS232.
% Thus it seems to be reasonable to compare EPI2 and RK4. }

%---------------------
% TEMPORAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in two dimensions:
    time convergence study on a uniform mesh.
    The computational domain is discretized with $N_e = 256$ and $k=8$.
    The error is measured at $T=1$. 
}
\tablab{expo-euler-isentropic-tconv-uni-p8}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
\hline
\multirow{2}{*}{$k=8$} 
  & \multirow{2}{*}{$Cr$}  
  % & \multirow{2}{*}{$dt$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  & \multirow{2}{*}{wc $[s]$}    \tabularnewline
  &       &  error & order &  error & order &  error & order &     \tabularnewline
\hline\hline
\multirow { 2}{*}{   RK2 }&  0.30   & 5.445E-08 &        - & 4.050E-08 &        - & 1.255E-08 &        - &     17.3 \tabularnewline
                         &  0.15   & 5.445E-08 &    0.000 & 3.942E-08 &    0.039 & 1.245E-08 &    0.012 &     37.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK3 }&  0.60   & 5.444E-08 &        - & 3.936E-08 &        - & 1.235E-08 &        - &     14.3 \tabularnewline
                         &  0.30   & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.242E-08 &   -0.008 &     24.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK4 }&  0.90   & 5.444E-08 &        - & 3.936E-08 &        - & 1.242E-08 &        - &     12.4 \tabularnewline
                         &  0.45   & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.001 &     24.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{  EPI2 }& 43.09   & 2.585E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &     14.1 \tabularnewline
                         & 21.54   & 5.097E-07 &    2.342 & 6.532E-07 &    2.364 & 1.790E-06 &    2.341 &     13.4 \tabularnewline
                         &  4.31   & 5.746E-08 &    1.356 & 4.642E-08 &    1.643 & 7.256E-08 &    1.992 &     13.5 \tabularnewline
                         % &  2.15 &  0.05 & 5.450E-08 &    0.076 & 3.986E-08 &    0.220 & 2.174E-08 &    1.739 &     23.9 \tabularnewline
                         % &  0.86 &  0.02 & 5.442E-08 &    0.002 & 3.938E-08 &    0.013 & 1.274E-08 &    0.583 &     65.4 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &   -0.001 & 3.936E-08 &    0.001 & 1.244E-08 &    0.034 &    109.4 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{EXPRB32} }& 43.09   & 1.869E-07 &        - & 1.667E-07 &        - & 6.295E-07 &        - &     28.6 \tabularnewline
                         & 21.54   & 5.556E-08 &    1.750 & 4.242E-08 &    1.974 & 4.184E-08 &    3.911 &     23.4 \tabularnewline
                         &  4.31   & 5.444E-08 &    0.013 & 3.936E-08 &    0.047 & 1.242E-08 &    0.755 &     25.7 \tabularnewline
                         % &  2.15 &  0.05 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.001 &     46.7 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    117.9 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    235.0 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{EXPRB42} }& 43.09   & 9.257E-08 &        - & 2.267E-07 &        - & 2.660E-07 &        - &     22.9 \tabularnewline
                         & 21.54   & 5.476E-08 &    0.757 & 3.982E-08 &    2.509 & 1.911E-08 &    3.799 &     21.4 \tabularnewline
                         &  4.31   & 5.444E-08 &    0.004 & 3.936E-08 &    0.007 & 1.241E-08 &    0.268 &     25.0 \tabularnewline
                         % &  2.15 &  0.05 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.002 &     46.8 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    121.1 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    234.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{ARS232 }}& 43.09   & 1.522E-06 &        - & 4.685E-05 &        - & 6.383E-06 &        - &    156.8 \tabularnewline
                         & 21.54   & 1.764E-07 &    3.109 & 1.193E-05 &    1.973 & 1.027E-06 &    2.636 &     94.2 \tabularnewline
                         &  4.31   & 5.439E-08 &    0.731 & 4.820E-07 &    1.994 & 3.801E-08 &    2.048 &     69.7 \tabularnewline
                         &  2.15   & 5.441E-08 &   -0.001 & 1.265E-07 &    1.930 & 1.486E-08 &    1.355 &     86.2 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &   -0.001 & 4.387E-08 &    1.156 & 1.239E-08 &    0.198 &    154.1 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.967E-08 &    0.145 & 1.240E-08 &   -0.001 &    270.8 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{ARS443 }}& 43.09   & 7.193E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &    850.8 \tabularnewline
                         & 21.54   & 1.541E-07 &    2.223 & 1.822E-06 &    2.938 & 5.063E-07 &    2.358 &    478.8 \tabularnewline
                         &  4.31   & 5.435E-08 &    0.648 & 4.204E-08 &    2.342 & 1.181E-08 &    2.335 &    234.2 \tabularnewline
                         &  2.15   & 5.441E-08 &   -0.002 & 3.938E-08 &    0.094 & 1.149E-08 &    0.040 &    244.4 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &   -0.001 & 3.936E-08 &    0.001 & 1.230E-08 &   -0.074 &    334.8 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.241E-08 &   -0.013 &    556.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}

 

On the non-uniform mesh, 
we observe that the convergence rates for 
EPI2, EXPRB32, EXPRB42, ARS232, and ARS443 agree to the theoretical convergence rates for a wide range of Courant numbers Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(a).
In Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(b), we compare the efficiency of Exponential DG methods to those of others. 
EPI2 is three times faster than ARS232 at $\mc{O}(10^{-10})$ error level. 
EXPRB32 is five times faster than ARS443 at $\mc{O}(10^{-12})$ error level.
EPI2 is almost two times faster than EXPRB32 and EXPRB42 above $\mc{O}(10^{-10})$ error level. 
However, as tighten the error level, the high-order EXPRB32 and EXPRB42 become more economical than EPI2.
Compared to explicit RK methods, 
at $\mc{O}(10^{-13})$ error level, EXPRB32 is comparable to RK2, RK3 and RK4 methods in terms of accuracy and efficiency. 
EXPRB42 shows slightly better performance than EXPRB32, RK2, RK3 and RK4 methods.
%  we observe that
% the similar temporal convergence results in Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(a).
% and \figref{expo-euler-isentropic-tconv-nonuni-p8}.
% We 
% we start to see the benefit of Exponential DG schemes. 
% In (b),
% the wall clock time of EXPRB42 becomes comparable to RK4 at $\mc{O}(10^{-12})$ error level.
Next, we add a spatial discretization error by lowering the solution order from $k=16$ to $k=8$. 
We see the computational gain of Exponential DG methods in Figure \figref{expo-euler-isentropic-tconv-nonuni-p8}(b) and Table 
\tabref{expo-euler-isentropic-tconv-nonuni-p8}.
At $\mc{O}(10^{-9})$ error level, 
the wallclock times of RK2, RK3 and RK4 are $188.2$, $107.6$ and $116.2$.
EPI2 is three times faster than RK2, and 
two times faster than RK3 and RK4. 
EPI2 is four times faster than ARS232. 
EXPRB32 is six times faster than ARS443. 

% \tanbui{see my above comments. Again, I think we should focus on RK4
%   verus EXPRB4. I think you can say similar thing for RK2 versus RK4,
%   that is RK2 can get similary accuracy with better wallclock time?}


%---------------------
% TIME CONVERGENCE non-uniform, N16
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N16-r}
      \figlab{expo-euler-isentropic-tconv-p16-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N16-wc}
      \figlab{expo-euler-isentropic-tconv-p16-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on non-uniform mesh.
        The computational domain is discretized with $N_e = 250$ and $k=16$. }
  \figlab{expo-euler-isentropic-tconv-nonuni-p16}
\end{figure}




%---------------------
% TIME CONVERGENCE - nonuniform, N8
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.44\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N8-r}
      \figlab{expo-euler-isentropic-tconv-p8-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N8-wc}
      \figlab{expo-euler-isentropic-tconv-p8-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a non-uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=8$. }
  \figlab{expo-euler-isentropic-tconv-nonuni-p8}
\end{figure}





% %---------------------
% % TEMPORAL CONVERGENCE k=16 on nonuniform mesh
% %---------------------
% \begin{table}[t]
% \caption{Isentropic vortex translation in two dimensions:
%     time convergence study on a nonuniform mesh.
%     The computational domain is discretized with $N_e = 256$ and $k=16$.
%     The error is measured at $T=1$. 
% }
% \tablab{expo-euler-isentropic-tconv-nonuni-p16}
% \begin{center}
% \begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
% \hline
% \multirow{2}{*}{$k=16$} 
%   & \multirow{2}{*}{$dt$}  
%   & \multirow{2}{*}{$Cr$}  
%   & \multicolumn{2}{c|}{$\rho$}   
%   & \multicolumn{2}{c|}{$\rho {\bf u}$}   
%   & \multicolumn{2}{c|}{$\rho E$}   
%   & \multirow{2}{*}{wc $[s]$}    \tabularnewline
%   &    &   &  error & order &  error & order &  error & order &     \tabularnewline
% \hline\hline
% \multirow { 2}{*}{   RK2 }&  0.30 &  0.00 & 5.339E-13 &        - & 8.416E-12 &        - & 8.095E-13 &        - &   1001.9 \tabularnewline
%                          &  0.15 &  0.00 & 9.172E-13 &   -0.781 & 3.474E-12 &    1.277 & 7.404E-13 &    0.129 &   2017.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 2}{*}{   RK3 }&  0.60 &  0.00 & 3.081E-13 &        - & 2.833E-12 &        - & 2.037E-13 &        - &    703.1 \tabularnewline
%                          &  0.30 &  0.00 & 5.085E-13 &   -0.723 & 2.837E-12 &   -0.002 & 3.759E-13 &   -0.884 &   1375.5 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 2}{*}{   RK4 }&  0.90 &  0.00 & 4.578E-13 &        - & 2.837E-12 &        - & 4.165E-13 &        - &    778.3 \tabularnewline
%                          &  0.45 &  0.00 & 8.476E-13 &   -0.889 & 2.860E-12 &   -0.012 & 8.353E-13 &   -1.004 &   1579.9 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{  EPI2 }& 1497.94 &  1.00 & 2.583E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &    314.2 \tabularnewline
%                          & 748.97 &  0.50 & 5.085E-07 &    2.345 & 6.518E-07 &    2.367 & 1.790E-06 &    2.341 &    318.0 \tabularnewline
%                          & 149.79 &  0.10 & 2.031E-08 &    2.001 & 2.437E-08 &    2.042 & 7.154E-08 &    2.001 &    307.9 \tabularnewline
%                          & 74.90 &  0.05 & 5.079E-09 &    2.000 & 6.079E-09 &    2.003 & 1.789E-08 &    2.000 &    306.5 \tabularnewline
%                          & 29.96 &  0.02 & 8.087E-10 &    2.005 & 1.033E-09 &    1.934 & 2.849E-09 &    2.005 &    309.2 \tabularnewline
%                          & 14.98 &  0.01 & 1.933E-10 &    2.065 & 6.806E-10 &    0.602 & 6.844E-10 &    2.058 &    333.1 \tabularnewline
%                          &  7.49 &  0.01 & 5.086E-11 &    1.926 & 6.075E-11 &    3.486 & 1.792E-10 &    1.933 &    451.8 \tabularnewline
%                          &  3.00 &  0.00 & 8.142E-12 &    1.999 & 1.011E-11 &    1.957 & 2.867E-11 &    2.000 &   1127.4 \tabularnewline
%                          &  1.50 &  0.00 & 2.048E-12 &    1.991 & 3.730E-12 &    1.439 & 7.169E-12 &    2.000 &   2196.0 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ EXPRB32 }& 1497.94 &  1.00 & 1.807E-07 &        - & 1.608E-07 &        - & 6.291E-07 &        - &    658.2 \tabularnewline
%                          & 748.97 &  0.50 & 1.125E-08 &    4.006 & 1.562E-08 &    3.364 & 3.957E-08 &    3.991 &    691.8 \tabularnewline
%                          & 149.79 &  0.10 & 7.677E-11 &    3.099 & 1.186E-10 &    3.032 & 2.707E-10 &    3.097 &    682.5 \tabularnewline
%                          & 74.90 &  0.05 & 9.519E-12 &    3.012 & 1.516E-11 &    2.968 & 3.355E-11 &    3.012 &    697.9 \tabularnewline
%                          & 29.96 &  0.02 & 6.435E-13 &    2.940 & 3.122E-12 &    1.725 & 2.156E-12 &    2.996 &    699.9 \tabularnewline
%                          & 14.98 &  0.01 & 2.173E-13 &    1.566 & 3.139E-12 &   -0.008 & 3.400E-13 &    2.665 &    747.2 \tabularnewline
%                          &  7.49 &  0.01 & 1.980E-13 &    0.134 & 2.831E-12 &    0.149 & 9.341E-14 &    1.864 &    925.7 \tabularnewline
%                          &  3.00 &  0.00 & 2.034E-13 &   -0.029 & 2.831E-12 &    0.000 & 9.202E-14 &    0.016 &   2320.2 \tabularnewline
%                          &  1.50 &  0.00 & 2.182E-13 &   -0.101 & 2.831E-12 &    0.000 & 1.118E-13 &   -0.281 &   4569.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 6}{*}{ EXPRB42 }& 1497.94 &  1.00 & 7.521E-08 &        - & 2.216E-07 &        - & 2.652E-07 &        - &    569.9 \tabularnewline
%                          & 748.97 &  0.50 & 4.273E-09 &    4.138 & 4.914E-09 &    5.495 & 1.518E-08 &    4.127 &    557.5 \tabularnewline
%                          & 149.79 &  0.10 & 4.552E-12 &    4.253 & 7.129E-12 &    4.061 & 1.628E-11 &    4.249 &    570.7 \tabularnewline
%                          & 74.90 &  0.05 & 3.442E-13 &    3.725 & 2.984E-12 &    1.256 & 1.010E-12 &    4.011 &    576.4 \tabularnewline
%                          & 29.96 &  0.02 & 1.977E-13 &    0.605 & 2.956E-12 &    0.010 & 1.110E-13 &    2.410 &    586.0 \tabularnewline
%                          & 14.98 &  0.01 & 1.977E-13 &    0.000 & 3.141E-12 &   -0.088 & 1.418E-13 &   -0.353 &    616.5 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ ARS232P }& 1497.94 &  1.00 & 1.521E-06 &        - & 4.685E-05 &        - & 6.384E-06 &        - &  15105.5 \tabularnewline
%                          & 748.97 &  0.50 & 1.714E-07 &    3.150 & 1.193E-05 &    1.973 & 1.028E-06 &    2.635 &  12694.5 \tabularnewline
%                          & 149.79 &  0.10 & 4.126E-09 &    2.316 & 4.803E-07 &    1.996 & 3.718E-08 &    2.063 &   2196.1 \tabularnewline
%                          & 74.90 &  0.05 & 1.003E-09 &    2.040 & 1.201E-07 &    2.000 & 9.267E-09 &    2.004 &   1407.4 \tabularnewline
%                          & 29.96 &  0.02 & 1.589E-10 &    2.011 & 1.922E-08 &    2.000 & 1.481E-09 &    2.001 &   1179.5 \tabularnewline
%                          & 14.98 &  0.01 & 3.964E-11 &    2.003 & 4.804E-09 &    2.000 & 3.703E-10 &    2.000 &   1399.6 \tabularnewline
%                          &  7.49 &  0.01 & 9.904E-12 &    2.001 & 1.201E-09 &    2.000 & 9.257E-11 &    2.000 &   1909.1 \tabularnewline
%                          &  3.00 &  0.00 & 1.598E-12 &    1.991 & 1.922E-10 &    2.000 & 1.481E-11 &    2.000 &   3540.6 \tabularnewline
%                          &  1.50 &  0.00 & 4.542E-13 &    1.815 & 4.812E-11 &    1.998 & 3.703E-12 &    2.000 &   6299.9 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ ARS443P }& 1497.94 &  1.00 & 7.160E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &  57792.7 \tabularnewline
%                          & 748.97 &  0.50 & 1.429E-07 &    2.325 & 1.822E-06 &    2.938 & 5.065E-07 &    2.357 &  48308.7 \tabularnewline
%                          & 149.79 &  0.10 & 1.298E-09 &    2.921 & 1.484E-08 &    2.989 & 4.701E-09 &    2.908 &  11462.6 \tabularnewline
%                          & 74.90 &  0.05 & 1.583E-10 &    3.036 & 1.858E-09 &    2.998 & 5.777E-10 &    3.025 &   6100.7 \tabularnewline
%                          & 29.96 &  0.02 & 9.950E-12 &    3.020 & 1.190E-10 &    2.999 & 3.645E-11 &    3.016 &   3776.6 \tabularnewline
%                          & 14.98 &  0.01 & 1.256E-12 &    2.986 & 1.515E-11 &    2.974 & 4.545E-12 &    3.004 &   3764.3 \tabularnewline
%                          &  7.49 &  0.01 & 2.552E-13 &    2.299 & 3.398E-12 &    2.157 & 5.890E-13 &    2.948 &   4862.9 \tabularnewline
%                          &  3.00 &  0.00 & 2.026E-13 &    0.252 & 2.834E-12 &    0.198 & 1.032E-13 &    1.901 &   7826.9 \tabularnewline
%                          &  1.50 &  0.00 & 2.187E-13 &   -0.110 & 2.831E-12 &    0.002 & 1.119E-13 &   -0.117 &  13226.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}
 
%---------------------
% TEMPORAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in two dimensions:
    time convergence study on a nonuniform mesh.
    The computational domain is discretized with $N_e = 256$ and $k=8$.
    The error is measured at $T=1$. 
}
\tablab{expo-euler-isentropic-tconv-nonuni-p8}

\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
\hline
\multirow{2}{*}{$k=8$} 
  % & \multirow{2}{*}{$dt$}  
  & \multirow{2}{*}{$Cr$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  & \multirow{2}{*}{wc $[s]$}    \tabularnewline
  &     &  error & order &  error & order &  error & order &     \tabularnewline
\hline\hline
\multirow { 2}{*}{   RK2 }&  0.29  & 1.618E-09 &        - & 1.586E-09 &        - & 5.310E-10 &        - &    188.2 \tabularnewline
                         &  0.15  & 1.618E-09 &    0.000 & 1.584E-09 &    0.002 & 5.309E-10 &    0.000 &    393.2 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK3 }&  0.59  & 1.618E-09 &        - & 1.584E-09 &        - & 5.308E-10 &        - &    107.6 \tabularnewline
                         &  0.29  & 1.618E-09 &    0.000 & 1.584E-09 &    0.000 & 5.308E-10 &    0.000 &    227.8 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK4 }&  0.90  & 1.618E-09 &        - & 1.584E-09 &        - & 5.308E-10 &        - &    116.2 \tabularnewline
                         &  0.45  & 1.618E-09 &    0.000 & 1.584E-09 &    0.000 & 5.308E-10 &    0.000 &    259.3 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{  EPI2 }& 452.34  & 2.583E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &     55.2 \tabularnewline
                         & 226.17  & 5.085E-07 &    2.345 & 6.518E-07 &    2.367 & 1.790E-06 &    2.341 &     61.3 \tabularnewline
                         & 45.23  & 2.038E-08 &    1.999 & 2.442E-08 &    2.041 & 7.153E-08 &    2.001 &     54.2 \tabularnewline
                         & 22.62  & 5.326E-09 &    1.936 & 6.298E-09 &    1.955 & 1.786E-08 &    2.002 &     53.6 \tabularnewline
                         &  9.05  & 1.810E-09 &    1.178 & 1.872E-09 &    1.324 & 2.885E-09 &    1.990 &     58.0 \tabularnewline
                         &  4.52  & 1.631E-09 &    0.150 & 1.603E-09 &    0.224 & 8.786E-10 &    1.715 &    114.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ EXPRB32 }& 452.34  & 1.807E-07 &        - & 1.608E-07 &        - & 6.291E-07 &        - &    108.4 \tabularnewline
                         & 226.17  & 1.142E-08 &    3.984 & 1.571E-08 &    3.356 & 3.958E-08 &    3.990 &    108.8 \tabularnewline
                         & 45.23  & 1.623E-09 &    1.212 & 1.591E-09 &    1.423 & 5.922E-10 &    2.611 &    111.6 \tabularnewline
                         & 22.62  & 1.619E-09 &    0.004 & 1.588E-09 &    0.003 & 5.280E-10 &    0.166 &    114.9 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.001 & 1.621E-09 &   -0.022 & 5.304E-10 &   -0.005 &    120.1 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.033 & 5.308E-10 &   -0.001 &    228.7 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ EXPRB42 }& 452.34  & 7.525E-08 &        - & 2.216E-07 &        - & 2.652E-07 &        - &     89.7 \tabularnewline
                         & 226.17  & 4.623E-09 &    4.025 & 5.182E-09 &    5.418 & 1.518E-08 &    4.127 &     92.0 \tabularnewline
                         & 45.23  & 1.618E-09 &    0.652 & 1.585E-09 &    0.736 & 5.280E-10 &    2.087 &     94.4 \tabularnewline
                         & 22.62  & 1.618E-09 &    0.000 & 1.586E-09 &   -0.001 & 5.262E-10 &    0.005 &     93.0 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.000 & 1.595E-09 &   -0.006 & 5.298E-10 &   -0.007 &    120.0 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.010 & 5.308E-10 &   -0.003 &    229.3 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ ARS232 }& 452.34  & 1.521E-06 &        - & 4.685E-05 &        - & 6.384E-06 &        - &   1707.7 \tabularnewline
                         & 226.17  & 1.715E-07 &    3.149 & 1.193E-05 &    1.973 & 1.028E-06 &    2.635 &    934.7 \tabularnewline
                         & 45.23  & 4.427E-09 &    2.272 & 4.803E-07 &    1.996 & 3.718E-08 &    2.063 &    260.1 \tabularnewline
                         & 22.62  & 1.904E-09 &    1.217 & 1.201E-07 &    2.000 & 9.274E-09 &    2.003 &    217.6 \tabularnewline
                         &  9.05  & 1.626E-09 &    0.172 & 1.928E-08 &    1.996 & 1.566E-09 &    1.941 &    241.1 \tabularnewline
                         &  4.52  & 1.619E-09 &    0.006 & 5.062E-09 &    1.929 & 6.429E-10 &    1.284 &    345.7 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ ARS443 }& 452.34  & 7.160E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &   6312.7 \tabularnewline
                         & 226.17  & 1.430E-07 &    2.324 & 1.822E-06 &    2.938 & 5.065E-07 &    2.357 &   4786.2 \tabularnewline
                         & 45.23  & 2.113E-09 &    2.619 & 1.493E-08 &    2.985 & 4.694E-09 &    2.909 &   1268.1 \tabularnewline
                         & 22.62  & 1.631E-09 &    0.374 & 2.443E-09 &    2.611 & 7.124E-10 &    2.720 &    910.2 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.009 & 1.588E-09 &    0.470 & 5.168E-10 &    0.350 &    743.4 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.004 & 5.285E-10 &   -0.032 &    869.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}

To demonstrate the high-order convergence in space,  
we perform the spatial convergence test.
We use a sequence of nested meshes with $N_e = \LRp{256,1024,4096,16384}$ 
for $k=\LRp{1,2,3,4}$ and measure the errors at $t=1$. 
As can be seen in Table \tabref{expo-euler-isentropic-sconv-uni},
the convergence rate of $(k + \half)$ is observed as refining the meshes.

%---------------------
% SPATIAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Spatial convergence for the isentropic vortex translation in two dimensions.
    We use a sequence of nested meshes with $N_e = \LRc{256, 1024, 4096, 16384}$ for $k=\LRc{1,2,3,4}$. 
    We use EXPRB42 scheme with $dt=0.01$ and measure the errors at $t=1$.  
}
\tablab{expo-euler-isentropic-sconv-uni}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
\hline
\multirow{2}{*}{ } 
  & \multirow{2}{*}{$h$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  \tabularnewline
  &    &  error & order &  error & order &  error & order       \tabularnewline
\hline\hline
\multirow { 4}{*}{    k=1 }&  1.00 & 9.942E-04 &        - & 7.389E-03 &        - & 1.595E-03 &        - \tabularnewline
                         &  0.50 & 7.662E-04 &    0.376 & 1.999E-03 &    1.886 & 5.181E-04 &    1.622 \tabularnewline
                         &  0.25 & 4.344E-04 &    0.819 & 5.312E-04 &    1.912 & 2.049E-04 &    1.338 \tabularnewline
                         &  0.12 & 2.312E-04 &    0.910 & 1.383E-04 &    1.941 & 8.571E-05 &    1.257 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=2 }&  1.00 & 2.909E-04 &        - & 7.382E-04 &        - & 4.423E-04 &        - \tabularnewline
                         &  0.50 & 1.201E-04 &    1.276 & 1.418E-04 &    2.380 & 4.965E-05 &    3.155 \tabularnewline
                         &  0.25 & 3.235E-05 &    1.892 & 1.570E-05 &    3.175 & 7.084E-06 &    2.809 \tabularnewline
                         &  0.12 & 5.787E-06 &    2.483 & 2.084E-06 &    2.913 & 1.257E-06 &    2.495 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=3 }&  1.00 & 1.286E-04 &        - & 2.343E-04 &        - & 6.979E-05 &        - \tabularnewline
                         &  0.50 & 1.972E-05 &    2.705 & 1.541E-05 &    3.926 & 5.605E-06 &    3.638 \tabularnewline
                         &  0.25 & 2.123E-06 &    3.215 & 9.655E-07 &    3.996 & 4.450E-07 &    3.655 \tabularnewline
                         &  0.12 & 2.112E-07 &    3.329 & 6.849E-08 &    3.817 & 4.386E-08 &    3.343 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=4 }&  1.00 & 2.686E-05 &        - & 3.180E-05 &        - & 1.311E-05 &        - \tabularnewline
                         &  0.50 & 2.067E-06 &    3.700 & 1.283E-06 &    4.631 & 4.381E-07 &    4.903 \tabularnewline
                         &  0.25 & 9.543E-08 &    4.437 & 4.294E-08 &    4.901 & 1.333E-08 &    5.039 \tabularnewline
                         &  0.12 & 4.540E-09 &    4.394 & 1.458E-09 &    4.880 & 5.294E-10 &    4.654 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}


%------------------------------3D---------------------------
Figure \figref{expo-euler3d-ss-isentropic} shows snapshots of advecting isentropic vortex at $t=[0,10,25]$ in three-dimensions. For spatial discretization, we 
take $N_e = 6400$ elements and $k=8$ solution order on a uniform mesh. 
For time discretization, we choose EPI2 with $dt=0.25 (Cr=27.9)$. 
We see the center of the vortex is located at the lateral boundary at $t=25$
because the mean speed of the flow is $0.2$ and the half-length of the
domain is $5$.
% \tanbui{Do we have exact solution here? If yes, plotting the error
%   (i.e. contours or pointwise values)
%   between the exact and numerical solutions is much more informative.}
% \shinhoo{I think we can do later if it needed.}

%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[$t=0$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t0}
      \figlab{expo-euler3d-ss-isentropic-epi2-t0}
    }
    \subfigure[$t=10$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t10}
      \figlab{expo-euler3d-ss-isentropic-epi2-t10}
    }
    \subfigure[$t=25$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t25}
      \figlab{expo-euler3d-ss-isentropic-epi2-t25}
    }
  \caption{Isentropic vortex translation in three dimensions: 
    snapshots for (a) EPI2 with $Cr=27.9 (dt=0.25)$.
    Simulations are performed on the grid with $N_e = 6400$ and $k=8$ solution order for $t \in [0,20]$.}
  \figlab{expo-euler3d-ss-isentropic}
\end{figure}

Now we study the parallel performance of Exponential DG methods for three-dimensional Euler model.
Parallel simulations are conducted on Stampede2 at the Texas Advanced Computing Center (TACC).  
Stampede 2 provides 4,200 Knights Landing (KNL) nodes and 1,736 Skylake (SKX) nodes. Each node of KNL consists of 68 cores of Intel Xeon Phi 7250 1.4GHz processors, 96 GB of traditional DDR4 RAM, and 16 GB high-speed MCDRAM. 
Each node of SKX consists of 48 cores of Intel Xeon Platinum 8160 2.1 GHz processors and 192GB DDR4 RAM. The interconnect is a 100 GB/s Intel Omni-Path (OPA) network with a fat-tree topology. We conduct strong and weak scaling study on SKX system. 
%To this end, we have implemented the adaptive Krylov subspace method \cite{gaudreault2018kiops}
%on top of the DG finite element library written in C\texttt{++}, which is the spin-off library from \texttt{mangll} \cite{wilcox2010high}. 
%For computing a matrix exponential, 
%we use \texttt{EIGEN} C\texttt{++} library.
%Parallel implementations mainly focus on vector-vector multiplication and matrix-vector multiplication.
%The matrix-vector multiplication is carried out in a matrix-free manner 
%by calling the linear operator $L\qb$ in \eqnref{EXPO-SemiDiscretizedForm_ode}. 
%By the virtue of the DG discretization, the computation of $L\qb$ is embarrassingly parallel.
%For a dot product (vector-vector multiplication), we initially scatter a global vector to each processor, and then we perform the dot product with the local vector.  
%Next, we call \texttt{MPI ALLreduce} function. 

Recall that EPI2 and RK4 show similar performance for $k=8$ solution on the uniform mesh,
as seen in Figure \figref{expo-euler-isentropic-tconv-uni-p8}.
We will see how they perform in parallel computing. 
In Table \tabref{expo-euler-strongscale-isentropic-withRK}, 
strong scaling results of EPI2 are compared with the RK4 counterpart. 
Domain is discretized with $N_e=6400$ elements and $k=8$ solution order.
We take $dt=0.25 (Cr=27.9)$ for EPI2 and $dt=0.005 (Cr=0.56)$ for RK4 
and perform the simulations up to $t=2$. 
In general, EPI2 is comparable to RK4 in terms of wallclock time. 
The efficiency 
\footnote{
Efficiency is defined by $\frac{T_s}{T_p n_p}$
with $n_p$ the number of processors, $T_s$ serial wallclock time and $T_p$ parallel wallclock time.
Here, we approximate $T_s \simeq T_{base} \times n_{p_{base}}$ 
where $T_{base}$ is parallel wallclock time with $n_{p_{base}}$ cores. 
}
of EPI2 is slightly better than the RK4 counterpart. 
For both EPI2 and RK4, we see the efficiency drops as increasing the number of processors. This is because the number of elements per core decreases as increasing cores so that the communication cost starts to dominate over the computational cost. 

%---------------------
% STRONG SCALING
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with $Cr=27.9 (dt=0.25)$ 
  and RK4 with $Cr=0.56 (dt=0.005)$
  are performed with $N_e=6400$ and $k=8$ solution order up to $t=2$. 
}
\tablab{expo-euler-strongscale-isentropic-withRK}
\begin{center}
\begin{tabular}{c|c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} & \multirow{2}{*}{$N_e/core$}
& \multicolumn{2}{c|}{EPI2}
& \multicolumn{2}{c}{RK4}   \tabularnewline
     &     & Wallclock [s] & Efficiency
           & Wallclock [s] & Efficiency \tabularnewline
\hline\hline
32 & 200  & 1283& 100& 1014&100 \tabularnewline
64 & 100    & 537.3& 119.4& 501.6&101.1\tabularnewline
128 & 50     & 424.8& 75.5& 315.5& 80.3\tabularnewline
256 & 25      &148.6& 107.9& 225.9&56.1\tabularnewline
512 & 12.5   & 114.1& 70.3& 118.1& 53.7\tabularnewline
1024 & 6.3   & 64.38&62.3& 64.49& 49.1\tabularnewline
2048 & 3.1& 39.38& 50.9& 37.11&42.7\tabularnewline
4096 &  1.6 & 24.39&41.1&20.17&39.3\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

We can increase the efficiency by assigning more elements to each processor. 
%Next, we assign additional elements to each processor by refining the mesh. 
  Table \tabref{expo-euler-strongscale-isentropic-ndof} compares the efficiencies of two different spatial discretization: 
(i) $N_e=51200$ elements and $k=6$ solution order, 
and (ii)$N_e=6400$ elements and $k=8$ solution order. 
The number of elements per core for the former discretization is eight-times larger than that for the latter. 
The efficiency with the former becomes higher than the latter counterpart as increasing the number of cores. 
%That is the number of elements per core decreases. 
\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with different degrees-of-freedoms (DOF).
  For the number of DOF (NDOF) of $17,561,600$, 
   simulations are performed on $N_e=51200$ and $k=6$ solution order
   with $dt=0.25(Cr=32.98)$ up to $t=1$, 
   whereas for NDOF of $4,665,600$, 
   simulations are performed on $N_e=6400$ and $k=8$ solution order
   with $dt=0.25(Cr=27.93)$ up to $t=2$.  
}
\tablab{expo-euler-strongscale-isentropic-ndof}
\begin{center}
\begin{tabular}{c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} 
& \multicolumn{2}{c|}{$NDOF=17,561,600$}
& \multicolumn{2}{c}{$NDOF=4,665,600$}   \tabularnewline
           & $N_e/core$ & Efficiency
           & $N_e/core$ & Efficiency \tabularnewline
\hline\hline
32  & 1600  & 100   & 200  & 100   \tabularnewline
64  & 800   & 97.9  & 100  & 119.4 \tabularnewline
128 & 400   & 82.7  & 50   & 75.5  \tabularnewline
256 & 200   & 85.7  & 25   & 107.9 \tabularnewline
512 & 100   & 61.9  & 12.5 & 70.3  \tabularnewline
1024 & 50   & 59.2  & 6.3  & 62.3  \tabularnewline
2048 & 25   & 55.0  & 3.1  & 50.9  \tabularnewline
4096 & 12.5 & 51.4  & 1.6  & 41.1  \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


To understand the effect of the timestep size on efficiency, 
we conduct strong scaling tests with two different timestep sizes, 
$dt=0.125$ and $dt=0.25$, 
on the mesh with $N_e=51200$ elements and $k=6$ solution order. 
As shown in Table \tabref{expo-euler-strongscale-isentropic-varyCr}, 
the efficiency with $dt=0.125$ is slightly higher than that with $dt=0.25$. 
This is because the latter case involves more Krylov iterations than the former case.
The total number of Krylov steps $N_{Krylov}$ is 
$561$ for $dt=0.125$ and $1024$ for $dt=0.25$.
This implies that the spectrum of the linear operator becomes broad by increasing the timestep size 
\footnote{
Note that the input argument of $\varphi$-function is $\triangle t L$. 
}.


%EPI2 allows a large timestep size, but the cost increases, too. %It seems that doubling the timestep size increases the computational cost two-times. This is somewhat makes sense because EPI2 adds more sub-steps with the large time intervals. 

\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with $Cr=16.49 (dt=0.125)$
  and $Cr=32.98 (dt=0.25)$
  are performed with $N_e=51200$ and $k=6$ solution order up to $t=1$.
}
\tablab{expo-euler-strongscale-isentropic-varyCr}
\begin{center}
\begin{tabular}{c|c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} & \multirow{2}{*}{$N_e/core$}
& \multicolumn{2}{c|}{$dt=0.125$}
& \multicolumn{2}{c}{$dt=0.25$}   \tabularnewline
     &     & Wallclock [s] & Efficiency
            & Wallclock [s] & Efficiency \tabularnewline
\hline\hline
32   & 1600 & 2346  & 100  & 4151  & 100 \tabularnewline
64   & 800  & 1199  & 97.8 & 2121  & 97.9 \tabularnewline
128  & 400  & 607.7 & 96.5 & 1255  & 82.7 \tabularnewline
256  & 200  & 306.9 & 95.6 & 605.7 & 85.7 \tabularnewline
512  & 100  & 237.3 & 61.8 & 419.1 & 61.9 \tabularnewline
1024 & 50   & 122.7 & 59.7 & 219.1 & 59.2 \tabularnewline
2048 & 25   & 61.33 & 59.5 & 118.0 & 55.0 \tabularnewline
4096 & 12.5 & 33.72 & 54.4 & 63.12 & 51.4 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

Based on the above observations, 
we conduct a strong scaling test for EPI2 
with $Cr=8.1 (dt=0.03125)$, $N_e = 3,276,800$ and $k=4$ solution order.
We use the consecutive processors, $n_p=\LRc{16,32,64,128,256,512,868}\times 48$
so that the number of elements per core approximately becomes $\LRc{4267, 2133, 1067, 533, 267, 133, 79}$. 
%so that the number of elements per core becomes $\LRc{4266.7, 2133.3, 1066.7, 533.3, 266.7, 133.3, 78.6}$. 
In Figure \figref{expo-euler-strongscale-isentropic-withEPI2},
the speedup
\footnote{
Speedup is defined as $\frac{T_s}{T_p}$
with $T_s$ serial wallclock time and $T_p$ parallel wallclock time.
} factor shows a good strong scalability up to 41664 cores 
(which is the maximum cores in Skylake system in TACC).

% and is comparable to 
%the speedup factor of RK4 up to 4096 cores. 

\begin{figure}[h!t!b!]
    \centering
%    \subfigure[EPI2]{
      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.83\textwidth]{./figures/EXPO-euler-strongscale-epi2}
      \figlab{expo-euler-strongscale-isentropic-epi2}
 %   }
  %  \subfigure[RK4]{
  %   \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler-strongscale-rk4} 
  %    \figlab{expo-euler-strongscale-isentropic-rk4}
  %  }
  \caption{Isentropic vortex translation in three dimensions: 
    strong scaling study for EPI2 with $Cr=8.1 (dt=0.03125)$. 
    The computational domain is discretized with $N_e = 3,276,800$ and $k=4$ solution order
 for $n_p=\LRc{16,32,64,128,256,512,868}\times 48$.}
  \figlab{expo-euler-strongscale-isentropic-withEPI2}
\end{figure}


For the weak scaling test, 
we assign the same amount of work to each processor 
while increasing the number of processors. 
We discretize the domain with 
$N_e = \LRc{1, 8, 64, 512, 4096}\times 100$ elements and $k=8$ solution order, 
and decompose the domain with $n_p = \LRc{4, 32, 256, 2048, 16384}$ processors. 
That is, we make the number of elements per core to be 25.
We also keep the Courant number fixed 
so that the total number of Krylov steps, $N_{Krylov}$ to be uniform.
We have tabulated the weak scaling results in Table \tabref{expo-euler-weakscale-isentropic-fixcr}. We observe that $N_{Krylov}$ tends to linearly increase with the Courant number. We also see that the increment of wallclock time is relatively small for a fixed Courant number. We plot the average time per timestep against the number of degrees-of-freedom in Figure \figref{expo-euler-weakscale-isentropic-fixcr}, from which we see Exponential DG methods show a good weak scaling result. 

%---------------------
% Weak scaling test 
%---------------------

\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  weak scaling results for EPI2 with fixed Courant numbers.
  Each core has $18,225$ degrees-of-freedom (=$25$ elements and $8th$ solution order). 
}
\tablab{expo-euler-weakscale-isentropic-fixcr}
\begin{center}
\begin{tabular}{cc|c|c|c|c}
\hline
$Cr$ &$N_e$ & $dt$ & Final time & Wallclock [s] & $N_{Krylov}$ \tabularnewline
\hline\hline 
\multirow{4}{*}{$ 5.59$}  
  &  4   & 0.2    & 0.8  & 15.3  & 103 \tabularnewline
  & 32   & 0.1    & 0.4  & 17.8  & 90 \tabularnewline
  & 256  & 0.05   & 0.2  & 24.4  & 81 \tabularnewline
  & 2048 & 0.025  & 0.1  & 27.8  & 81 \tabularnewline
  & 16384& 0.0125 & 0.05 & 29.3  & 82 \tabularnewline
\tabularnewline
\multirow{4}{*}{$ 22.4$}  
  &  4   & 0.2   & 0.8  & 50.4  & 397 \tabularnewline
  & 32   & 0.1   & 0.4  & 89.9  & 381 \tabularnewline
  & 256  & 0.05  & 0.2  & 85.8  & 355 \tabularnewline
  & 2048 & 0.025 & 0.1  & 86.9  & 348 \tabularnewline
  &16384 & 0.0125& 0.05 & 93.1  & 358 \tabularnewline
\tabularnewline
\multirow{4}{*}{$ 55.9$}  
  &  4   & 0.2   & 0.8  & 130.9 & 1024\tabularnewline
  & 32   & 0.1   & 0.4  & 240.4 & 1023 \tabularnewline
  & 256  & 0.05  & 0.2  & 246.2 & 1024 \tabularnewline
  & 2048 & 0.025 & 0.1  & 248.8 & 1024 \tabularnewline
  &16384 & 0.0125& 0.05 & 342.2 & 1408 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-euler-weakscale-fixedCr} 
  \caption{Isentropic vortex translation in 3D: 
    weak scaling study with fixed Courant numbers. 
    The computational domain is discretized with $N_e = \LRc{1, 8, 64, 512,4096}\times 100$ and $k=8$ solution order for $n_p=\LRc{4,32,256,2048,16384}$, respectively,
    so that each processor has 25 elements. }
  \figlab{expo-euler-weakscale-isentropic-fixcr}
\end{figure}

What would happen if we fix timestep size $dt$ instead of Courant number $Cr$? 
By refining the mesh, we add geometrically-induced stiffness to the system,
which causes the total number of Krylov steps to grow. 
This is why we see the wallclock time tends to increase with the number of degrees-of-freedom for a fixed $dt$ 
in Figure \figref{expo-euler-weakscale-isentropic-fixdt}. 
The corresponding total number of Krylov steps are summarized in 
Table \tabref{expo-euler-weakscale-isentropic-fixdt}.
As we refine the mesh by a factor of two along $x$, $y$, and $z-$direction,
the total number of Krylov steps tends to linearly increase for $dt=0.25$ and $dt=2.5$. 
%That is, we add geometrically-induced stiffness to the system.
%We can consider the total number of Krylov steps as an indicator of stiffness in the system. 
%One of the attractive feature of the adaptive Krylov subspace method is that 
%the stiffness is automatically detected and handled by adding more substeps or increasing the dimension of Krylov subspace methods.

\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-euler-weakscale-fixedDt} 
  \caption{Isentropic vortex translation in three dimensions: 
    weak scaling study with a fixed timestep size.
    The computational domain is discretized with $N_e = \LRc{100, 800, 6400, 51200}$ and $k=8$ solution order for $n_p=\LRc{4,32,256,2048}$, respectively,
    so that each processor has 25 elements. }
  \figlab{expo-euler-weakscale-isentropic-fixdt}
\end{figure}



\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  the total number of Krylov steps, $N_{Krylov}$, approximately linearly depends on Courant number for $dt=0.25$ and $dt=2.5$. 
}
\tablab{expo-euler-weakscale-isentropic-fixdt}
\begin{center}
\begin{tabular}{c||cc|cc|cc|cc}
\hline
\multirow{2}{*}{$dt$} 
& \multicolumn{2}{c|}{$N_e=100$}  
& \multicolumn{2}{c|}{$N_e=800$} 
& \multicolumn{2}{c|}{$N_e=6400$} 
& \multicolumn{2}{c}{$N_e=51200$}   \tabularnewline
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$\tabularnewline
 \hline\hline
 0.025 & 0.7   & 40     & 1.4    & 40    & 2.8       & 45    & 5.6     & 81  \tabularnewline
 0.25  &  7.0  & 128   & 14.0 & 233   & 27.9.    &448   & 55.9   & 1024 \tabularnewline
 2.5    & 69.8 & 1536 &139.7 & 3072 &279.32 &5120 & 558.7 & 10112 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}




==> NumericalResults_allenCahn.tex <==
\section{Numerical Results}
\seclab{NumericalResults}

% \tanbui{
% Our main point to show for exponential DG is: 1) its stability is similar to
% implicit method, 2) its cost is similar to explicit RK DG method (and thus
% more efficient than implicit DG method), 3) its paralell
% scalability is similar to explicit DG methods, 3) it is high-order in
% both space and time; 4) it can deal with stiff problems robustly and
% efficiently (large Courant numbers without stability compared to
% explicit methods, and much less cost compared to fully implicit
% method, and 5) it is more efficient, e.g. scalability, than IMEX methods.
% If you can show all these points, the method (and hence the paper) is
% very convincing and appealing. Otherwise, we will run into the
% problems with the reviewers later and it will be very hard to publish
% the work. We have already had similar experinece with the IMEX HDG-DG
% paper, and we don't want to run in to the same problems again if we
% like to publish the work in SISC, or JCP, or CMAME.
% }
% \shinhoo{
%   We show the main point through numerical examples.
%   Exponential DG 
%   1) is stable with a large Courant number ($Cr>1$) similar to IMEX DG;
%   2) becomes comparable to RKDG on uniform grid, and beneficial on nonuniform grid;
%   3) shows similar parallel performance to RKDG; 
%   4) supports high-order solutions in space and time in isentropic vortext case;
%   5) is more efficient than IMEX DG in terms of computational cost. 
% }
  
In this section, we conduct several numerical experiments 
to evaluate the performance of the proposed framework.
In particular, we examine the numerical stability for a wide range of Courant numbers $(Cr>1)$;
the high-order convergence; the accuracy and the efficiency; its weak and strong scalability.
For numerical simulations, 
we consider a system of ordinary differential equations
(ODE), Allen-Cahn equation, viscous Burgers
equation, and Euler equations. 



% differential equations (ODE) with different linearized forms. Then, we
%  deal with
% the one-dimensional Allen-Cahn equation and viscous Burgers
% equation. Finally, we solve Euler equations in two- and
% % three-dimensional domains.
% Of interest are the high-order convergence in both time and space, the
% strong and weak
% scalability, and the ability to use large Courant number ($Cr > 1$) of
% the proposed approach.

%\tanbui{We need to present the convergence in space as
%  well to justify the proposed exponential DG.}

\subsection{A system of two ordinary differential equations (ODE)}
\seclab{EXPO-numericalResults-ODE}

%Exponential time integrators require the decomposed system in \eqnref{nonlinear_ivp_split}, i.e., the linear and the nonlinear terms.
% In Exponential DG framework, we construct the linear term in \eqnref{linearflux} and \eqnref{linearsource}, based on linearization.
% This is because linearized operators typically  capture the rapidly varying physics. 
% %This is one way to build the linear term in \eqnref{nonlinear_ivp_split}.
% We will illustrate the benefit of using Jacobian in the following example.
%The question is how we build the linear operator?

We consider the autonomous system of two ODEs
 proposed by \cite{cox2002exponential}
\begin{subequations}
\begin{align}
  \DD{u(t)}{t} &= c u - v + (\lambda v - c u)  r^2, \\
  \DD{v(t)}{t} &= u + c v - (\lambda u + c v)  r^2,
\end{align}
 \eqnlab{ode-system-ex-goveq}
\end{subequations}
where $r^2 = u^2 + v^2$, $c>0$ constant, 
$u=r\cos \theta$, $v = r\sin\theta$. 
The exact solution is given by 
% \begin{subequations}
\begin{align*}
  r^2(t) &= r_0^{2}
  \LRp{r_0^2 \LRp{1-e^{-2 c t }} + e^{-2 c t} }^{-1},\\
  \theta(t) &= \theta_0 + (1-\lambda)t 
             - \frac{\lambda}{2 c} 
             \log\LRp{r_0^2 \LRp{1-e^{-2 c t}} + e^{-2c t} }.
\end{align*}
 % \eqnlab{ode-system-ex-exactsolution}
% \end{subequations}
For a numerical simulation, we take $c=100$,
$\lambda=\half$, $u_0 = u(0)=2$ and $v_0= v(0)=1$. 
The exact solution with the parameters is shown in Figure \figref{system-ode-ex-sol}.
The magnitude and the phase of the solution rapidly change within a
short period of time. 

%---------------------
% EXACT SOLUTION PLOT
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Magnitude]{
      \includegraphics[trim=1.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.45\textwidth]{./figures/EXPO-SystemODE-exact-magnitude}
      \figlab{system-ode-ex-exact-magnitude}
    }
    \subfigure[Phase]{
      \includegraphics[trim=1.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.45\textwidth]{./figures/EXPO-SystemODE-exact-phase} 
      \figlab{system-ode-exact-phase}
    }
    \caption{System of two ODEs: (a) magnitude and (b) phase of the exact solution.}
     % of 
     %  \eqnref{ode-system-ex-exactsolution}. }
    \figlab{system-ode-ex-sol}
  \end{figure}


Let $\qb=(u,v)^T$ and $\Rb(\qb)$ be the right hand-side of \eqnref{ode-system-ex-goveq}. We define two linear operators:
one is the constant linear operator \cite{cox2002exponential}
\begin{align}
\eqnlab{linearop-const}
L_{c}:=\begin{pmatrix}
c & -1\\
1 & c
\end{pmatrix}
\end{align} 
and the other is Jacobian 
%\tanbui{Please recheck. I could be wrong,
%  but a quick check on the second row does not give the same results
%  as yours. Also the Jacobian is a function of $\qb$, we should
%  make it clear in the definition of $L_d$, e.g. $L_q\LRp{\qb}$. To be consistent with
%  \eqnref{linearflux}, we should also use $\tilde{\qb}$ here.}
%How do we choose a linear operator to capture the characteristics of a rapidly changing system?
%To address the question, we consider the two linear operators: 
%the dynamic Jacobian operator
\begin{align}
\eqnlab{linearop-dynamic}
L_{d}\LRp{\qbtilde}:=\dd{\Rb}{\qb}\bigg|_\qbtilde
=\begin{pmatrix}
    c(1-\rtilde^2) + 2 \utilde (\lambda \vtilde - c \utilde) 
  & -1 + \lambda \rtilde^2 + 2 \vtilde (\lambda \vtilde - c \utilde) \\
    1 - \lambda \rtilde^2 - 2 \utilde (\lambda \utilde + c \vtilde)
  & c(1-\rtilde^2) - 2 \vtilde (\lambda \utilde + c \vtilde) 
\end{pmatrix}.
\end{align}
% evaluated at each timestep $t^n$, 
%Since $L_d$ is a function of $(u,v)$, we can dynamically update $L_d(u^n,v^n)$ at each time $t^n$,
%whereas $L_c$ is a constant matrix, which may not capture the fast characteristics of the system.

The first-order exponential time differencing (ETD1) method \cite{cox2002exponential} 
reads
\begin{align}
  \eqnlab{etd1}
  \qb^{n+1}
  = e^{\dt L} \qb^n
  + \dt \varphi_1 (\dt L) \mc{N}^{(0)},
\end{align}
where
$\qb^n:=\qb(t^n)$, $L=L_d \text{ or } L_c$,
$ \mc{N}^{(0)} := \Rb^n - L \qb^n$ and 
$\Rb^n:=\Rb(\qb^n)$. 
We denote ETD1 method with the constant linear operator \eqnref{linearop-const} by ETD1-L, 
and the one with the Jacobian \eqnref{linearop-dynamic} by ETD1-J 
in which the Jacobian is evaluated at each timestep. 
We also let the ETD1 method with the fixed Jacobian \eqnref{linearop-dynamic} 
evaluated at $\qbtilde_0=(u_0,v_0)^T$ by ETD1-J0.
Indeed, ETD1-J is equivalent to the second-order EPI2 \cite{tokman2006efficient},
\begin{align*}
  \qb^{n+1}
  &= \qb^n + \dt \varphi_1(L_d\triangle t) \Rb^n.
\end{align*}
This form is computationally attractive because it needs only one matrix exponential instead of two in \eqnref{etd1} \cite{hochbruck2010exponential}. 

\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-ode-tconv}
  \caption{System of two ODEs: time convergence study of ETD1-L, ETD1-J, and EPI2.
  We observe the first-order convergence rate for ETD1-L and the second-order convergence rate for ETD1-J and EPI2.
  The use of Jacobian improves not only the accuracy but also the stability of ETD1. }
  \figlab{expo-ode-tconv}
\end{figure}


Figure \figref{expo-ode-tconv} demonstrates the benefit of using the Jacobian in terms of accuracy and stability. 
We measure the errors of magnitude $r$ and phase $\theta$ at $T=1$ for ETD1-L, ETD1-J, and EPI2 methods. 
The error levels of ETD1-J0 for $r$ and $\theta$ are three orders of magnitude and four times larger than ETD1-L counterparts, respectively.
However, ETD1-J0 shows better stability than ETD1-L.
The errors of ETD1-L and ETD1-J0 show the first-order convergence rate in both the magnitude and the phase errors,
whereas the ETD1-J counterpart shows the second-order convergence rate.
Not only that, ETD1-J allows a larger timestep size without facing
instabilities.  %than ETD1-L.
This demonstrates the importance of using Jacobian.
%\tanbui{you didn't discuss the reference value $\tilde{u}$ here. Does
%  it change for each time step? We should compare the case with fixed
%  reference $\tilde{\qb}$ and varying (linearize around the solution of
%  the previous time step) $\tilde{\qb}$}


%% \begin{table}[t]
%% \caption{System of two ODEs: time convergence study of ARS111 and ETD1.
%% Using $L_d$ gives better stability and accuracy than using $L_c$. 
%% With the small timestep size ($dt < 10^{-3}$), 
%% ETD1 solutions are more accurate than ARS111 solutions. 
%% }
%%  \tablab{expo-ode-tconv}
%% \begin{center}
%% \begin{tabular}{*{1}{c}|c||cccc|cccc}
%% \hline
%% \multirow{2}{*}{ $L$ } 
%%   & \multirow{2}{*}{dt} 
%%   & \multicolumn{4}{c|}{$ETD1$}   
%%   & \multicolumn{4}{c}{$ARS1$}   \tabularnewline
%%     &    
%%     &   $\norm{r - r^e}$ & {\small rate} & $\norm{\theta-\theta^e}$ & {\small rate}
%%     &   $\norm{r - r^e}$ & {\small rate} & $\norm{\theta-\theta^e}$ & {\small rate}\tabularnewline
%% \hline\hline
%% \multirow { 6}{*}{    $ L_c$ }& 2.0E-5 & 1.3E-08 &        - & 5.2E-04 &        - & 3.8E-08 &        - & 1.0E-03 &        - \tabularnewline
%%                          & 5.0E-5 & 3.1E-08 &      1.0 & 1.3E-03 &      1.0 & 9.4E-08 &      1.0 & 2.6E-03 &      1.0 \tabularnewline
%%                          & 1.0E-4 & 6.2E-08 &      1.0 & 2.6E-03 &      1.0 & 1.9E-07 &      1.0 & 5.2E-03 &      1.0 \tabularnewline
%%                          & 2.0E-4 & 1.3E-07 &      1.0 & 5.2E-03 &      1.0 & 3.8E-07 &      1.0 & 1.1E-02 &      1.0 \tabularnewline
%%                          & 5.0E-4 & 3.1E-07 &      1.0 & 1.3E-02 &      1.0 & 9.9E-07 &      1.0 & 2.7E-02 &      1.0 \tabularnewline
%%                          & 1.0E-3 & 6.1E-07 &      1.0 & 2.6E-02 &      1.0 & 2.1E-06 &      1.1 & 5.6E-02 &      1.1 \tabularnewline
%% \multicolumn{6}{c}{} \tabularnewline
%% \multirow { 9}{*}{    $ L_d$ }& 2.0E-5 & 1.7E-11 &        - & 2.8E-08 &        - & 1.3E-08 &        - & 2.1E-06 &        - \tabularnewline
%%                          & 5.0E-5 & 1.0E-10 &      2.0 & 1.8E-07 &      2.0 & 3.1E-08 &      1.0 & 5.2E-06 &      1.0 \tabularnewline
%%                          & 1.0E-4 & 4.2E-10 &      2.0 & 7.5E-07 &      2.0 & 6.1E-08 &      1.0 & 1.0E-05 &      1.0 \tabularnewline
%%                          & 2.0E-4 & 1.7E-09 &      2.0 & 3.2E-06 &      2.1 & 1.2E-07 &      1.0 & 2.0E-05 &      1.0 \tabularnewline
%%                          & 5.0E-4 & 1.1E-08 &      2.0 & 2.3E-05 &      2.1 & 2.8E-07 &      0.9 & 5.4E-05 &      1.1 \tabularnewline
%%                          & 1.0E-3 & 4.4E-08 &      2.0 & 9.2E-05 &      2.0 & 5.0E-07 &      0.8 & 1.6E-04 &      1.5 \tabularnewline
%%                          & 1.0E-2 & 6.3E-06 &      2.2 & 4.8E-03 &      1.7 & 6.3E-06 &      1.1 & 9.0E-03 &      1.8 \tabularnewline
%%                          & 1.0E-1 & 1.1E-03 &      2.2 & 1.6E-01 &      1.5 & 1.1E-03 &      2.3 & 1.8E-01 &      1.3 \tabularnewline
%%                          & 1.0 & 6.0E-01 &      2.7 & 5.2E-01 &      0.5 & 6.0E-01 &      2.7 & 5.2E-01 &      0.5 \tabularnewline
%% \hline\hline
%% \end{tabular}
%% \end{center}
%% \end{table}
 

%% We also perform the time convergence study for ARS111 in Figure \figref{expo-ode-tconv-ars}.
%% ARS111-L and ARS111-J stand for ARS111 method with the constant linear operator \eqnref{linearop-const} 
%% and the dynamic Jacobian \eqnref{linearop-dynamic}, respectively.
%% ARS111-L shows the first-order convergence rate, 
%%     whereas ARS111-J shows the first-order convergence rate
%%   near $10^{-4}$ timestep size, but the second-order convergence rate 
%%   as loosen the timestep size.
%% This implies that the error associated with the fast modes starts to dominate as tighten the timestep size. 
%% We also notice that the difference of the phase error between ARS111-L and ARS111-J 
%% is relatively larger than that of the magnitude error. 
%% The same behavior is observed between ETD1-L and ETD1-J. 
%% The dynamic Jacobian $L_d$ significantly improves the phase error.
%% We tabulate the time convergence results in Table \tabref{expo-ode-tconv}.
%% We see that ETD1 solutions are more accurate than ARS111 solutions
%% with the small timestep sizes ($dt < 10^{-3}$).
%% This makes sense because the IMEX scheme is known to damp out the high-frequency modes in the system,
%% whereas exponential integrators exactly treat the fast modes. 
%% In particular, exponential integrators subdivide a timestep size $\triangle t$ into several sub-steps $\triangle t=\tau_1 + \tau_2  + \cdots$ and march the approximation step-by-step
%% similar to an explicit time integration method. 
%% Overall, exponential integrators are promising in the sense that it is not only accurate but also stable with a large timestep size. 


\subsection{Allen-Cahn equation}

In this section we consider the following Allen-Cahn equation:
\begin{align*}
% \eqnlab{pde-allen-eq}
 \dd{u}{t} 
  = \dd{}{x} \LRp{\kappa \dd{u}{x} } - \LRp{u^3 - u} \text{ in } \Omega,  
\end{align*}
with $\Omega=\LRc{x: x \in \LRp{-1,1} }$, the following smooth initial solution, 
%We choose a smooth initial condition,
\begin{align*}
    u(x,t=0) = 0.53 x + 0.47 \sin(-1.5\pi x)
\end{align*}
and a constant viscosity $\kappa=0.001$.
We impose Dirichlet boundary conditions, 
$u(-1,t) = -1$ and $u(1,t) = 1$. 


%-------------------------
% EXAMPLES FOR ALLEN-CAHN EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
  % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-Allen-smooth}
  % \figlab{pde-allen-ex-smooth}
    \subfigure[solutions]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Allen-smooth}
      \figlab{pde-allen-ex-smooth}
    }
    \subfigure[differences]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Allen-smooth-difference}
      \figlab{pde-allen-ex-smooth-difference}
    }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{(a) Smooth solutions and (b) their differences with RK4 for Allen-Cahn equation at $t=1$.
RK2 with $Cr_d=0.16$, EPI2 with $Cr_d=26.8$ and EPI2 with $Cr_d=56.7$ are simulated with
$k=4$ solution order and $N_e=80$ elements.
Dirichlet boundary conditions are imposed at $x=-1$ and $x=1$.}
    \figlab{pde-allen-smooth}
  \end{figure}
  
We perform the simulation for $t \in [0, 1]$ with  $k = 4$ solution
order and a uniform mesh with $N_e = 80$ elements.
We define the diffusion Courant number $Cr_d=\frac{\kappa dt}{(dx)^2}$ where 
$dx$ is the minimum distance between the interpolation nodes on $\Omega$. 
%\tanbui{is the mesh uniform or not? Please state it.}
The solution snapshots (at $t = 1$) for the second-order Runge-Kutta method (RK2)
with $Cr_d=0.16$ and EPI2 ($Cr_d=26.8$ and $Cr_d=56.7$) are shown 
in Figure \figref{pde-allen-smooth}.
% \tanbui{I think we should put the curves on the same figure with
%   different colors/symbols to clearly see the similarity of the
%   solutions that we claim. Also, the plot at $t=0$ is not meaningful/necessary
%   but makes the figures busy/confused. Please remove the initial
%   condition plots, and do the same for the
%   other numerical examples below.}
Both the EPI2 solutions with $Cr_d=26.8$ and $Cr_d=56.7$ produce a similar result to the RK2 counterpart even with two orders of magnitude larger timestep size. 
Compared to the EPI2 solution with $Cr_d=26.8$, we see that the EPI2 solution with $Cr_d=56.7$ has a larger difference from the RK4 due to the time truncation error. 
We conduct a temporal convergence study for EPI2 and EXPRB32\footnote{
EXPRB32  \cite{hochbruck2010exponential} is the third-order two-stage method,
\begin{align*}
  q^{(2)} &= q^n + \dt \varphi_1(L \dt) R^n,\\
  q^{n+1} &= q^n + \dt \varphi_1(L \dt) R^n
                 + \dt \varphi_3(L \dt) 2 D_{n,2},
  %q^{n+1} = q^n  + \dt \varphi_1(L \dt) R^n + \frac{2}{3}\dt \varphi_2 (L \dt) D_{n,2},
\end{align*}
where $D_{n,2}:= \LRp{R(q^{(2)}) - L q^{(2)}} - \LRp{R(q^{n}) - L q^n}$.
%Since this method requires both $q^0$ and $q^1$ solutions for advancing in time, 
%we compute $q^1$ using EPI2 method, in which the local error is the third-order, 
%so that the global error of EPI3 becomes the third-order. \tanbui{Is
%  the statement true? I thought that global error is always one-order
%  less than the local error?}
} by taking 
the RK4 solution (with $dt=2\times 10^{-5}$, $k=10$ and $N_e=80$)
as ``the ground truth'' solution.
As expected, the theoretical convergence rates (second and third orders) are observed for EPI2 and EXPRB32 
in Table \tabref{expo-allen-tconv-smooth}.

\begin{table}[t]
\caption{A smooth function for Allen-Cahn equation:
time convergence study is conducted with $k=4$ solution order and $N_e=80$ elements. 
The expected second- and third-order convergence rates are
observed for EPI2
and EXPRB32, respectively.}
\tablab{expo-allen-tconv-smooth}
\begin{center}
%\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
\begin{tabular}{cc||cc|cc}
\hline
\multirow{2}{*}{$dt$} 
& \multirow{2}{*}{$Cr$}
& \multicolumn{2}{c|}{ EPI2 } 
& \multicolumn{2}{c}{ EXPRB32 } \tabularnewline
  &  &  error & order & error & order \tabularnewline
\hline\hline
  0.50 & 115.83 & 1.179E-02 &      $-$ &       1.636E-03 &      $-$ \tabularnewline 
  0.10 & 23.17  & 2.993E-03 &    1.978 &       1.462E-04 &    3.485 \tabularnewline 
  0.05 & 11.58  & 4.898E-04 &    1.975 &       7.593E-06 &    3.228 \tabularnewline 
  0.01 & 2.32   & 1.237E-04 &    1.986 &       8.869E-07 &    3.098 \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}




\subsection{Viscous Burgers equation}

We consider a steady-state manufactured solution,
$$ u(x,t) = \sin(x^2) x (x-1) $$ 
by adding a source term to \eqnref{pde-burgers-eq}. 
We perform 
a spatial convergence study with Lax-Friedrich (LF) flux and entropy flux (EF),
where we take $\sigma=0$ and $\sigma=3\times 10^{-4}$. 
We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
The error is measured at $t=0.01$ and the results are summarized in Table \tabref{expo-burgers-sconv-mms}.
% with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.
In general, the convergence results show similar behavior.
All the error levels are similar to each other.
We also see that the rates of convergence with LF and EF are not optimal for odd order,
e.g., both the rates for $k=3$ are $\mc{O}(h^3)$, but optimal for even order. 
This behavior is well-known for parabolic equations with a central flux \cite{cockburn1998local}.
However, for the case of EF $(\sigma=3\times 10^{-4})$,  
we observe that the rate of convergence tends to increase 
due to the presence of the non-zero jump term.  
These results support our theoretical results. 

In the following two examples: smooth solution and shock solution, 
we use EF flux for EPI2 and EXPRB32. 
% \begin{table}[t]
% \caption{A smooth solution for viscous Burgers equation:
% a spatial convergence study is conducted with Lax-Friedrich (LF) flux and entropy flux (EF). 
% We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
% The error is measured at $t=0.01$ with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.}
% \tablab{expo-burgers-sconv-smooth}
% \begin{center}
% \begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}}
% \hline
% \multirow{2}{*}{}%$k=16$} 
%   & \multirow{2}{*}{$h$}  
%   & \multicolumn{2}{c|}{$LF$}   
%   & \multicolumn{2}{c|}{$EF$}   
%   \tabularnewline
%   &    &  error & order &  error & order       \tabularnewline
% \hline\hline
% \multirow { 4}{*}{   k=1}&  0.050 & 7.047E-03 &      $-$ & 7.116E-03 &      $-$ \tabularnewline
%                          &  0.030 & 2.092E-03 &    1.752 & 2.272E-03 &    1.647 \tabularnewline
%                          &  0.010 & 6.967E-04 &    1.586 & 9.015E-04 &    1.334 \tabularnewline
%                          &  0.005 & 2.646E-04 &    1.397 & 4.175E-04 &    1.111 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=2}&  0.050 & 3.013E-04 &      $-$ & 3.038E-04 &      $-$ \tabularnewline
%                          &  0.030 & 3.373E-05 &    3.159 & 3.385E-05 &    3.166 \tabularnewline
%                          &  0.010 & 3.985E-06 &    3.082 & 3.992E-06 &    3.084 \tabularnewline
%                          &  0.005 & 4.907E-07 &    3.022 & 4.912E-07 &    3.023 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=3}&  0.050 & 3.252E-05 &      $-$ & 3.284E-05 &      $-$ \tabularnewline
%                          &  0.030 & 3.750E-06 &    3.116 & 3.876E-06 &    3.083 \tabularnewline
%                          &  0.010 & 4.629E-07 &    3.018 & 4.775E-07 &    3.021 \tabularnewline
%                          &  0.005 & 5.739E-08 &    3.012 & 5.944E-08 &    3.006 \tabularnewline
% \multicolumn{6}{c}{} \tabularnewline
% \multirow { 4}{*}{   k=4}&  0.050 & 1.599E-06 &      $-$ & 1.602E-06 &      $-$ \tabularnewline
%                          &  0.030 & 5.413E-08 &    4.884 & 5.791E-08 &    4.790 \tabularnewline
%                          &  0.010 & 1.486E-09 &    5.187 & 1.691E-09 &    5.098 \tabularnewline
%                          &  0.005 & 4.362E-11 &    5.091 & 5.183E-11 &    5.028 \tabularnewline
% % \multicolumn{6}{c}{} %\tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}
\begin{table}[t]
\caption{A manufactured solution for viscous Burgers equation:
a spatial convergence study is conducted with Lax-Friedrich (LF) flux and
 entropy flux (EF). 
We use EXPRB32 scheme with $dt=\LRc{8,4,2,1}\times 0.00005$ for $N_e=\LRc{20,40,80,160}$ elements.
% The error is measured at $t=0.01$ with the RK4 solution of 
%  (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=160$) as a reference solution.}
}
\tablab{expo-burgers-sconv-mms}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
\hline
\multirow{2}{*}{ } 
  & \multirow{2}{*}{$h$}  
  & \multicolumn{2}{c|}{$LF$}   
  & \multicolumn{2}{c|}{$EF$ ($\sigma=3\times 10^{-4}$)}   
  & \multicolumn{2}{c|}{$EF$ ($\sigma=0$)}   
  \tabularnewline
  &    &  error & order &  error & order &  error & order       \tabularnewline
\hline\hline
\multirow { 4}{*}{   k=1 }&  0.05 & 4.093E-04 &      $-$ & 4.096E-04 &      $-$ & 4.097E-04 &      $-$ \tabularnewline
                         &  0.03 & 1.223E-04 &    1.743 & 1.225E-04 &    1.741 & 1.232E-04 &    1.734 \tabularnewline
                         &  0.01 & 4.494E-05 &    1.445 & 4.378E-05 &    1.484 & 4.620E-05 &    1.415 \tabularnewline
                         &  0.01 & 1.937E-05 &    1.214 & 1.562E-05 &    1.487 & 2.074E-05 &    1.155 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{   k=2 }&  0.05 & 2.630E-06 &      $-$ & 2.632E-06 &      $-$ & 2.632E-06 &      $-$ \tabularnewline
                         &  0.03 & 3.210E-07 &    3.034 & 3.213E-07 &    3.034 & 3.213E-07 &    3.034 \tabularnewline
                         &  0.01 & 3.966E-08 &    3.017 & 3.952E-08 &    3.023 & 3.952E-08 &    3.023 \tabularnewline
                         &  0.01 & 4.916E-09 &    3.012 & 4.833E-09 &    3.032 & 4.833E-09 &    3.032 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=3}&  0.05 & 1.431E-07 &      $-$ & 1.459E-07 &      $-$ & 1.471E-07 &      $-$ \tabularnewline
                         &  0.03 & 1.709E-08 &    3.066 & 1.742E-08 &    3.066 & 1.819E-08 &    3.015 \tabularnewline
                         &  0.01 & 2.003E-09 &    3.093 & 1.876E-09 &    3.215 & 2.268E-09 &    3.003 \tabularnewline
                         &  0.01 & 2.251E-10 &    3.154 & 1.441E-10 &    3.703 & 2.834E-10 &    3.001 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{   k=4}&  0.05 & 5.946E-10 &      $-$ & 5.991E-10 &      $-$ & 6.013E-10 &      $-$ \tabularnewline
                         &  0.03 & 1.827E-11 &    5.024 & 1.837E-11 &    5.027 & 1.860E-11 &    5.015 \tabularnewline
                         &  0.01 & 5.626E-13 &    5.021 & 5.590E-13 &    5.039 & 5.796E-13 &    5.004 \tabularnewline
                         &  0.01 & 1.730E-14 &    5.023 & 1.690E-14 &    5.048 & 1.810E-14 &    5.001 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}
%We test two examples to the viscous Burgers equation in Figure \figref{pde-burgers-ex}. 
%The first example, shown in Figure \figref{pde-burgers-ex}(a), is a smooth Gaussian profile develops sharp gradient as time goes on, $t\in[0,2]$. The initial condition is given as 
%\begin{align}
%    u(x,t) = e^{-2x^2},
%\end{align}
%where $x\in [-1,1]$, $\kappa=0.01$. Periodic boundary condition is imposed. 
We take the following smooth initial condition, 
\begin{align}
  \eqnlab{burgers-smooth}
    u(x,t=0) = \sin^3(2\pi x) (1-x)^{\frac{3}{2}}, %\quad x \in [0,1],
\end{align}
homogeneous boundary condition, and viscosity $\kappa=0.03$.
We perform the simulation for $t \in [0, 1]$ with $k = 4$ solution order and $N_e = 40$ elements.
The smooth initial profile is spread out due to the viscosity as time passes by.
Figure \figref{pde-burgers-smooth} shows the snapshots at $t=1$
for RK2 $(Cr_d=0.16)$ and EPI2 $(Cr_d=161.0, Cr_d=804.9)$. 
% and $t=1$ for RK4 integrator with $Cr=0.32$ and EPI2 integrator with $Cr=319.98$. 
% As can be seen, the smooth initial profile is spread out due to the viscosity.
%and the solutions from both methods  are in good agreement with each other.
Compared to RK2, EPI2 $(Cr_d=161.0)$ uses one-hundred times larger timestep size but
produces a comparable result.
Even with five-hundred times larger timestep size, 
EPI2 $(Cr_d=804.9)$ solution captures the general trend of the evolution.
% \tanbui{again, I think it is much more informative to plot them on the
% same figure. Also, in this kind of comparison, the stability is very
% important to point out for EI. Is $Cr=0.32$ the stability limit for RK4?}

%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[solutions ]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-all}
      \figlab{pde-burgers-ex-smooth-all}
    }
    \subfigure[differences ]{
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-difference}
      \figlab{pde-burgers-ex-smooth-difference}
    }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{(a) Smooth solutions and (b) their differences with RK4 for viscous Burgers equation at $t=1$.
RK2 with $Cr_d=0.16$, EPI2 with $Cr_d=161.0$ and EPI2 with $Cr_d=804.9$ are used with
$k=4$ solution order and $N_e=40$ elements.
Homogeneous boundary conditions are imposed at $x=0$ and $x=1$.}
%     \caption{A smooth solution to the viscous Burgers equation is simulated for $t \in [0,1]$: 
% (a) RK4 with $Cr=0.32$ and (b) EPI2 with $Cr=321.98$ are used on the grid of $k=4$ and $N_e=40$.
% Homogeneous boundary conditions are imposed at $x=0$ and $x=1$.}
    \figlab{pde-burgers-smooth}
  \end{figure}


To measure the temporal convergence of EPI2 and EXPRB32,
%\footnote{
%EPI3 \cite{tokman2006efficient} is the third-order multi-step method,
%\begin{align}
%  \qb^{n+1} = \qb^n  + \dt \varphi_1(L_d \dt) R^n + \frac{2}{3}\dt \varphi_2 (L_d \dt) D_{n,n-1},
%\end{align}
%where $D_{n,n-1}:= \LRp{R(\qb^{n-1}) - L_d \qb^{n-1}} - \LRp{R(\qb^{n}) - L_d \qb^n}$.
%Since this method requires both $\qb^0$ and $\qb^1$ solutions for advancing in time, 
%we compute $\qb^1$ using EPI2 method, in which the local error is the third-order, 
%so that the global error for EPI3 becomes the third-order accurate. 
%},
we take the RK4 solution (with $dt=5\times 10^{-6}$,  $k=10$, and
$N_e=40$) as a ground truth.
In Table \tabref{expo-burgers-tconv-smooth}, we again observe the second- and third-order convergence rates
for EPI2 and EXPRB32, respectively. 

\begin{table}[t]
\caption{A smooth solution for viscous Burgers equation:
a time convergence study is conducted with $k=4$ solution order and $N_e=40$ elements. 
We observe the second- and the third-order convergence rates for EPI2
and EXPRB32, respectively.}
\tablab{expo-burgers-tconv-smooth}
\begin{center}
%\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
\begin{tabular}{cc||cc|cc}
\hline
\multirow{2}{*}{$dt$} 
& \multirow{2}{*}{$Cr$} 
& \multicolumn{2}{c|}{ EPI2 } 
& \multicolumn{2}{c}{ EXPRB32 } \tabularnewline
  &  &  error & order & error & order \tabularnewline
\hline\hline
  % LF flux
  % 0.50 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  % 0.25 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  % 0.10 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  % 0.05 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.880 \tabularnewline
  % 0.01 &  16.1 &   4.944E-06 &    2.037 &       1.065E-07 &    2.986 \tabularnewline
  % entropy flux
  % 0.5000 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  % 0.2500 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  % 0.1000 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  % 0.0500 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.880 \tabularnewline
  % 0.0100 &  16.1 &   4.944E-06 &    2.037 &       1.068E-07 &    2.983 \tabularnewline  
  % entropy flux with sigma = kappa/100
  0.5000 & 804.9 &   1.171E-02 &      $-$ &       5.272E-03 &      $-$ \tabularnewline
  0.2500 & 402.5 &   3.303E-03 &    1.827 &       1.077E-03 &    2.292 \tabularnewline
  0.1000 & 161.0 &   5.411E-04 &    1.974 &       9.575E-05 &    2.641 \tabularnewline
  0.0500 &  80.5 &   1.312E-04 &    2.044 &       1.300E-05 &    2.881 \tabularnewline
  0.0100 &  16.1 &   4.943E-06 &    2.037 &       1.042E-07 &    2.999 \tabularnewline  
\hline\hline
\end{tabular}
\end{center}
\end{table} 



%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[solutions]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-all}
      \figlab{pde-burgers-ex-stationary-shock-all}
    }
    \subfigure[differences]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-difference}
      \figlab{pde-burgers-ex-stationary-shock-difference}
    }
    % \subfigure[EPI2 with $Cr=6.71$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
    % }
    % \subfigure[EPI2 with $Cr=13.42$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
    % }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{
    (a) Shock solutions to the viscous Burgers equation at $t=1$, and 
    (b) their differences with RK4.
    EF ($\sigma=10^{-5}$) flux is used for EPI2 and EXPRB32 
    with solution order $k=4$ and $N_e=40$ elements.}
    \figlab{pde-burgers-stationary-shock}
  \end{figure} 

% We have seen that Exponential DG methods work well for the smooth
% solution in \eqnref{burgers-smooth}.
% \tanbui{DG is not useful here if we don't demonstrate correct order of
% convergence in both time and space. So please also show the
% convergence rate for space.}
% \shinhoo{we don't have exact solution for this problem. I will show the spatial convergence in 2D Euler equation}.
Next, we consider a solution with a steep gradient.
A stationary shock evolves in time 
due to the nonlinear convection term \eqnref{pde-burgers-eq}.
The initial condition is given as
\begin{align*}
  u(x,t=0) = \sin(2\pi x)
\end{align*}
for $x \in [0,1]$ with homogeneous boundary conditions.
We take $\kappa=0.001$ and 
 perform the simulation for $t \in [0, 1]$ with $k = 4$ and $N_e = 40$.
 In Figure \figref{pde-burgers-stationary-shock}, 
 we compare EPI2 and EXPRB32 solutions with the RK2 solution.
 We take the RK4 solution 
  (with $dt=1\times 10^{-4}$,  $k=10$, and
$N_e=40$) as a reference, and plot the difference. 
We use EF ($\sigma=10^{-5}$) flux for EPI2 and EXPRB32 and LF flux for RK2 and RK4
% \footnote{
% We numerically observe that the difference between the results with LF and EF fluxes for EPI2 and EXPRB32 is within $\mc{O}(10^{-3})$ in this example, hence omit the EPI2 and EXPRB32 results with LF flux in Figure \figref{pde-burgers-stationary-shock}.  
% }
.

We see that EPI2 $(Cr_d=10.73)$ has an overshoot
% slighly departs from the reference solution 
near the shock interface.
% compared to others.
This is due to the time truncation error associated with the nonlinear convection term. 
To amend this issue,
 we can either shrink a timestep size or employ a high-order time integrator. 
We see that EPI2 $(Cr_d=5.36)$ and EXPRB32 $(Cr_d=10.73)$ become closer to the reference solution near the interface. 
  

% We observe the overshoot near the shock interface for EPI2 $(Cr_d=13.42)$.  
% This is due to the time truncation error associated with the nonlinear convection term. 
% To amend this issue,
%  we can either shrink a timestep size or employ a high-order time integrator. 
% We see that the solutions of EPI2 $(Cr_d=6.71)$ and EXPRB32 $(Cr_d=13.42)$ do not suffer from the overshoot near the interface in Figure \figref{pde-burgers-shock}.

%  %-------------------------
% % EXAMPLES FOR BURGERS EQ.
% %-------------------------
% \begin{figure}[h!t!b!]
%     \centering
% %    \subfigure[Gaussian]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
% %      \figlab{pde-burgers-ex-Gaussian}
% %    }
%     \subfigure[solutions]{
%       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all2}      
%       \figlab{pde-burgers-ex-shock-all}
%     }
%     \subfigure[differences]{
%       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
%       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference2}
%       \figlab{pde-burgers-ex-shock-difference}
%     }
%     % \subfigure[EPI2 with $Cr=6.71$]{
%     %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
%     %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
%     % }
%     % \subfigure[EPI2 with $Cr=13.42$]{
%     %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
%     %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
%     % }
% %    \subfigure[Tanh]{
% %      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
% %      \figlab{pde-burgers-ex-Tanh}
% %    }    
%     %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
%     \caption{
%     (a) Shock solutions to the viscous Burgers equation at $t=2$, and 
%     (b) their differences with RK4.
%     RK2 with $Cr_d=0.13$, EPI2 with $Cr_d=6.71$ and EPI2 with $Cr_d=13.42$
%  are used with solution order $k=4$ and $N_e=40$ elements.}
%     \figlab{pde-burgers-shock}
%   \end{figure} 

%  The initial condition is given as
% \begin{align*}
%   u(x,t=0) = e^{-2x^2}.
% \end{align*}
% We take $\kappa=0.01$ and $x \in [-1,1]$. 
% We perform the simulation for $t \in [0, 2]$ with $k = 4$ and $N_e = 40$.
% Periodic boundary condition is imposed at $x=-1$ and $x=1$. 
% This is a challenging problem because the nonlinear convection term in
% \eqnref{pde-burgers-eq} develops a shock, i.e., solution with a steep gradient.
% %
% %frequently update Jacobian,
% %which eventually prevents a large timestep size.
% %\tanbui{I thought the opposite: updating the Jacobian allows larger
% %  stepsize then keeping it fixed?}
% Figure \figref{pde-burgers-shock} shows the solutions at
%  $t=2$ for RK2 $(Cr_d=0.13)$, EPI2 ($Cr_d=6.71$ and $Cr_d=13.42$) and EXPRB32 ($Cr_d=13.42)$. 
%  %  A shock is developed as it travels with a small dissipation.
%  % \tanbui{putting the figures together in the same plot is
%  %  more informative. Can you get and use a result with RK4 as the
%  %  reference solution to compare with these two solutions?}
% We observe the overshoot near the shock interface for EPI2 $(Cr_d=13.42)$.  
% This is due to the time truncation error associated with the nonlinear convection term. 
% To amend this issue,
%  we can either shrink a timestep size or employ a high-order time integrator. 
% We see that the solutions of EPI2 $(Cr_d=6.71)$ and EXPRB32 $(Cr_d=13.42)$ do not suffer from the overshoot near the interface in Figure \figref{pde-burgers-shock}.
% % Compared to Figure \figref{pde-burgers-shock}a, 
% % Figure \figref{pde-burgers-shock}b shows the overshoot near the shock
% % interface. 
% % To amend this issue, we may employ various techniques such as strong-stability preserving (SSP) methods \cite{gottlieb2005high} and non-oscillatory schemes \cite{gottlieb2006recovering}. However, since it needs a comprehensive investigation, 
% % we will pose the issue in future work. 
% %However, it is not clear how to determine the update frequency for the Jacobian.
% %As an alternative, we may employ strong-stability preserving (SSP) type method \cite{gottlieb2005high} 
% %or reconstruction \cite{gottlieb2006recovering}, but thorough investigation is needed. 
% %We will tackle this issue in future work. 
% %

 
%EPI2 time integrators with 
%As shown in Figure \figref{pde-burgers-ex}(b),
%$\tanh$ shape is translated from left to right. 
%The exact solution is given as 
%\begin{align}
%    u(x,t) = 1 -\tanh \LRp{\frac{x+0.5-t}{2\kappa}}.
%\end{align}
%We impose exact boundary condition at both the ends. 

We also perform the same simulations above for EPI2 and EXPRB32 with Lax-Friedrich flux.
The results are summarized in Figure \figref{pde-burgers-fluxdifference}.
The differences between the results with Lax-Friedrich and entropy fluxes are 
orders of $\mc{O}(10^{-8})$ for the smooth solution case and $\mc{O}(10^{-3})$ for the shock solution case.
Considering these small differences between two fluxes %that these differences are not significant and 
and the simplicity of Lax-Friedrich flux, we use Lax-Friedrich flux for Euler equations 
in the following examples.

%-------------------------
% EXAMPLES FOR BURGERS EQ.
%-------------------------
\begin{figure}[h!t!b!]
    \centering
%    \subfigure[Gaussian]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Gaussian}
%      \figlab{pde-burgers-ex-Gaussian}
%    }
    \subfigure[smooth case]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-smooth-difference-flux-difference}      
      \figlab{pde-burgers-ex-smooth-fluxdiff}
    }
    \subfigure[shock case]{
      % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-stationary-shock-flux-difference}
      \figlab{pde-burgers-ex-sShock-fluxdiff}
    }
    % \subfigure[EPI2 with $Cr=6.71$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx1}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx1}
    % }
    % \subfigure[EPI2 with $Cr=13.42$]{
    %   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Gaussian-periodic-epi2-dtx2}
    %   \figlab{pde-burgers-ex-shock-epi2-dtx2}
    % }
%    \subfigure[Tanh]{
%      \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-Bugers-ex-Tanh} 
%      \figlab{pde-burgers-ex-Tanh}
%    }    
    %\caption{We illustrate three examples to the viscous Burgers` equation: (a) Gaussian shape with periodic boundary condition, (b) Sine shape with homogeneous boundary condition and (c) Tanh shape with nonhomogeneous boundary condition.}
    \caption{
    The differences between the results with Lax-Friedrich flux and with entropy flux are plotted: (a) the smooth solution case in Figure \figref{pde-burgers-smooth} and 
    (b) the shock solution case in Figure \figref{pde-burgers-stationary-shock}.
    }
    \figlab{pde-burgers-fluxdifference}
\end{figure} 






\subsection{Euler equations: Isentropic vortex translation}

We study the isentropic vortex example \cite{zhou2003high}, 
where small perturbations of a vortex are added to the uniform mean flow 
and translated without changing its shape. 
The superposed flow is given as 
\begin{align*}
u &= u_\infty - \frac{\lambda}{2\pi} \tilde{y} e^{\alpha \LRp{1-r^2}/2}, \\
v & = v_\infty + \frac{\lambda}{2\pi}\tilde{x} e^{\alpha\LRp{1-r^2}/2}, \\
T & = T_\infty - \LRp{\frac{1}{2\alpha c_p} } \LRp{\frac{\lambda}{2\pi}}^2 e^{\alpha\LRp{1-r^2}},
% T & = T_\infty - T_\infty\LRp{\frac{\gamma-1}{2\alpha a_\infty^2} } \LRp{\frac{\lambda}{2\pi}}^2 e^{\alpha\LRp{1-r^2}},
\end{align*}
where $r = \norm{\xb - \xb_c - \ub_\infty t}$,
$\tilde{x}=x - x_c - u_\infty t$,
$\tilde{y}=y - y_c - v_\infty t$,
$\ub_\infty=(u_\infty,v_\infty)$ the velocity of the mean flow,
$\xb_c=(5,0)$, $c_p$ specific heat ratio at constant pressure 
and $\lambda$ the vortex strength. 
The mean flows are set to be $(u_\infty,v_\infty,\rho_\infty,T_\infty,\pres_\infty) = (0.2,0,1,1,1)$.
We take $\alpha=2$, $\gamma=1.4$, $\lambda=0.05$ and 
$c_p=\frac{\gamma}{\gamma-1}$.
% and the perturbations are given as 
% \begin{align*}
% u^\prime & = - \frac{\lambda}{2\pi} e^{\LRp{1-r^2}}(y - y_c), \\
% v^\prime & = + \frac{\lambda}{2\pi} e^{\LRp{1-r^2}}(x - x_c), \\
% T^\prime & = - \frac{\LRp{\gamma - 1}\lambda^2}{16\gamma\pi^2} e^{2\LRp{1-r^2}}
% \end{align*}
The exact solutions are generated from the isentropic relation\footnote{
$$\frac{\rho}{\rho_\infty} = \LRp{\frac{T}{T_\infty}}^{\frac{1}{\gamma-1}}
=\LRp{\frac{\pres}{\pres_\infty}}^{\frac{1}{\gamma}}
$$
}. 
%$$ \rho = \LRp{T_\infty + T^\prime}^{1/(\gamma-1)}. $$
%We take $\gamma=1.4$ and 
The domain is $\Omega = \LRp{0,10} \times \LRp{-5,5}$ and 
periodic boundary conditions are applied to all directions. 
For a three-dimensional simulation, we take the zero vertical velocity, $w = 0$ and extrude domain vertically, $\Omega = \LRp{0,10} \times \LRp{-5,5} \times \LRp{0,1}$. 

We perform the simulation for $t\in [0,15]$ 
with $k=12$ and $N_e=256$ in Figure \figref{expo-pde-euler2d-vortex}.
We increase the timestep size of EPI2 until it shows a notable time truncation error. 
Compared to the EPI2 $(Cr=42.75)$ solution in the left panel, 
the EPI2 $(Cr=85.56)$ solution in the center panel 
shows the oscillatory solution in the mean flows,
 which starts from the edge of the vortex and propagates the entire domain.
 Due to the hyperbolic nature of the Euler system, 
 the oscillation remains throughout the simulation, 
 but the shape of the vortex and its movement are still comparable to 
 the one with EPI2 $(Cr=42.75)$.
To alleviate the oscillation, we can employ a high-order time integrator.
For example, the third-order EXPRB32 $(Cr=85.56)$ in the right panel significantly improves the solution accuracy in Figure \figref{expo-pde-euler2d-vortex}.
% This is 
% EPI2 and EXPRB42 can use one-hundred times larger timestep size than RK4, 
% and still capture the vortex movement. 
% However, the solution of EPI2 degrades
% \tanbui{perhaps we should make the statement more precise. I see that
%   the solution is osillatory, though the magnitude is similar. Is this
% what you meant by ``degrade''?}
% due to the time truncation error. % in Figure \figref{expo-pde-euler2d-vortex}(b). %The artificial 

% For time discretization, 
% RK4 with $Cr=0.86$, 
% %EPI2 with $Cr=8.56$ and 
% EPI2 with $Cr=85.56$ and 
% EXPRB42 \cite{hochbruck2010exponential} with $Cr=85.56$
% \tanbui{a few words, put it in parentheses or footnote,introducing EXPRB42 are necessary here}
% are chosen. 
% As can be seen in Figure \figref{expo-pde-euler2d-vortex}(b) 
% and Figure \figref{expo-pde-euler2d-vortex}(c), 
% EPI2 and EXPRB42 can use one-hundred times larger timestep size than RK4, 
% and still capture the vortex movement. 
% However, the solution of EPI2 degrades
% \tanbui{perhaps we should make the statement more precise. I see that
%   the solution is osillatory, though the magnitude is similar. Is this
% what you meant by ``degrade''?}
% due to the time truncation error. % in Figure \figref{expo-pde-euler2d-vortex}(b). %The artificial oscillation is caused by the time truncation error for EPI2.
%This is a consequence of the time trunction error. 
%Since Euler system is nonlinear, exponential integrators are not free from the time truncation error.  
%the 
%have the time truncation error. This is why we observe the oscillation in Figure \figref{expo-pde-euler2d-vortex}(b). However, the time truncation error is significantly reduced 
% To alleviate the error, we can use a high-order time integration method.
% For example, in Figure \figref{expo-pde-euler2d-vortex}(c), 
% the time truncation error of EXPRB42
% \tanbui{what is the order of EXPRB42? what if we use smaller Cr
%   (i.e. do we still see the similar degrade)? Perhaps providing
%   solution with different Cr's (similar to our IMEX paper) is
%   informative and provides a more complete picture of the behavior of
%   the EPI2 method. It is also weird that EXPRB42 comes out of
%   blue. You introduced EPI3 before, why not using it here? As a
%   reader/reviewer, I would raise a lot concerns about this
%   inconsistency of the manuscript.}
% is significantly reduced compared to the EPI2 counterpart. 


%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
\centering
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t5}
  % \figlab{pde-euler2d-epi2-Cr42-t5}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t5} 
  % \figlab{pde-euler2d-epi2-Cr85-t5}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t5}
   % \figlab{pde-euler2d-exprb32-Cr85-t5}
   \\
% }\\
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t10}
  % \figlab{pde-euler2d-epi2-Cr42-t10}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t10} 
  % \figlab{pde-euler2d-epi2-Cr85-t10}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t10}
   % \figlab{pde-euler2d-exprb32-Cr85-t10}
   \\
% }\\
% \subfigure[EPI2 {\tiny $(Cr=42.75)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr42-t15}
  % \figlab{pde-euler2d-epi2-Cr42-t15}
% }
% \subfigure[EPI2 {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-epi2-Cr85-t15} 
  % \figlab{pde-euler2d-epi2-Cr85-t15}
% }    
% \subfigure[{\tiny EXPRB32} {\tiny $(Cr=85.56)$}]{
% \subfigure[]{
   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-exprb32-Cr85-t15}
   % \figlab{pde-euler2d-exprb32-Cr85-t15}
% }
% \subfigure[RK4 with $Cr=0.86$]{
%   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-rk4}
%   \figlab{pde-euler2d-rk4}
% }
% %\subfigure[EPI2 with $Cr=8.56$]{
% %  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-epi2-10x} 
% % % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-10x} 
% %  \figlab{pde-euler2d-epi2-10x}
% %}
% \subfigure[EPI2 with $Cr=85.56$]{
%   \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-epi2-100x} 
%   %\includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-100x} 
%   \figlab{pde-euler2d-epi2-100x}
% }    
% \subfigure[{\tiny EXPRB42} with $Cr=85.56$]{
%    \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-100x}
%    \figlab{pde-euler2d-exprb42-100x}
% }
\caption{Isentropic vortex example to the two-dimensional Euler equations: 
translating density fields for EPI2 ($Cr=42.75$, left), EPI2 ($Cr=85.56$, center) and EXPRB32 ($Cr=85.56$, right) at times $t=5$ (top), $t=10$ (middle) and $t=15$ (bottom).}
\figlab{expo-pde-euler2d-vortex}
\end{figure}



%\begin{table}[t]
%\caption{Isentropic vortex in two-dimensions: 
%time convergence study is conducted with $k=16$ solution order and $N_e=256$ elements. We observe the second-order convergence rate for EPI2 as expected.}
%\tablab{expo-euler2d-tconv-isentropic}
%\begin{center}
%\begin{tabular}{*{1}{c}||c|cc|cc|cc|c}
%\hline
%    & $Cr$ 
%& {\small $ \norm{\rho - \rho^e}_2$} & rate
%& {\small $ \norm{\rho {\bf u} - \rho \ub^e}_2$} & rate 
%& {\small $\small \norm{\rho E - \rho E^e}_2 $} & rate &  wc $[s]$ \tabularnewline
%\hline\hline
%\multirow { 6}{*}{  {\small EPI2} }& 71.4 & 2.89E-07 &        - & 6.18E-07 &        - & 1.02E-06 &        - &     75.4 \tabularnewline
%                         & 35.7 & 8.75E-08 &    1.73 & 1.26E-07 &    2.30 & 3.08E-07 &    1.73 &     43.9 \tabularnewline
%                         & 14.3 & 1.52E-08 &    1.91 & 1.82E-08 &    2.11 & 5.34E-08 &    1.91 &     37.0 \tabularnewline
%                         &  7.1 & 3.88E-09 &    1.97 & 4.43E-09 &    2.04 & 1.37E-08 &    1.97 &     38.8 \tabularnewline
%                         &  1.4 & 1.58E-10 &    1.99 & 1.74E-10 &    2.01 & 5.57E-10 &    1.99 &    108.1 \tabularnewline
%                         &  0.7 & 3.96E-11 &    2.00 & 4.33E-11 &    2.00 & 1.40E-10 &    2.00 &    230.8 \tabularnewline
%\multicolumn{9}{c}{} \tabularnewline
%\multirow { 2}{*}{   { \small RK4} }&  0.7 & 1.44E-13 &        - & 1.24E-12 &        - & 6.26E-14 &        - &     35.5 \tabularnewline
%                         &  0.4 & 1.53E-13 &   -0.10 & 1.24E-12 &    0.00 & 7.77E-14 &   -0.31 &     78.1 \tabularnewline
%\hline\hline
%\end{tabular}
%\end{center}
%\end{table}



To examine the error growth rate, 
time convergence studies are conducted with $k=\LRc{8,16}$ for $t\in[0,1]$ on a uniform mesh and a non-uniform mesh in Figure \figref{expo-pde-euler2d-mesh}.
%Here, we take the Krylov subspace size $m$ from the previous time step as a first guess for the adaptive Krylov subspace method \cite{gaudreault2018kiops} at the current time step. 
To verify the high-order accuracy in time, 
we take the second, the third, and the fourth-order exponential integrators:
EPI2, EXPRB32, and EXPRB42
\footnote{
EXPRB42  \cite{luan2017fourth} is the fourth-order two-stage method,
\begin{align*}
  q^{(2)} &= q^n + \frac{3}{4} \dt \varphi_1 \LRp{ \frac{3}{4} L \dt } R^n,\\
  q^{n+1} &= q^n + \dt \varphi_1(L \dt) R^n
                 + \frac{32}{9} \dt \varphi_3 \LRp{ L \dt } D_{n,2},
  %q^{n+1} = q^n  + \dt \varphi_1(L \dt) R^n + \frac{2}{3}\dt \varphi_2 (L \dt) D_{n,2},
\end{align*}
where $D_{n,2}:= \LRp{R(q^{(2)}) - L q^{(2)}} - \LRp{R(q^{n}) - L q^n}$.
}
.
We compare Exponential DG methods with IMEX DG and RKDG \cite{shu1988total} methods. 
In particular, we take the second-order, ARS232 \cite{ascher1997implicit} and the third-order, ARS443 \cite{ascher1997implicit} schemes without any preconditioner. 
The results for $\rho$ on a uniform mesh are summarized in 
Figure \figref{expo-euler-isentropic-tconv-uni-p16} 
and Figure \figref{expo-euler-isentropic-tconv-uni-p8}.
% Also, we do not consider the fourth-order IMEX methods because 
% the second and the third order IMEX schemes  
% have already shown its relative performance 

In Figure \figref{expo-euler-isentropic-tconv-uni-p16}(a),
 we observe 
 that the RK2 solution converges to the true solution with the second-order accuracy, 
 and the high-order RK (RK3 and RK4) solutions have reached the saturated error level at 
 $\mc{O}(10^{-13})$, 
 where the spatial discretization error starts to dominate.
We also see that Exponential DG (EPI2, EXPRB32, EXPRB42) and IMEX DG (ARS232 and ARS443) methods show the theoretical convergence rates for a wide range of time stepsizes. %Courant number. % This is a very
                                %attractive feature compared to the
                                %IMEX scheme.
This is attractive because that Exponential DG and IMEX DG supports a high-order solution in time, 
and overcomes the timestep size restriction 
the explicit RKDG methods suffer from. 
% \tanbui{You put the RK4 results there and you have to explain why. You
% can not let the readers to read the figure by themselves. For example,
% you can talk about why you have only two points for RK4 in Figure
% \figref{expo-euler-isentropic-tconv-uni-p16}(a). You need to label the
% numbers (I think they are Courant numbers, on the top of the figure. Also, some mutual
% comparison among RK4, EPI2, and EXPRB42 need to be spelled out. In
% particular, you need to really tell one should do EPI instead of
% RK: if you were a reader, why should you care about EPI?}

In Figure \figref{expo-euler-isentropic-tconv-uni-p16}(b), 
we see that the high-order EXPRB32 and EXPRB42 schemes are beneficial compared to
the second-order EPI2 below $\mc{O}(10^{-10})$ error level,
 but the second-order EPI2 become two times faster than EXPRB32 and EXPRB42 
 above $\mc{O}(10^{-8})$ error level. 
 Both EXPRB32 and EXPRB42 require two-stage matrix exponential evaluations, 
 hence, their wallclock times are similar. 
 However, due to the high-order accuracy, EXPRB42 is slightly more efficient than EXPRB32.
 Compared to IMEX DG, EPI2 and EXPRB32 are more economical than ARS232 and ARS443. 
 EPI2 is four times faster than ARS232, and 
 EXPRB32 is ten times faster than ARS443 at $\mc{O}(10^{-8})$ error level.
 Compared to explicit RKDG, EXPRB42 becomes comparable to RK2 near $\mc{O}(10^{-11})$ error level but
 is slightly slower than RK3 and RK4 at $\mc{O}(10^{-13})$ error level.
 Note that we use a smooth solution for convergence study. 
 In practice, $\mc{O}(10^{-13})$ error level is hard to be attainable when involving a non-smooth solution, heterogeneous materials and so on. 
% tanbui{beneficial in which sense, even me I have to decode the figure
%   to see why EXPRB42 is more beneficial? You have to spell it out.}
% However, we
% still see that RK4 DG is more economical than Exponential DG methods
% at $\mc{O}(10^{-13})$ error level.
% \tanbui{Again, why are there only two points for RK4 at a very low
%   error levels? saying RK is more advantage at
%   $10^{-13}$ is not actually  useful because one typically does not go down that
% far. Can we compare the methods in terms of accuracy and wall-clock time, at the same time stepsizes?}
%This shows that an exponential time integrator captures the fast modes in the system more accurately 
%than the IMEX method. The wall clock time of EPI2 drops sharply until Courant number reaches 7 and grows after 7. There is a sweet spot near $Cr=1.43$, of which the wall clock time of EPI2 is comparable to that of RK4. In general, the computational cost is more expensive than RK4, but there are tune parameters in the algorithm \cite{gaudreault2018kiops}. Here, we use the parameters of \texttt{tol}=$10^{-10}$, \texttt{mmin}=10, \texttt{mmax}=128 and \texttt{orth$\_$len}=100.
%The results are tabulated in \tabref{expo-euler2d-tconv-isentropic}. 

%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
\centering
\subfigure[Uniform mesh]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-msh-uniform}
  \figlab{pde-euler2d-mesh-uniform}
}
\subfigure[Non-uniform mesh]{
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-msh-nonuniform} 
 % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.3\textwidth]{./figures/EXPO-euler2d-vortex-exprb42-10x} 
  \figlab{pde-euler2d-mesh-nonuniform}
}
\caption{(a) Uniform mesh with $N_e=256$ elements and (b) non-uniform meshes with $N_e=250$ elements.}
\figlab{expo-pde-euler2d-mesh}
\end{figure}





% %---------------------
% % TIME CONVERGENCE - uniform - N16
% %---------------------
% \begin{figure}[h!t!b!]
%     \centering
%     \subfigure[Accuracy]{
%             \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N16-r}
%       \figlab{expo-euler-isentropic-tconv-uni-p16-accuracy}
%     }
%     \subfigure[Efficiency]{
%      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.413\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N16-wc}
%       \figlab{expo-euler-isentropic-tconv-uni-p16-efficiency}
%     }
%   \caption{Isentropic vortex translation in two dimensions:
%     time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
%         The computational domain is discretized with $N_e = 256$ and $k=16$. }
%   \figlab{expo-euler-isentropic-tconv-uni-p16}
% \end{figure}


%---------------------
% TIME CONVERGENCE - uniform - N16
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N16-r}
      \figlab{expo-euler-isentropic-tconv-uni-p16-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.413\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N16-wc}
      \figlab{expo-euler-isentropic-tconv-uni-p16-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=16$. }
  \figlab{expo-euler-isentropic-tconv-uni-p16}
\end{figure}


% %---------------------
% % TIME CONVERGENCE - uniform, N8
% %---------------------
% \begin{figure}[h!t!b!]
%     \centering
%     \subfigure[Accuracy]{
%             \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N8-r}
%       \figlab{expo-euler-isentropic-tconv-uni-p8-accuracy}
%     }
%     \subfigure[Efficiency]{
%      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-uni-N8-wc}
%       \figlab{expo-euler-isentropic-tconv-uni-p8-efficiency}
%     }
%   \caption{Isentropic vortex translation in two dimensions:
%     time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
%         The computational domain is discretized with $N_e = 256$ and $k=8$. }
%   \figlab{expo-euler-isentropic-tconv-uni-p8}
% \end{figure}


%---------------------
% TIME CONVERGENCE - Uniform, N8
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N8-r}
      \figlab{expo-euler-isentropic-tconv-uni-p8-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-Uniform-N8-wc}
      \figlab{expo-euler-isentropic-tconv-uni-p8-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=8$. }
  \figlab{expo-euler-isentropic-tconv-uni-p8}
\end{figure}

To mimic such a situation, we increase a spatial discretization error by lowering the polynomial order from $k=16$ to $k=8$ so that the saturation error level rises in Figure \figref{expo-euler-isentropic-tconv-uni-p8}. 
We omit the results of RK2 and RK3 in Figure \figref{expo-euler-isentropic-tconv-uni-p8}
because the errors of RK2, RK3, and RK4 are almost the same, 
but the wallclock time of RK4 is faster than those of RK2 and RK3
in Table \tabref{expo-euler-isentropic-tconv-uni-p8}.
%the errors are saturated at $\mc{O}(10^{-8})$ error level, 
In this case, the wallclock time of EPI2 becomes comparable to that of RK4
and slightly shorter than RK2.
At $\mc{O}(10^{-8})$ error level, EPI2 is two times faster than EXPRB32 and EXPRB42, 
five times faster than ARS232, and seventeen times faster than ARS443. 

% \tanbui{I don't know why we have EPI2 there because it is not
%   fourth-order accuracy as RK4. I think we should focus on EXPRB4
%   verus RK4 because they are compatible. You can do EPI2 verus RK2. I
%   think the appealing messages from these two figures are: 1) EXPRB4
% is more robust (not stability issues) with time steps, 2) EXPRB4 can
% attain the same accuracy with higher CFL numbers compared to RK4, 3)
% EXPRB4 has similar/same wall-clock time as RK4 at the same accuracy
% level. You can add more positive points here.}
% \shinhoo{In this case for $k=8$ on uniform mesh, 
% the saturation error level is at $\mc{O}(10^{-8})$. 
% The best performed methods for RKDG, Exponential DG and IMEX DG are
% RK4, EPI2 and ARS232.
% Thus it seems to be reasonable to compare EPI2 and RK4. }

%---------------------
% TEMPORAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in two dimensions:
    time convergence study on a uniform mesh.
    The computational domain is discretized with $N_e = 256$ and $k=8$.
    The error is measured at $T=1$. 
}
\tablab{expo-euler-isentropic-tconv-uni-p8}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
\hline
\multirow{2}{*}{$k=8$} 
  & \multirow{2}{*}{$Cr$}  
  % & \multirow{2}{*}{$dt$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  & \multirow{2}{*}{wc $[s]$}    \tabularnewline
  &       &  error & order &  error & order &  error & order &     \tabularnewline
\hline\hline
\multirow { 2}{*}{   RK2 }&  0.30   & 5.445E-08 &        - & 4.050E-08 &        - & 1.255E-08 &        - &     17.3 \tabularnewline
                         &  0.15   & 5.445E-08 &    0.000 & 3.942E-08 &    0.039 & 1.245E-08 &    0.012 &     37.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK3 }&  0.60   & 5.444E-08 &        - & 3.936E-08 &        - & 1.235E-08 &        - &     14.3 \tabularnewline
                         &  0.30   & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.242E-08 &   -0.008 &     24.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK4 }&  0.90   & 5.444E-08 &        - & 3.936E-08 &        - & 1.242E-08 &        - &     12.4 \tabularnewline
                         &  0.45   & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.001 &     24.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{  EPI2 }& 43.09   & 2.585E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &     14.1 \tabularnewline
                         & 21.54   & 5.097E-07 &    2.342 & 6.532E-07 &    2.364 & 1.790E-06 &    2.341 &     13.4 \tabularnewline
                         &  4.31   & 5.746E-08 &    1.356 & 4.642E-08 &    1.643 & 7.256E-08 &    1.992 &     13.5 \tabularnewline
                         % &  2.15 &  0.05 & 5.450E-08 &    0.076 & 3.986E-08 &    0.220 & 2.174E-08 &    1.739 &     23.9 \tabularnewline
                         % &  0.86 &  0.02 & 5.442E-08 &    0.002 & 3.938E-08 &    0.013 & 1.274E-08 &    0.583 &     65.4 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &   -0.001 & 3.936E-08 &    0.001 & 1.244E-08 &    0.034 &    109.4 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{EXPRB32} }& 43.09   & 1.869E-07 &        - & 1.667E-07 &        - & 6.295E-07 &        - &     28.6 \tabularnewline
                         & 21.54   & 5.556E-08 &    1.750 & 4.242E-08 &    1.974 & 4.184E-08 &    3.911 &     23.4 \tabularnewline
                         &  4.31   & 5.444E-08 &    0.013 & 3.936E-08 &    0.047 & 1.242E-08 &    0.755 &     25.7 \tabularnewline
                         % &  2.15 &  0.05 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.001 &     46.7 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    117.9 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    235.0 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{EXPRB42} }& 43.09   & 9.257E-08 &        - & 2.267E-07 &        - & 2.660E-07 &        - &     22.9 \tabularnewline
                         & 21.54   & 5.476E-08 &    0.757 & 3.982E-08 &    2.509 & 1.911E-08 &    3.799 &     21.4 \tabularnewline
                         &  4.31   & 5.444E-08 &    0.004 & 3.936E-08 &    0.007 & 1.241E-08 &    0.268 &     25.0 \tabularnewline
                         % &  2.15 &  0.05 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &   -0.002 &     46.8 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    121.1 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.243E-08 &    0.000 &    234.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{ARS232 }}& 43.09   & 1.522E-06 &        - & 4.685E-05 &        - & 6.383E-06 &        - &    156.8 \tabularnewline
                         & 21.54   & 1.764E-07 &    3.109 & 1.193E-05 &    1.973 & 1.027E-06 &    2.636 &     94.2 \tabularnewline
                         &  4.31   & 5.439E-08 &    0.731 & 4.820E-07 &    1.994 & 3.801E-08 &    2.048 &     69.7 \tabularnewline
                         &  2.15   & 5.441E-08 &   -0.001 & 1.265E-07 &    1.930 & 1.486E-08 &    1.355 &     86.2 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &   -0.001 & 4.387E-08 &    1.156 & 1.239E-08 &    0.198 &    154.1 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.967E-08 &    0.145 & 1.240E-08 &   -0.001 &    270.8 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ \small{ARS443 }}& 43.09   & 7.193E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &    850.8 \tabularnewline
                         & 21.54   & 1.541E-07 &    2.223 & 1.822E-06 &    2.938 & 5.063E-07 &    2.358 &    478.8 \tabularnewline
                         &  4.31   & 5.435E-08 &    0.648 & 4.204E-08 &    2.342 & 1.181E-08 &    2.335 &    234.2 \tabularnewline
                         &  2.15   & 5.441E-08 &   -0.002 & 3.938E-08 &    0.094 & 1.149E-08 &    0.040 &    244.4 \tabularnewline
                         % &  0.86 &  0.02 & 5.444E-08 &   -0.001 & 3.936E-08 &    0.001 & 1.230E-08 &   -0.074 &    334.8 \tabularnewline
                         % &  0.43 &  0.01 & 5.444E-08 &    0.000 & 3.936E-08 &    0.000 & 1.241E-08 &   -0.013 &    556.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}

 

On the non-uniform mesh, 
we observe that the convergence rates for 
EPI2, EXPRB32, EXPRB42, ARS232, and ARS443 agree to the theoretical convergence rates for a wide range of Courant numbers Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(a).
In Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(b), we compare the efficiency of Exponential DG methods to those of others. 
EPI2 is three times faster than ARS232 at $\mc{O}(10^{-10})$ error level. 
EXPRB32 is five times faster than ARS443 at $\mc{O}(10^{-12})$ error level.
EPI2 is almost two times faster than EXPRB32 and EXPRB42 above $\mc{O}(10^{-10})$ error level. 
However, as tighten the error level, the high-order EXPRB32 and EXPRB42 become more economical than EPI2.
Compared to explicit RK methods, 
at $\mc{O}(10^{-13})$ error level, EXPRB32 is comparable to RK2, RK3 and RK4 methods in terms of accuracy and efficiency. 
EXPRB42 shows slightly better performance than EXPRB32, RK2, RK3 and RK4 methods.
%  we observe that
% the similar temporal convergence results in Figure \figref{expo-euler-isentropic-tconv-nonuni-p16}(a).
% and \figref{expo-euler-isentropic-tconv-nonuni-p8}.
% We 
% we start to see the benefit of Exponential DG schemes. 
% In (b),
% the wall clock time of EXPRB42 becomes comparable to RK4 at $\mc{O}(10^{-12})$ error level.
Next, we add a spatial discretization error by lowering the solution order from $k=16$ to $k=8$. 
We see the computational gain of Exponential DG methods in Figure \figref{expo-euler-isentropic-tconv-nonuni-p8}(b) and Table 
\tabref{expo-euler-isentropic-tconv-nonuni-p8}.
At $\mc{O}(10^{-9})$ error level, 
the wallclock times of RK2, RK3 and RK4 are $188.2$, $107.6$ and $116.2$.
EPI2 is three times faster than RK2, and 
two times faster than RK3 and RK4. 
EPI2 is four times faster than ARS232. 
EXPRB32 is six times faster than ARS443. 

% \tanbui{see my above comments. Again, I think we should focus on RK4
%   verus EXPRB4. I think you can say similar thing for RK2 versus RK4,
%   that is RK2 can get similary accuracy with better wallclock time?}


%---------------------
% TIME CONVERGENCE non-uniform, N16
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N16-r}
      \figlab{expo-euler-isentropic-tconv-p16-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.405\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N16-wc}
      \figlab{expo-euler-isentropic-tconv-p16-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on non-uniform mesh.
        The computational domain is discretized with $N_e = 250$ and $k=16$. }
  \figlab{expo-euler-isentropic-tconv-nonuni-p16}
\end{figure}




%---------------------
% TIME CONVERGENCE - nonuniform, N8
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[Accuracy]{
            \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.44\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N8-r}
      \figlab{expo-euler-isentropic-tconv-p8-accuracy}
    }
    \subfigure[Efficiency]{
     \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.42\textwidth]{./figures/EXPO-euler2d-TimeConv-NonUniform-N8-wc}
      \figlab{expo-euler-isentropic-tconv-p8-efficiency}
    }
  \caption{Isentropic vortex translation in two dimensions:
    time convergence study for (a) accuracy and (b) efficiency on a non-uniform mesh.
        The computational domain is discretized with $N_e = 256$ and $k=8$. }
  \figlab{expo-euler-isentropic-tconv-nonuni-p8}
\end{figure}





% %---------------------
% % TEMPORAL CONVERGENCE k=16 on nonuniform mesh
% %---------------------
% \begin{table}[t]
% \caption{Isentropic vortex translation in two dimensions:
%     time convergence study on a nonuniform mesh.
%     The computational domain is discretized with $N_e = 256$ and $k=16$.
%     The error is measured at $T=1$. 
% }
% \tablab{expo-euler-isentropic-tconv-nonuni-p16}
% \begin{center}
% \begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
% \hline
% \multirow{2}{*}{$k=16$} 
%   & \multirow{2}{*}{$dt$}  
%   & \multirow{2}{*}{$Cr$}  
%   & \multicolumn{2}{c|}{$\rho$}   
%   & \multicolumn{2}{c|}{$\rho {\bf u}$}   
%   & \multicolumn{2}{c|}{$\rho E$}   
%   & \multirow{2}{*}{wc $[s]$}    \tabularnewline
%   &    &   &  error & order &  error & order &  error & order &     \tabularnewline
% \hline\hline
% \multirow { 2}{*}{   RK2 }&  0.30 &  0.00 & 5.339E-13 &        - & 8.416E-12 &        - & 8.095E-13 &        - &   1001.9 \tabularnewline
%                          &  0.15 &  0.00 & 9.172E-13 &   -0.781 & 3.474E-12 &    1.277 & 7.404E-13 &    0.129 &   2017.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 2}{*}{   RK3 }&  0.60 &  0.00 & 3.081E-13 &        - & 2.833E-12 &        - & 2.037E-13 &        - &    703.1 \tabularnewline
%                          &  0.30 &  0.00 & 5.085E-13 &   -0.723 & 2.837E-12 &   -0.002 & 3.759E-13 &   -0.884 &   1375.5 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 2}{*}{   RK4 }&  0.90 &  0.00 & 4.578E-13 &        - & 2.837E-12 &        - & 4.165E-13 &        - &    778.3 \tabularnewline
%                          &  0.45 &  0.00 & 8.476E-13 &   -0.889 & 2.860E-12 &   -0.012 & 8.353E-13 &   -1.004 &   1579.9 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{  EPI2 }& 1497.94 &  1.00 & 2.583E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &    314.2 \tabularnewline
%                          & 748.97 &  0.50 & 5.085E-07 &    2.345 & 6.518E-07 &    2.367 & 1.790E-06 &    2.341 &    318.0 \tabularnewline
%                          & 149.79 &  0.10 & 2.031E-08 &    2.001 & 2.437E-08 &    2.042 & 7.154E-08 &    2.001 &    307.9 \tabularnewline
%                          & 74.90 &  0.05 & 5.079E-09 &    2.000 & 6.079E-09 &    2.003 & 1.789E-08 &    2.000 &    306.5 \tabularnewline
%                          & 29.96 &  0.02 & 8.087E-10 &    2.005 & 1.033E-09 &    1.934 & 2.849E-09 &    2.005 &    309.2 \tabularnewline
%                          & 14.98 &  0.01 & 1.933E-10 &    2.065 & 6.806E-10 &    0.602 & 6.844E-10 &    2.058 &    333.1 \tabularnewline
%                          &  7.49 &  0.01 & 5.086E-11 &    1.926 & 6.075E-11 &    3.486 & 1.792E-10 &    1.933 &    451.8 \tabularnewline
%                          &  3.00 &  0.00 & 8.142E-12 &    1.999 & 1.011E-11 &    1.957 & 2.867E-11 &    2.000 &   1127.4 \tabularnewline
%                          &  1.50 &  0.00 & 2.048E-12 &    1.991 & 3.730E-12 &    1.439 & 7.169E-12 &    2.000 &   2196.0 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ EXPRB32 }& 1497.94 &  1.00 & 1.807E-07 &        - & 1.608E-07 &        - & 6.291E-07 &        - &    658.2 \tabularnewline
%                          & 748.97 &  0.50 & 1.125E-08 &    4.006 & 1.562E-08 &    3.364 & 3.957E-08 &    3.991 &    691.8 \tabularnewline
%                          & 149.79 &  0.10 & 7.677E-11 &    3.099 & 1.186E-10 &    3.032 & 2.707E-10 &    3.097 &    682.5 \tabularnewline
%                          & 74.90 &  0.05 & 9.519E-12 &    3.012 & 1.516E-11 &    2.968 & 3.355E-11 &    3.012 &    697.9 \tabularnewline
%                          & 29.96 &  0.02 & 6.435E-13 &    2.940 & 3.122E-12 &    1.725 & 2.156E-12 &    2.996 &    699.9 \tabularnewline
%                          & 14.98 &  0.01 & 2.173E-13 &    1.566 & 3.139E-12 &   -0.008 & 3.400E-13 &    2.665 &    747.2 \tabularnewline
%                          &  7.49 &  0.01 & 1.980E-13 &    0.134 & 2.831E-12 &    0.149 & 9.341E-14 &    1.864 &    925.7 \tabularnewline
%                          &  3.00 &  0.00 & 2.034E-13 &   -0.029 & 2.831E-12 &    0.000 & 9.202E-14 &    0.016 &   2320.2 \tabularnewline
%                          &  1.50 &  0.00 & 2.182E-13 &   -0.101 & 2.831E-12 &    0.000 & 1.118E-13 &   -0.281 &   4569.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 6}{*}{ EXPRB42 }& 1497.94 &  1.00 & 7.521E-08 &        - & 2.216E-07 &        - & 2.652E-07 &        - &    569.9 \tabularnewline
%                          & 748.97 &  0.50 & 4.273E-09 &    4.138 & 4.914E-09 &    5.495 & 1.518E-08 &    4.127 &    557.5 \tabularnewline
%                          & 149.79 &  0.10 & 4.552E-12 &    4.253 & 7.129E-12 &    4.061 & 1.628E-11 &    4.249 &    570.7 \tabularnewline
%                          & 74.90 &  0.05 & 3.442E-13 &    3.725 & 2.984E-12 &    1.256 & 1.010E-12 &    4.011 &    576.4 \tabularnewline
%                          & 29.96 &  0.02 & 1.977E-13 &    0.605 & 2.956E-12 &    0.010 & 1.110E-13 &    2.410 &    586.0 \tabularnewline
%                          & 14.98 &  0.01 & 1.977E-13 &    0.000 & 3.141E-12 &   -0.088 & 1.418E-13 &   -0.353 &    616.5 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ ARS232P }& 1497.94 &  1.00 & 1.521E-06 &        - & 4.685E-05 &        - & 6.384E-06 &        - &  15105.5 \tabularnewline
%                          & 748.97 &  0.50 & 1.714E-07 &    3.150 & 1.193E-05 &    1.973 & 1.028E-06 &    2.635 &  12694.5 \tabularnewline
%                          & 149.79 &  0.10 & 4.126E-09 &    2.316 & 4.803E-07 &    1.996 & 3.718E-08 &    2.063 &   2196.1 \tabularnewline
%                          & 74.90 &  0.05 & 1.003E-09 &    2.040 & 1.201E-07 &    2.000 & 9.267E-09 &    2.004 &   1407.4 \tabularnewline
%                          & 29.96 &  0.02 & 1.589E-10 &    2.011 & 1.922E-08 &    2.000 & 1.481E-09 &    2.001 &   1179.5 \tabularnewline
%                          & 14.98 &  0.01 & 3.964E-11 &    2.003 & 4.804E-09 &    2.000 & 3.703E-10 &    2.000 &   1399.6 \tabularnewline
%                          &  7.49 &  0.01 & 9.904E-12 &    2.001 & 1.201E-09 &    2.000 & 9.257E-11 &    2.000 &   1909.1 \tabularnewline
%                          &  3.00 &  0.00 & 1.598E-12 &    1.991 & 1.922E-10 &    2.000 & 1.481E-11 &    2.000 &   3540.6 \tabularnewline
%                          &  1.50 &  0.00 & 4.542E-13 &    1.815 & 4.812E-11 &    1.998 & 3.703E-12 &    2.000 &   6299.9 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \multirow { 9}{*}{ ARS443P }& 1497.94 &  1.00 & 7.160E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &  57792.7 \tabularnewline
%                          & 748.97 &  0.50 & 1.429E-07 &    2.325 & 1.822E-06 &    2.938 & 5.065E-07 &    2.357 &  48308.7 \tabularnewline
%                          & 149.79 &  0.10 & 1.298E-09 &    2.921 & 1.484E-08 &    2.989 & 4.701E-09 &    2.908 &  11462.6 \tabularnewline
%                          & 74.90 &  0.05 & 1.583E-10 &    3.036 & 1.858E-09 &    2.998 & 5.777E-10 &    3.025 &   6100.7 \tabularnewline
%                          & 29.96 &  0.02 & 9.950E-12 &    3.020 & 1.190E-10 &    2.999 & 3.645E-11 &    3.016 &   3776.6 \tabularnewline
%                          & 14.98 &  0.01 & 1.256E-12 &    2.986 & 1.515E-11 &    2.974 & 4.545E-12 &    3.004 &   3764.3 \tabularnewline
%                          &  7.49 &  0.01 & 2.552E-13 &    2.299 & 3.398E-12 &    2.157 & 5.890E-13 &    2.948 &   4862.9 \tabularnewline
%                          &  3.00 &  0.00 & 2.026E-13 &    0.252 & 2.834E-12 &    0.198 & 1.032E-13 &    1.901 &   7826.9 \tabularnewline
%                          &  1.50 &  0.00 & 2.187E-13 &   -0.110 & 2.831E-12 &    0.002 & 1.119E-13 &   -0.117 &  13226.2 \tabularnewline
% \multicolumn{10}{c}{} \tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}
 
%---------------------
% TEMPORAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in two dimensions:
    time convergence study on a nonuniform mesh.
    The computational domain is discretized with $N_e = 256$ and $k=8$.
    The error is measured at $T=1$. 
}
\tablab{expo-euler-isentropic-tconv-nonuni-p8}

\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{1}{c}}
\hline
\multirow{2}{*}{$k=8$} 
  % & \multirow{2}{*}{$dt$}  
  & \multirow{2}{*}{$Cr$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  & \multirow{2}{*}{wc $[s]$}    \tabularnewline
  &     &  error & order &  error & order &  error & order &     \tabularnewline
\hline\hline
\multirow { 2}{*}{   RK2 }&  0.29  & 1.618E-09 &        - & 1.586E-09 &        - & 5.310E-10 &        - &    188.2 \tabularnewline
                         &  0.15  & 1.618E-09 &    0.000 & 1.584E-09 &    0.002 & 5.309E-10 &    0.000 &    393.2 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK3 }&  0.59  & 1.618E-09 &        - & 1.584E-09 &        - & 5.308E-10 &        - &    107.6 \tabularnewline
                         &  0.29  & 1.618E-09 &    0.000 & 1.584E-09 &    0.000 & 5.308E-10 &    0.000 &    227.8 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 2}{*}{   RK4 }&  0.90  & 1.618E-09 &        - & 1.584E-09 &        - & 5.308E-10 &        - &    116.2 \tabularnewline
                         &  0.45  & 1.618E-09 &    0.000 & 1.584E-09 &    0.000 & 5.308E-10 &    0.000 &    259.3 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{  EPI2 }& 452.34  & 2.583E-06 &        - & 3.363E-06 &        - & 9.068E-06 &        - &     55.2 \tabularnewline
                         & 226.17  & 5.085E-07 &    2.345 & 6.518E-07 &    2.367 & 1.790E-06 &    2.341 &     61.3 \tabularnewline
                         & 45.23  & 2.038E-08 &    1.999 & 2.442E-08 &    2.041 & 7.153E-08 &    2.001 &     54.2 \tabularnewline
                         & 22.62  & 5.326E-09 &    1.936 & 6.298E-09 &    1.955 & 1.786E-08 &    2.002 &     53.6 \tabularnewline
                         &  9.05  & 1.810E-09 &    1.178 & 1.872E-09 &    1.324 & 2.885E-09 &    1.990 &     58.0 \tabularnewline
                         &  4.52  & 1.631E-09 &    0.150 & 1.603E-09 &    0.224 & 8.786E-10 &    1.715 &    114.9 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ EXPRB32 }& 452.34  & 1.807E-07 &        - & 1.608E-07 &        - & 6.291E-07 &        - &    108.4 \tabularnewline
                         & 226.17  & 1.142E-08 &    3.984 & 1.571E-08 &    3.356 & 3.958E-08 &    3.990 &    108.8 \tabularnewline
                         & 45.23  & 1.623E-09 &    1.212 & 1.591E-09 &    1.423 & 5.922E-10 &    2.611 &    111.6 \tabularnewline
                         & 22.62  & 1.619E-09 &    0.004 & 1.588E-09 &    0.003 & 5.280E-10 &    0.166 &    114.9 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.001 & 1.621E-09 &   -0.022 & 5.304E-10 &   -0.005 &    120.1 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.033 & 5.308E-10 &   -0.001 &    228.7 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ EXPRB42 }& 452.34  & 7.525E-08 &        - & 2.216E-07 &        - & 2.652E-07 &        - &     89.7 \tabularnewline
                         & 226.17  & 4.623E-09 &    4.025 & 5.182E-09 &    5.418 & 1.518E-08 &    4.127 &     92.0 \tabularnewline
                         & 45.23  & 1.618E-09 &    0.652 & 1.585E-09 &    0.736 & 5.280E-10 &    2.087 &     94.4 \tabularnewline
                         & 22.62  & 1.618E-09 &    0.000 & 1.586E-09 &   -0.001 & 5.262E-10 &    0.005 &     93.0 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.000 & 1.595E-09 &   -0.006 & 5.298E-10 &   -0.007 &    120.0 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.010 & 5.308E-10 &   -0.003 &    229.3 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ ARS232 }& 452.34  & 1.521E-06 &        - & 4.685E-05 &        - & 6.384E-06 &        - &   1707.7 \tabularnewline
                         & 226.17  & 1.715E-07 &    3.149 & 1.193E-05 &    1.973 & 1.028E-06 &    2.635 &    934.7 \tabularnewline
                         & 45.23  & 4.427E-09 &    2.272 & 4.803E-07 &    1.996 & 3.718E-08 &    2.063 &    260.1 \tabularnewline
                         & 22.62  & 1.904E-09 &    1.217 & 1.201E-07 &    2.000 & 9.274E-09 &    2.003 &    217.6 \tabularnewline
                         &  9.05  & 1.626E-09 &    0.172 & 1.928E-08 &    1.996 & 1.566E-09 &    1.941 &    241.1 \tabularnewline
                         &  4.52  & 1.619E-09 &    0.006 & 5.062E-09 &    1.929 & 6.429E-10 &    1.284 &    345.7 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\multirow { 6}{*}{ ARS443 }& 452.34  & 7.160E-07 &        - & 1.396E-05 &        - & 2.595E-06 &        - &   6312.7 \tabularnewline
                         & 226.17  & 1.430E-07 &    2.324 & 1.822E-06 &    2.938 & 5.065E-07 &    2.357 &   4786.2 \tabularnewline
                         & 45.23  & 2.113E-09 &    2.619 & 1.493E-08 &    2.985 & 4.694E-09 &    2.909 &   1268.1 \tabularnewline
                         & 22.62  & 1.631E-09 &    0.374 & 2.443E-09 &    2.611 & 7.124E-10 &    2.720 &    910.2 \tabularnewline
                         &  9.05  & 1.618E-09 &    0.009 & 1.588E-09 &    0.470 & 5.168E-10 &    0.350 &    743.4 \tabularnewline
                         &  4.52  & 1.618E-09 &    0.000 & 1.584E-09 &    0.004 & 5.285E-10 &   -0.032 &    869.1 \tabularnewline
\multicolumn{9}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}

To demonstrate the high-order convergence in space,  
we perform the spatial convergence test.
We use a sequence of nested meshes with $N_e = \LRp{256,1024,4096,16384}$ 
for $k=\LRp{1,2,3,4}$ and measure the errors at $t=1$. 
As can be seen in Table \tabref{expo-euler-isentropic-sconv-uni},
the convergence rate of $(k + \half)$ is observed as refining the meshes.

%---------------------
% SPATIAL CONVERGENCE
%---------------------
\begin{table}[t]
\caption{Spatial convergence for the isentropic vortex translation in two dimensions.
    We use a sequence of nested meshes with $N_e = \LRc{256, 1024, 4096, 16384}$ for $k=\LRc{1,2,3,4}$. 
    We use EXPRB42 scheme with $dt=0.01$ and measure the errors at $t=1$.  
}
\tablab{expo-euler-isentropic-sconv-uni}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
\hline
\multirow{2}{*}{ } 
  & \multirow{2}{*}{$h$}  
  & \multicolumn{2}{c|}{$\rho$}   
  & \multicolumn{2}{c|}{$\rho {\bf u}$}   
  & \multicolumn{2}{c|}{$\rho E$}   
  \tabularnewline
  &    &  error & order &  error & order &  error & order       \tabularnewline
\hline\hline
\multirow { 4}{*}{    k=1 }&  1.00 & 9.942E-04 &        - & 7.389E-03 &        - & 1.595E-03 &        - \tabularnewline
                         &  0.50 & 7.662E-04 &    0.376 & 1.999E-03 &    1.886 & 5.181E-04 &    1.622 \tabularnewline
                         &  0.25 & 4.344E-04 &    0.819 & 5.312E-04 &    1.912 & 2.049E-04 &    1.338 \tabularnewline
                         &  0.12 & 2.312E-04 &    0.910 & 1.383E-04 &    1.941 & 8.571E-05 &    1.257 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=2 }&  1.00 & 2.909E-04 &        - & 7.382E-04 &        - & 4.423E-04 &        - \tabularnewline
                         &  0.50 & 1.201E-04 &    1.276 & 1.418E-04 &    2.380 & 4.965E-05 &    3.155 \tabularnewline
                         &  0.25 & 3.235E-05 &    1.892 & 1.570E-05 &    3.175 & 7.084E-06 &    2.809 \tabularnewline
                         &  0.12 & 5.787E-06 &    2.483 & 2.084E-06 &    2.913 & 1.257E-06 &    2.495 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=3 }&  1.00 & 1.286E-04 &        - & 2.343E-04 &        - & 6.979E-05 &        - \tabularnewline
                         &  0.50 & 1.972E-05 &    2.705 & 1.541E-05 &    3.926 & 5.605E-06 &    3.638 \tabularnewline
                         &  0.25 & 2.123E-06 &    3.215 & 9.655E-07 &    3.996 & 4.450E-07 &    3.655 \tabularnewline
                         &  0.12 & 2.112E-07 &    3.329 & 6.849E-08 &    3.817 & 4.386E-08 &    3.343 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 4}{*}{    k=4 }&  1.00 & 2.686E-05 &        - & 3.180E-05 &        - & 1.311E-05 &        - \tabularnewline
                         &  0.50 & 2.067E-06 &    3.700 & 1.283E-06 &    4.631 & 4.381E-07 &    4.903 \tabularnewline
                         &  0.25 & 9.543E-08 &    4.437 & 4.294E-08 &    4.901 & 1.333E-08 &    5.039 \tabularnewline
                         &  0.12 & 4.540E-09 &    4.394 & 1.458E-09 &    4.880 & 5.294E-10 &    4.654 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}


%------------------------------3D---------------------------
Figure \figref{expo-euler3d-ss-isentropic} shows snapshots of advecting isentropic vortex at $t=[0,10,25]$ in three-dimensions. For spatial discretization, we 
take $N_e = 6400$ elements and $k=8$ solution order on a uniform mesh. 
For time discretization, we choose EPI2 with $dt=0.25 (Cr=27.9)$. 
We see the center of the vortex is located at the lateral boundary at $t=25$
because the mean speed of the flow is $0.2$ and the half-length of the
domain is $5$.
% \tanbui{Do we have exact solution here? If yes, plotting the error
%   (i.e. contours or pointwise values)
%   between the exact and numerical solutions is much more informative.}
% \shinhoo{I think we can do later if it needed.}

%---------------------
% SNAPSHOTS
%---------------------
\begin{figure}[h!t!b!]
    \centering
    \subfigure[$t=0$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t0}
      \figlab{expo-euler3d-ss-isentropic-epi2-t0}
    }
    \subfigure[$t=10$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t10}
      \figlab{expo-euler3d-ss-isentropic-epi2-t10}
    }
    \subfigure[$t=25$]{
      \includegraphics[trim=7.0cm 4.0cm 6.0cm 5.0cm,clip=true,width=0.30\textwidth]{./figures/EXPO-euler3d-isentropic_w_t25}
      \figlab{expo-euler3d-ss-isentropic-epi2-t25}
    }
  \caption{Isentropic vortex translation in three dimensions: 
    snapshots for (a) EPI2 with $Cr=27.9 (dt=0.25)$.
    Simulations are performed on the grid with $N_e = 6400$ and $k=8$ solution order for $t \in [0,20]$.}
  \figlab{expo-euler3d-ss-isentropic}
\end{figure}

Now we study the parallel performance of Exponential DG methods for three-dimensional Euler model.
Parallel simulations are conducted on Stampede2 at the Texas Advanced Computing Center (TACC).  
Stampede 2 provides 4,200 Knights Landing (KNL) nodes and 1,736 Skylake (SKX) nodes. Each node of KNL consists of 68 cores of Intel Xeon Phi 7250 1.4GHz processors, 96 GB of traditional DDR4 RAM, and 16 GB high-speed MCDRAM. 
Each node of SKX consists of 48 cores of Intel Xeon Platinum 8160 2.1 GHz processors and 192GB DDR4 RAM. The interconnect is a 100 GB/s Intel Omni-Path (OPA) network with a fat-tree topology. We conduct strong and weak scaling study on SKX system. 
%To this end, we have implemented the adaptive Krylov subspace method \cite{gaudreault2018kiops}
%on top of the DG finite element library written in C\texttt{++}, which is the spin-off library from \texttt{mangll} \cite{wilcox2010high}. 
%For computing a matrix exponential, 
%we use \texttt{EIGEN} C\texttt{++} library.
%Parallel implementations mainly focus on vector-vector multiplication and matrix-vector multiplication.
%The matrix-vector multiplication is carried out in a matrix-free manner 
%by calling the linear operator $L\qb$ in \eqnref{EXPO-SemiDiscretizedForm_ode}. 
%By the virtue of the DG discretization, the computation of $L\qb$ is embarrassingly parallel.
%For a dot product (vector-vector multiplication), we initially scatter a global vector to each processor, and then we perform the dot product with the local vector.  
%Next, we call \texttt{MPI ALLreduce} function. 

Recall that EPI2 and RK4 show similar performance for $k=8$ solution on the uniform mesh,
as seen in Figure \figref{expo-euler-isentropic-tconv-uni-p8}.
We will see how they perform in parallel computing. 
In Table \tabref{expo-euler-strongscale-isentropic-withRK}, 
strong scaling results of EPI2 are compared with the RK4 counterpart. 
Domain is discretized with $N_e=6400$ elements and $k=8$ solution order.
We take $dt=0.25 (Cr=27.9)$ for EPI2 and $dt=0.005 (Cr=0.56)$ for RK4 
and perform the simulations up to $t=2$. 
In general, EPI2 is comparable to RK4 in terms of wallclock time. 
The efficiency 
\footnote{
Efficiency is defined by $\frac{T_s}{T_p n_p}$
with $n_p$ the number of processors, $T_s$ serial wallclock time and $T_p$ parallel wallclock time.
Here, we approximate $T_s \simeq T_{base} \times n_{p_{base}}$ 
where $T_{base}$ is parallel wallclock time with $n_{p_{base}}$ cores. 
}
of EPI2 is slightly better than the RK4 counterpart. 
For both EPI2 and RK4, we see the efficiency drops as increasing the number of processors. This is because the number of elements per core decreases as increasing cores so that the communication cost starts to dominate over the computational cost. 

%---------------------
% STRONG SCALING
%---------------------
\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with $Cr=27.9 (dt=0.25)$ 
  and RK4 with $Cr=0.56 (dt=0.005)$
  are performed with $N_e=6400$ and $k=8$ solution order up to $t=2$. 
}
\tablab{expo-euler-strongscale-isentropic-withRK}
\begin{center}
\begin{tabular}{c|c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} & \multirow{2}{*}{$N_e/core$}
& \multicolumn{2}{c|}{EPI2}
& \multicolumn{2}{c}{RK4}   \tabularnewline
     &     & Wallclock [s] & Efficiency
           & Wallclock [s] & Efficiency \tabularnewline
\hline\hline
32 & 200  & 1283& 100& 1014&100 \tabularnewline
64 & 100    & 537.3& 119.4& 501.6&101.1\tabularnewline
128 & 50     & 424.8& 75.5& 315.5& 80.3\tabularnewline
256 & 25      &148.6& 107.9& 225.9&56.1\tabularnewline
512 & 12.5   & 114.1& 70.3& 118.1& 53.7\tabularnewline
1024 & 6.3   & 64.38&62.3& 64.49& 49.1\tabularnewline
2048 & 3.1& 39.38& 50.9& 37.11&42.7\tabularnewline
4096 &  1.6 & 24.39&41.1&20.17&39.3\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

We can increase the efficiency by assigning more elements to each processor. 
%Next, we assign additional elements to each processor by refining the mesh. 
  Table \tabref{expo-euler-strongscale-isentropic-ndof} compares the efficiencies of two different spatial discretization: 
(i) $N_e=51200$ elements and $k=6$ solution order, 
and (ii)$N_e=6400$ elements and $k=8$ solution order. 
The number of elements per core for the former discretization is eight-times larger than that for the latter. 
The efficiency with the former becomes higher than the latter counterpart as increasing the number of cores. 
%That is the number of elements per core decreases. 
\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with different degrees-of-freedoms (DOF).
  For the number of DOF (NDOF) of $17,561,600$, 
   simulations are performed on $N_e=51200$ and $k=6$ solution order
   with $dt=0.25(Cr=32.98)$ up to $t=1$, 
   whereas for NDOF of $4,665,600$, 
   simulations are performed on $N_e=6400$ and $k=8$ solution order
   with $dt=0.25(Cr=27.93)$ up to $t=2$.  
}
\tablab{expo-euler-strongscale-isentropic-ndof}
\begin{center}
\begin{tabular}{c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} 
& \multicolumn{2}{c|}{$NDOF=17,561,600$}
& \multicolumn{2}{c}{$NDOF=4,665,600$}   \tabularnewline
           & $N_e/core$ & Efficiency
           & $N_e/core$ & Efficiency \tabularnewline
\hline\hline
32  & 1600  & 100   & 200  & 100   \tabularnewline
64  & 800   & 97.9  & 100  & 119.4 \tabularnewline
128 & 400   & 82.7  & 50   & 75.5  \tabularnewline
256 & 200   & 85.7  & 25   & 107.9 \tabularnewline
512 & 100   & 61.9  & 12.5 & 70.3  \tabularnewline
1024 & 50   & 59.2  & 6.3  & 62.3  \tabularnewline
2048 & 25   & 55.0  & 3.1  & 50.9  \tabularnewline
4096 & 12.5 & 51.4  & 1.6  & 41.1  \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


To understand the effect of the timestep size on efficiency, 
we conduct strong scaling tests with two different timestep sizes, 
$dt=0.125$ and $dt=0.25$, 
on the mesh with $N_e=51200$ elements and $k=6$ solution order. 
As shown in Table \tabref{expo-euler-strongscale-isentropic-varyCr}, 
the efficiency with $dt=0.125$ is slightly higher than that with $dt=0.25$. 
This is because the latter case involves more Krylov iterations than the former case.
The total number of Krylov steps $N_{Krylov}$ is 
$561$ for $dt=0.125$ and $1024$ for $dt=0.25$.
This implies that the spectrum of the linear operator becomes broad by increasing the timestep size 
\footnote{
Note that the input argument of $\varphi$-function is $\triangle t L$. 
}.


%EPI2 allows a large timestep size, but the cost increases, too. %It seems that doubling the timestep size increases the computational cost two-times. This is somewhat makes sense because EPI2 adds more sub-steps with the large time intervals. 

\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  strong scaling results for EPI2 with $Cr=16.49 (dt=0.125)$
  and $Cr=32.98 (dt=0.25)$
  are performed with $N_e=51200$ and $k=6$ solution order up to $t=1$.
}
\tablab{expo-euler-strongscale-isentropic-varyCr}
\begin{center}
\begin{tabular}{c|c||cc|cc}
\hline
\multirow{2}{*}{$\# cores$} & \multirow{2}{*}{$N_e/core$}
& \multicolumn{2}{c|}{$dt=0.125$}
& \multicolumn{2}{c}{$dt=0.25$}   \tabularnewline
     &     & Wallclock [s] & Efficiency
            & Wallclock [s] & Efficiency \tabularnewline
\hline\hline
32   & 1600 & 2346  & 100  & 4151  & 100 \tabularnewline
64   & 800  & 1199  & 97.8 & 2121  & 97.9 \tabularnewline
128  & 400  & 607.7 & 96.5 & 1255  & 82.7 \tabularnewline
256  & 200  & 306.9 & 95.6 & 605.7 & 85.7 \tabularnewline
512  & 100  & 237.3 & 61.8 & 419.1 & 61.9 \tabularnewline
1024 & 50   & 122.7 & 59.7 & 219.1 & 59.2 \tabularnewline
2048 & 25   & 61.33 & 59.5 & 118.0 & 55.0 \tabularnewline
4096 & 12.5 & 33.72 & 54.4 & 63.12 & 51.4 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

Based on the above observations, 
we conduct a strong scaling test for EPI2 
with $Cr=8.1 (dt=0.03125)$, $N_e = 3,276,800$ and $k=4$ solution order.
We use the consecutive processors, $n_p=\LRc{16,32,64,128,256,512,868}\times 48$
so that the number of elements per core approximately becomes $\LRc{4267, 2133, 1067, 533, 267, 133, 79}$. 
%so that the number of elements per core becomes $\LRc{4266.7, 2133.3, 1066.7, 533.3, 266.7, 133.3, 78.6}$. 
In Figure \figref{expo-euler-strongscale-isentropic-withEPI2},
the speedup
\footnote{
Speedup is defined as $\frac{T_s}{T_p}$
with $T_s$ serial wallclock time and $T_p$ parallel wallclock time.
} factor shows a good strong scalability up to 41664 cores 
(which is the maximum cores in Skylake system in TACC).

% and is comparable to 
%the speedup factor of RK4 up to 4096 cores. 

\begin{figure}[h!t!b!]
    \centering
%    \subfigure[EPI2]{
      \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.83\textwidth]{./figures/EXPO-euler-strongscale-epi2}
      \figlab{expo-euler-strongscale-isentropic-epi2}
 %   }
  %  \subfigure[RK4]{
  %   \includegraphics[trim=0.0cm 0.cm 0.0cm 0.0cm,clip=true,width=0.43\textwidth]{./figures/EXPO-euler-strongscale-rk4} 
  %    \figlab{expo-euler-strongscale-isentropic-rk4}
  %  }
  \caption{Isentropic vortex translation in three dimensions: 
    strong scaling study for EPI2 with $Cr=8.1 (dt=0.03125)$. 
    The computational domain is discretized with $N_e = 3,276,800$ and $k=4$ solution order
 for $n_p=\LRc{16,32,64,128,256,512,868}\times 48$.}
  \figlab{expo-euler-strongscale-isentropic-withEPI2}
\end{figure}


For the weak scaling test, 
we assign the same amount of work to each processor 
while increasing the number of processors. 
We discretize the domain with 
$N_e = \LRc{1, 8, 64, 512, 4096}\times 100$ elements and $k=8$ solution order, 
and decompose the domain with $n_p = \LRc{4, 32, 256, 2048, 16384}$ processors. 
That is, we make the number of elements per core to be 25.
We also keep the Courant number fixed 
so that the total number of Krylov steps, $N_{Krylov}$ to be uniform.
We have tabulated the weak scaling results in Table \tabref{expo-euler-weakscale-isentropic-fixcr}. We observe that $N_{Krylov}$ tends to linearly increase with the Courant number. We also see that the increment of wallclock time is relatively small for a fixed Courant number. We plot the average time per timestep against the number of degrees-of-freedom in Figure \figref{expo-euler-weakscale-isentropic-fixcr}, from which we see Exponential DG methods show a good weak scaling result. 

%---------------------
% Weak scaling test 
%---------------------

\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  weak scaling results for EPI2 with fixed Courant numbers.
  Each core has $18,225$ degrees-of-freedom (=$25$ elements and $8th$ solution order). 
}
\tablab{expo-euler-weakscale-isentropic-fixcr}
\begin{center}
\begin{tabular}{cc|c|c|c|c}
\hline
$Cr$ &$N_e$ & $dt$ & Final time & Wallclock [s] & $N_{Krylov}$ \tabularnewline
\hline\hline 
\multirow{4}{*}{$ 5.59$}  
  &  4   & 0.2    & 0.8  & 15.3  & 103 \tabularnewline
  & 32   & 0.1    & 0.4  & 17.8  & 90 \tabularnewline
  & 256  & 0.05   & 0.2  & 24.4  & 81 \tabularnewline
  & 2048 & 0.025  & 0.1  & 27.8  & 81 \tabularnewline
  & 16384& 0.0125 & 0.05 & 29.3  & 82 \tabularnewline
\tabularnewline
\multirow{4}{*}{$ 22.4$}  
  &  4   & 0.2   & 0.8  & 50.4  & 397 \tabularnewline
  & 32   & 0.1   & 0.4  & 89.9  & 381 \tabularnewline
  & 256  & 0.05  & 0.2  & 85.8  & 355 \tabularnewline
  & 2048 & 0.025 & 0.1  & 86.9  & 348 \tabularnewline
  &16384 & 0.0125& 0.05 & 93.1  & 358 \tabularnewline
\tabularnewline
\multirow{4}{*}{$ 55.9$}  
  &  4   & 0.2   & 0.8  & 130.9 & 1024\tabularnewline
  & 32   & 0.1   & 0.4  & 240.4 & 1023 \tabularnewline
  & 256  & 0.05  & 0.2  & 246.2 & 1024 \tabularnewline
  & 2048 & 0.025 & 0.1  & 248.8 & 1024 \tabularnewline
  &16384 & 0.0125& 0.05 & 342.2 & 1408 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-euler-weakscale-fixedCr} 
  \caption{Isentropic vortex translation in 3D: 
    weak scaling study with fixed Courant numbers. 
    The computational domain is discretized with $N_e = \LRc{1, 8, 64, 512,4096}\times 100$ and $k=8$ solution order for $n_p=\LRc{4,32,256,2048,16384}$, respectively,
    so that each processor has 25 elements. }
  \figlab{expo-euler-weakscale-isentropic-fixcr}
\end{figure}

What would happen if we fix timestep size $dt$ instead of Courant number $Cr$? 
By refining the mesh, we add geometrically-induced stiffness to the system,
which causes the total number of Krylov steps to grow. 
This is why we see the wallclock time tends to increase with the number of degrees-of-freedom for a fixed $dt$ 
in Figure \figref{expo-euler-weakscale-isentropic-fixdt}. 
The corresponding total number of Krylov steps are summarized in 
Table \tabref{expo-euler-weakscale-isentropic-fixdt}.
As we refine the mesh by a factor of two along $x$, $y$, and $z-$direction,
the total number of Krylov steps tends to linearly increase for $dt=0.25$ and $dt=2.5$. 
%That is, we add geometrically-induced stiffness to the system.
%We can consider the total number of Krylov steps as an indicator of stiffness in the system. 
%One of the attractive feature of the adaptive Krylov subspace method is that 
%the stiffness is automatically detected and handled by adding more substeps or increasing the dimension of Krylov subspace methods.

\begin{figure}[h!t!b!]
  \centering
  \includegraphics[trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true,width=0.8\textwidth]{./figures/EXPO-euler-weakscale-fixedDt} 
  \caption{Isentropic vortex translation in three dimensions: 
    weak scaling study with a fixed timestep size.
    The computational domain is discretized with $N_e = \LRc{100, 800, 6400, 51200}$ and $k=8$ solution order for $n_p=\LRc{4,32,256,2048}$, respectively,
    so that each processor has 25 elements. }
  \figlab{expo-euler-weakscale-isentropic-fixdt}
\end{figure}



\begin{table}[t]
\caption{Isentropic vortex translation in three dimensions:
  the total number of Krylov steps, $N_{Krylov}$, approximately linearly depends on Courant number for $dt=0.25$ and $dt=2.5$. 
}
\tablab{expo-euler-weakscale-isentropic-fixdt}
\begin{center}
\begin{tabular}{c||cc|cc|cc|cc}
\hline
\multirow{2}{*}{$dt$} 
& \multicolumn{2}{c|}{$N_e=100$}  
& \multicolumn{2}{c|}{$N_e=800$} 
& \multicolumn{2}{c|}{$N_e=6400$} 
& \multicolumn{2}{c}{$N_e=51200$}   \tabularnewline
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$ 
          &  $Cr$ &  $N_{Krylov}$\tabularnewline
 \hline\hline
 0.025 & 0.7   & 40     & 1.4    & 40    & 2.8       & 45    & 5.6     & 81  \tabularnewline
 0.25  &  7.0  & 128   & 14.0 & 233   & 27.9.    &448   & 55.9   & 1024 \tabularnewline
 2.5    & 69.8 & 1536 &139.7 & 3072 &279.32 &5120 & 558.7 & 10112 \tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}




==> NumericalResults_steepgrad.tex <==
 

% 9.11.2020 remove steep gradient section
\subsubsection{A solution with steep gradient}

We next consider a solution with steep gradient,
% \shinhoo{The temporal convergence results are nice. Can you also plot spatial convergence for this case as well? This will give us a complete picture of space-time convergence for this steep gradient problem.}
namely, a stationary shock that evolves in time from the following
% %due to the nonlinearity of the convection term in \eqnref{pde-burgers-eq}.
%  This is well-known for the nonlinear conservation laws,
% which admit discontinuous solutions within finite time,
% even if the initial solutions are smooth.
% The
initial condition % is chosen to be
\begin{align*}
  u(x,t=0) = \sin(2\pi x), \quad \text{ for } x \in [0,1],
\end{align*}
% for $x \in [0,1]$
and  homogeneous boundary conditions.
We %take $\kappa=0.001$ for regularizing solutions and 
 perform the simulation for $t \in [0, 1]$ with $k = 4$ and $N_e = 40$.
 As time goes on a sharp interface is progressively formed at $x=0.5$. 
Below, we take $\kappa = 0.002$ so that the diffusion effect is small and  all the meshes are chosen to align with the sharp interface.
%and is diffused due to the presence of the diffusion term via positive $\kappa$. %(see Figure \figref{pde-burgers-ex-stationary-shock-all-kappa}).
% so that no additional capturing tool is needed. % DG methods effectively handle the discontinuity.
 %Also, we use positive $\kappa$ to regularize the shock solutions. 
% Due to the presence of $\kappa$

%-------------------------
% EXAMPLES FOR BURGERS EQ.
% % %-------------------------
% % \begin{figure}[h!t!b!]
% %     \centering
% %     \subfigure[solutions]{
% %       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-all}
% %       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Burgers-ex-sShock-kappa}
% %       \figlab{pde-burgers-ex-stationary-shock-all-kappa}
% %     }
% %     \subfigure[differences]{
% %       % \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Bugers-ex-shock-difference}
% %       \includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,clip=true,width=0.4\textwidth]{./figures/EXPO-Burgers-ex-sShock-kappa-difference}
% %       \figlab{pde-burgers-ex-stationary-shock-difference-kappa}
% %     }
% %     \caption{Burgers equation with a steep gradient solution with EPI2 time integrator, $k=4$, and $N_e=40$: Figure 
% %     \figref{pde-burgers-ex-stationary-shock-all-kappa}
% %      presents solutions with EF flux at $t=1$ for three different values of  $\kappa\in \LRc{0.02,0.005,0.002}$, 
% %      \shinhoo{Can we superimpose  Figure 
% %     \figref{pde-burgers-ex-stationary-shock-all-kappa} with the LF solutions (with symbols)? That would give me and the readers on the perspective how the LF solution looks like.}
% %      and Figure \figref{pde-burgers-ex-stationary-shock-difference-kappa}
% %     shows the differences between solutions with LF and EF ($\sigma=10^{-3}$) fluxes.
% %     \shinhoo{Can we plot relative pointwise error here instead? It is not clear to me if the EF solution is more oscillatory or the RK one is as $\kappa$ decreases, that is, how do you know if the large deviation between EF and LF is due to "the fact" that EF is more wrong than LF?}
% %     }
% %     \figlab{pde-burgers-stationary-shock-kappa}
% %   \end{figure} 

% % To understand the behavior of EF flux, 
% In Figure \figref{pde-burgers-stationary-shock-kappa} are the solution snapshots at $t=1$ with $\kappa\in \LRc{0.02,0.005,0.002}$ and $dt=0.01$ with EPI2 time integrator.  Figure 
%     \figref{pde-burgers-ex-stationary-shock-all-kappa}
%      presents solutions with EF flux ($\sigma=10^{-3}$) for three different values of  $\kappa\in \LRc{0.02,0.005,0.002}$, 
%      and Figure \figref{pde-burgers-ex-stationary-shock-difference-kappa}
%     shows the differences between solutions with LF and EF ($\sigma=10^{-3}$) fluxes. As can be seen, as $\kappa$ decreases the corresponding solution is less smooth (i.e. steeper gradient)
    
% In Figure \figref{pde-burgers-stationary-shock-kappa} are the solution snapshots at $t=1$ with $\kappa\in \LRc{0.02,0.005,0.002}$ and $dt=0.01$.
% By decreasing $\kappa$, the shock solutions with EF ($\sigma=10^{-3}$) flux become stiffer, 
% and the difference of EPI2 solutions between LF flux and EF flux increases. 
% Note that LF flux is based on upwinding, where
% the penalty term $\half \max (|u^\pm|) \jump{u}$ takes into account the flow direction. 
% Similarly, the additional stabilization term (in terms of $\sigma$) in EF flux
% can mimic the upwinding feature.

%To examine the sensitivity for $\sigma$, 
For spatial convergence, we use nested meshes with $N_e=\LRc{40,80,160}$ and the
EXPRB32 integrator with $\dt=5\times 10^{-5}$.
%we perform a spatial convergence study with 
We consider LF, EF ($\sigma=10^{-3}$), and EF ($\sigma=0$) fluxes. 
% This may be caused by 
% the fact that .
% the lack of upwinding nature of EF flux. 
% The free parameter $\sigma/h$ in EF flux helps 
% whereas the 
% This difference between two fluxes are small for diffusion-dominated problems, 
% but it can matter when the problem becomes convection-dominated. 
% Since the numerical solution with $\kappa=0.02$ is smooth enough in Figure 
% \figref{pde-burgers-stationary-shock-kappa}, 
% we focus on the case with $\kappa=0.002$.
% % \shinhoo{I know that you like to cover different values of $\kappa$,
%   which what we should do in general. However, in this case, the large
% $\kappa$ corresponds to smooth solution, which was already covered
% above? Thus it may not be necessary to cover this case here unless I
% miss something. Note that we like to consider steep gradient case
% here and we should focus on it. This also cut down the writing space
% (including tables and figures) significantly while making the message focused.}
%\shinhoo{I cannot find the convergence in time, why do you have many time steps here? Similarly, I don't understand which time step you used for Table 1, though you listed all timne steps there?}
RK4 solution (with LF flux, $\dt=5\times 10^{-7}$,  $k=10$, and
$N_e=160$) is used as the "ground truth"
% \shinhoo{which flux is used for the reference RK4 solution?}
solution for measuring the $L^2$ error at
$t=1$. For this steep gradient scenario, unless the solution is well-resolved or sufficient artificial diffusion/stabilization is employed, aliasing errors can affect the stability and accuracy.
% \shinhoo{We have  an inconsistency problem here: first for temporal
%   convergence study, we take $t = 1$, but now $t = 0.5$ for spatial
%   convergence. Second, $t = 1$ seems to lead to steep gradient
%   problem, which is what we like to focus our study in this
%   section. Do we have steep gradient solution for $t=0.5$? if not, I
%   am sorry, but we have to rerun the all the numerical results with $t
% = 1$.}
Indeed, as can be seen in Table \tabref{expo-burgers-sconv-shock},
%we observe 
%that the convergence rates for odd solution orders are sub-optimal, 
%but optimal for even solution orders when $\kappa_1=0.02$.
%However, 
%when $\kappa=0.002$, 
% we see the difference between LF and EF fluxes. 
solutions using EF ($\sigma=0$, i.e. no artificial diffusion) flux are unstable most of the cases, while  those using EF ($\sigma=10^{-3}$, i.e. small artificial diffusion) flux are stable and high-order accurate except for the case with $k = 1$ and $h = 1/40$, for which small added stabilization via $\sigma = 10^{-3}$ is not sufficient to combat the growth of aliasing errors.
%has a larger error and shows unstable behavior compared to 
%LF and EF($\sigma=10^{-3}$) fluxes. 
%In particular, EF($\sigma=0$) flux leads to blow up in several cases (denoted by x in Table \tabref{expo-burgers-sconv-shock}).
%EF($\sigma=10^{-3}$) flux, however, significantly improves the accuracy and stability.
%Except for the case with $k=1$ and $h=1/40$, 
%EF($\sigma=10^{-3}$) flux shows similar behavior to LF flux. 
%Indeed 
%introducing positive $\sigma$ makes the simulation stable and comparable to LF flux counterpart, 
%especially when a problem is convection-dominated.
%However, there is a difficulty to determine the proper value of $\sigma$
%(here, we empirically find $\sigma$). 
LF flux turns out to have sufficient artificial diffusion to stabilize the solutions for all cases, though (a little) less accurate than  EF flux with ($\sigma=10^{-3}$ in most cases.






\begin{table}[h!t!b!]
\caption{A shock solution to the viscous Burgers equation with %$\kappa=2 \times 10^{-3}$:
a spatial convergence study using  $N_e=\LRc{40,80,160}$ elements is conducted with Lax-Friedrich (LF) flux and entropy flux (EF), and
EXPRB32 scheme with $\dt=5\times 10^{-5}$ as the time integrator.
We take the RK4 solution (with $\dt=5\times 10^{-7}$,  $k=10$, and
$N_e=160$) as a reference solution to measure the $L^2$ error at
$t=1$. Here, "x" denotes "blow-up" solution.
\shinhoo{It is interesting to see that EF with $\sigma = 0$ is superconvergent when it converges. Please check to make sure the number is correct. I would think that $k=3$ and $h = 1/80$ would converge because  $k=2$ and $h = 1/80$ does? }
\tanbui{I have checked it, but this is what I got. }
}
% \shinhoo{Unless there is a message for smooth solution with $\kappa =
%   0.02$ that we haven't covered in the smooth solution example, we can
%   remove the results with  $\kappa =
%   0.02$.}
% }
\tablab{expo-burgers-sconv-shock}
\begin{center}
\begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
\hline
\multirow{2}{*}{ } 
% $\kappa$
  & \multirow{2}{*}{$h$}  
  & \multicolumn{2}{c|}{$LF$}   
  & \multicolumn{2}{c|}{$EF (\sigma=10^{-3})$}   
  & \multicolumn{2}{c}{$EF (\sigma=0)$}   
  \tabularnewline
  &    &  error & order &  error & order &  error & order       \tabularnewline
\hline\hline
% \multirow { 3}{*}{  $k=2$ }&  1/40  & 9.012E-05 &      $-$ & 8.586E-05 &      $-$ & 8.777E-05 &      $-$ \tabularnewline
%                            &  1/80  & 9.606E-06 &    3.230 & 9.588E-06 &    3.163 & 9.594E-06 &    3.194 \tabularnewline
%                            &  1/160 & 1.173E-06 &    3.034 & 1.172E-06 &    3.032 & 1.173E-06 &    3.033 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=3$ }&  1/40  & 1.117E-05 &      $-$ & 1.092E-05 &      $-$ & 1.142E-05 &      $-$ \tabularnewline
%                            &  1/80  & 1.221E-06 &    3.194 & 1.157E-06 &    3.239 & 1.355E-06 &    3.075 \tabularnewline
%                            &  1/160 & 1.343E-07 &    3.185 & 1.068E-07 &    3.437 & 1.671E-07 &    3.020 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=4$ }&  1/40  & 4.900E-07 &      $-$ & 4.650E-07 &      $-$ & 5.187E-07 &      $-$ \tabularnewline
%                            &  1/80  & 1.051E-08 &    5.544 & 1.049E-08 &    5.471 & 1.050E-08 &    5.627 \tabularnewline
%                            &  1/160 & 3.122E-10 &    5.073 & 3.121E-10 &    5.070 & 3.122E-10 &    5.072 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
\multirow { 3}{*}{ $k=1$ }& 1/40 & 1.295E-02 &      $-$ &    x      &      $-$ &     x    &      $-$ \tabularnewline
                         & 1/80  & 5.558E-03 &    1.221 & 5.662E-03 &      $-$ &     x    &      $-$ \tabularnewline
                         & 1/160 & 2.001E-03 &    1.474 & 1.986E-03 &    1.512 &     x    &      $-$ \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 3}{*}{ $k=2$ }& 1/40  & 4.223E-03 &      $-$ & 4.239E-03 &      $-$ &         x &      $-$ \tabularnewline
                         &  1/80  & 6.722E-04 &    2.651 & 6.698E-04 &    2.662 & 5.163E-03 &      $-$ \tabularnewline
                         &  1/160 & 9.852E-05 &    2.770 & 8.481E-05 &    2.981 & 2.705E-04 &    4.255 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 3}{*}{ $k=3$ }& 1/40  & 9.976E-04 &      $-$ & 1.014E-03 &      $-$ &     x     &      $-$ \tabularnewline
                          & 1/80  & 1.435E-04 &    2.797 & 1.326E-04 &    2.935 &     x     &      $-$ \tabularnewline
                          & 1/160 & 1.224E-05 &    3.551 & 1.079E-05 &    3.619 & 9.626E-05 &      $-$ \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
\multirow { 3}{*}{ $k=4$ }& 1/40  & 3.606E-04 &      $-$ & 3.550E-04 &      $-$ & 1.335E-03 &      $-$ \tabularnewline
                          & 1/80  & 2.728E-05 &    3.724 & 2.471E-05 &    3.844 & 3.649E-04 &    1.871 \tabularnewline
                          & 1/160 & 8.084E-07 &    5.077 & 6.904E-07 &    5.162 & 1.613E-06 &    7.821 \tabularnewline
\multicolumn{8}{c}{} \tabularnewline
% \hline
% \multirow{2}{*}{$\kappa_2$}
%   & \multirow{2}{*}{$h$}  
%   & \multicolumn{2}{c|}{$LF$}   
%   & \multicolumn{2}{c|}{$EF (\sigma=10^{-3})$}   
%   & \multicolumn{2}{c}{$EF (\sigma=0)$}   
%   \tabularnewline
%   &    &  error & order &  error & order &  error & order       \tabularnewline
%   \hline\hline
% \multirow { 3}{*}{  $k=2$ }&  1/40  & 1.286E-02 &      $-$ & 1.284E-02 &      $-$ & 1.210E-01 &      $-$ \tabularnewline
%                            &  1/80  & 3.980E-03 &    1.692 & 3.981E-03 &    1.689 & 7.875E-03 &    3.942 \tabularnewline
%                            &  1/160 & 5.505E-04 &    2.854 & 5.438E-04 &    2.872 & 1.096E-03 &    2.845 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=3$ }&  1/40  & 5.327E-03 &      $-$ & 5.332E-03 &      $-$ &    $-$    &      $-$ \tabularnewline
%                            &  1/80  & 8.078E-04 &    2.721 & 8.264E-04 &    2.690 & 2.664E-03 &      $-$ \tabularnewline
%                            &  1/160 & 1.145E-04 &    2.819 & 1.042E-04 &    2.988 & 1.529E-04 &    4.123 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=4$ }&  1/40  & 1.873E-03 &      $-$ & 1.918E-03 &      $-$ & 2.560E-03 &      $-$ \tabularnewline
%                            &  1/80  & 3.135E-04 &    2.579 & 2.979E-04 &    2.687 & 4.700E-04 &    2.445 \tabularnewline
%                            &  1/160 & 1.389E-05 &    4.496 & 1.263E-05 &    4.559 & 2.646E-05 &    4.151 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
\hline\hline
\end{tabular}
\end{center}
\end{table}



For temporal convergence study, %we take $\kappa=\LRc{2\times 10^{-2},
  %5\times 10^{-3}, 2\times 10^{-3}}$ and 
  we consider
the EPI2 DG discretization using both LF and EF fluxes, $k=4$, and $N_e=160$.
We take the RK4 solution (with LF flux, $\dt=5\times 10^{-7}$,  $k=10$, and
$N_e=160$) as a reference solution to  measure the $L^2$ error at $t=1$.
%Spatial discretization is carried out using our DG approach with $k=4$ and $N_e=160$. 
%As can be seen from
Table \tabref{expo-burgers-tconv-shock} shows that
except for the case with EF ($\sigma=10^{-3}$),
we observe second- and third-order convergence rates for EPI2
and EXPRB32, respectively.
This is interesting because 
the case with $k=4$, $h=1/160$, $\dt=5\times 10^{-5}$ and EF ($\sigma=10^{-3}$) was stable in Table \tabref{expo-burgers-sconv-shock}. 
\shinhoo{This is actually not interesting as I don't know how to explain it :-). I need to talk to you a bit on this case to finish this section.}
With several numerical experiments, we found that 
increasing $\dt$ makes the solution unstable.
To address the issue, 
we take EF ($\sigma=10^{-3}\times dt$) flux, which leads to stable solutions. 

\begin{table}[h!t!b!]
\caption{Temporal convergence study of EPI2 and EXPRB32 for a shock solution to the viscous Burgers equation:
we take the RK4 solution (with LF flux, $\dt=5\times 10^{-7}$,  $k=10$, and
$N_e=160$) as a reference solution, and measure the $L^2$ error at $t=1$.
Spatial discretization is carried out using our DG approach with $k=4$ and $N_e=160$. 
Except the case with EF ($\sigma=10^{-3}$),
we observe second- and third-order convergence rates for EPI2
and EXPRB32, respectively.}
\tablab{expo-burgers-tconv-shock}
\begin{center}
%\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
\begin{tabular}{c|cc||cc|cc}
\hline
\multirow{2}{*}{flux} 
& \multirow{2}{*}{$\dt$} 
& \multirow{2}{*}{$Cr$} 
& \multicolumn{2}{c|}{ EPI2 } 
& \multicolumn{2}{c}{ EXPRB32 } \tabularnewline
&  &  &  error & order & error & order \tabularnewline
\hline\hline
% crset = [ 559.14, 213.25, 105.48, 41.96, 20.94] % at T=1
% crdset = [ 429.30, 171.72, 85.86,  42.93, 24.34,  17.17]
\multirow{5}{*}{LF} 
  % LF flux
  & 0.25 & 559.1 &   2.276E-02 &      $-$ &       8.424E-03 &      $-$ \tabularnewline
  & 0.10 & 213.3 &   3.706E-03 &    1.981 &       5.711E-04 &    2.937 \tabularnewline
  & 0.05 & 105.5 &   8.784E-04 &    2.077 &       6.440E-05 &    3.149 \tabularnewline
  & 0.02 & 42.0  &   1.327E-04 &    2.063 &       3.755E-06 &    3.102 \tabularnewline
  % & 0.01 & 20.9  &   3.242E-05 &    2.033 &       7.331E-07 &    2.357 \tabularnewline #reference solution uses dt=1e-7
  \\
\multirow{5}{*}{EF\small{($\sigma=10^{-3}$)}}   
  & 0.25 & 559.1 &    2.276E-02 &      $-$ &       8.424E-03 &      $-$ \tabularnewline
  & 0.10 & 213.3 &    3.706E-03 &    1.981 &       1.232E-02 &   -0.415 \tabularnewline
  & 0.05 & 105.5 &    1.693E-02 &   -2.192 &       2.039E-02 &   -0.727 \tabularnewline
  & 0.02 & 42.0  &    2.200E-02 &   -0.286 &       3.255E-02 &   -0.511 \tabularnewline
  % & 0.01 & 20.9  &    2.136E-02 &    0.043 &       1.124E-02 &    1.534 \tabularnewline #reference solution uses dt=1e-7
 \\
\multirow{5}{*}{EF\small{($\sigma=10^{-3}\times \dt$)}}
 & 0.25 & 559.1 &   2.276E-02 &      $-$ &       8.424E-03 &      $-$ \tabularnewline
 & 0.10 & 213.3 &   3.706E-03 &    1.981 &       5.711E-04 &    2.937 \tabularnewline
 & 0.05 & 105.5 &   8.784E-04 &    2.077 &       6.440E-05 &    3.148 \tabularnewline
 & 0.02 & 42.0  &   1.327E-04 &    2.063 &       3.879E-06 &    3.066 \tabularnewline
 % & 0.01 & 20.9  &   3.243E-05 &    2.032 &       1.674E-06 &    1.212 \tabularnewline #reference solution uses dt=1e-7
 \\ 
\multirow{5}{*}{EF\small{($\sigma=0$)}}    
  & 0.25 & 559.1 &  2.276E-02 &      $-$ &       8.424E-03 &      $-$ \tabularnewline
  & 0.10 & 213.3 &  3.706E-03 &    1.981 &       5.711E-04 &    2.937 \tabularnewline
  & 0.05 & 105.5 &  8.784E-04 &    2.077 &       6.440E-05 &    3.148 \tabularnewline
  & 0.02 & 42.0  &  1.327E-04 &    2.063 &       3.933E-06 &    3.051 \tabularnewline
  % & 0.01 & 20.9  &  3.244E-05 &    2.032 &       2.296E-06 &    0.777 \tabularnewline #reference solution uses dt=1e-7
\hline\hline
\end{tabular}
\end{center}
\end{table} 





% \shinhoo{is it with $dt=5\times 10^{-6}$ as above and EF flux? if yes
%   please write these out as this is a different example, and hence
%   different reference solution, and it is worth
% to repeat.}
% However, as solutions become less regular by reducing $\kappa$, 
% the convergence rate of EPI2 with EF flux and $dt=0.01$ decreases.
% \shinhoo{We see the good convergence for EF before and I am trying to understand why EF flux is bad in this
%   case and I am still struggling with convergence loss with the
%   smallest $dt = 0.01$, which
%   corresponds to supposedly the most accurate simulation. Perhaps due to the reference
%   RK4 solution or the little extra diffusion from $\sigma$ smears out
%   the solution and hence making it less accurate? 1) did you use EF or LF flux for
% the reference solution? 2) do you see the same problem for EF flux
% with $\sigma = 0$? Note that both LF and EF face the same regularity
% problem. Looking at the results in figure
% \figref{pde-burgers-stationary-shock-kappa}, I do see steep
% gradient. I think it is a good idea to plot the reference RK4 solution
% to visually see what happens. }


% \begin{table}[h!t!b!]
% \caption{A time convergence study for EPI2 using both LF and EF fluxes
%   for a steep gradient solution. Numerical experiments are conducted
%   with $k=4$ (the solution order) and $N_e=40$ (the number of elements). 
% With three values of $\kappa$, i.e. $\kappa=\LRc{2\times 10^{-2},
%   5\times 10^{-3}, 2\times 10^{-3}}$, EPI2 solutions with both LF and
% EF fluxes show the second-order convergence rates except for EF flux
% with
% $\kappa = 2\times 10^{-3}$.
% %the convergence rate of EPI2 with EF flux and $dt=0.01$ decreases.
% }
% \tablab{expo-burgers-tconv-shock}
% \begin{center}
% %\begin{tabular}{*{1}{c}|*{2}{c}|*{2}{c}}
% \begin{tabular}{c|cc||cc|cc}
% \hline
% \multirow{2}{*}{$\kappa$} 
% & \multirow{2}{*}{$dt$} 
% & \multirow{2}{*}{$Cr_d$} 
% & \multicolumn{2}{c|}{ LF } 
% & \multicolumn{2}{c}{ EF ($\sigma=10^{-3}$) } \tabularnewline
%   & &  &  error & order & error & order \tabularnewline
% \hline\hline
% \multirow{4}{*}{$2\times10^{-2}$}  
%   & 0.25 & 268.31 &      1.075E-02 &      $-$ &   1.075E-02 &      $-$  \tabularnewline
%   & 0.10 & 107.33 &      1.803E-03 &    1.949 &   1.803E-03 &    1.949  \tabularnewline
%   & 0.05 &  53.66 &      4.472E-04 &    2.011 &   4.472E-04 &    2.011  \tabularnewline
%   & 0.01 &  10.73 &      1.741E-05 &    2.017 &   1.741E-05 &    2.017  \tabularnewline
% \\
% \multirow{4}{*}{$5\times10^{-3}$} 
%   % & 0.25 &  67.08  &     2.030E-02 &      $-$ &   2.031E-02 &      $-$ \tabularnewline % sigma=k/100
%   % & 0.10 &  26.83  &     3.303E-03 &    1.982 &   3.304E-03 &    1.982 \tabularnewline
%   % & 0.05 &  13.42  &     7.928E-04 &    2.059 &   7.928E-04 &    2.059 \tabularnewline
%   % & 0.01 &   2.68  &     3.136E-05 &    2.007 &   4.864E-05 &    1.734 \tabularnewline
%   & 0.25 &  67.08  &     2.030E-02 &      $-$ &    2.030E-02 &     $-$  \tabularnewline %sigma=0.001
%   & 0.10 &  26.83  &     3.303E-03 &    1.982 &    3.303E-03 &    1.982 \tabularnewline
%   & 0.05 &  13.42  &     7.928E-04 &    2.059 &    7.927E-04 &    2.059 \tabularnewline
%   & 0.01 &   2.68  &     3.136E-05 &    2.007 &    3.108E-05 &    2.012 \tabularnewline  
% \\
% \multirow{4}{*}{$2\times10^{-3}$}   
%   % & 0.25 & 26.83 &       1.201E-02 &      $-$  &  2.276E-02 &      $-$  \tabularnewline % sigma=k/100
%   % & 0.10 & 10.73 &       1.648E-03 &    2.167  &  3.720E-03 &    1.977  \tabularnewline
%   % & 0.05 &  5.37 &       3.656E-04 &    2.173  &  8.945E-04 &    2.056  \tabularnewline
%   % & 0.01 &  1.07 &       1.299E-05 &    2.074  &  3.550E-04 &    0.574  \tabularnewline
%   & 0.25 & 26.83 &       1.201E-02 &      $-$  &  2.276E-02 &      $-$  \tabularnewline %sigma=0.001
%   & 0.10 & 10.73 &       1.648E-03 &    2.167  &  3.708E-03 &    1.980  \tabularnewline
%   & 0.05 &  5.37 &       3.656E-04 &    2.173  &  9.038E-04 &    2.037  \tabularnewline
%   & 0.01 &  1.07 &       1.299E-05 &    2.074  &  1.836E-04 &    0.990  \tabularnewline  
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table} 





% \begin{table}[h!t!b!]
% \caption{A shock solution to the viscous Burgers equation for $\kappa=0.002$:
% a temporal convergence study for EPI2 using $dt=\LRc{0.25, 0.1, 0.05, 0.02,0.01}$.
% Lax-Friedrich (LF) flux and entropy flux (EF) are compared. 
% Spatial discretization is carried out using our DG approach with $k=4$ and $N_e = 80$.
% We take the RK4 solution (with $dt=5\times 10^{-7}$,  $k=10$, and
% $N_e=80$) as a reference solution, and measure the $L^2$ error at $t=1$.}
% \tablab{expo-burgers-tconv-shock}
% \begin{center}
% \begin{tabular}{*{2}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
% \hline
% \multirow{2}{*}{$dt$} 
%   & \multirow{2}{*}{$Cr$}  
%   & \multicolumn{2}{c|}{$LF$}   
%   & \multicolumn{2}{c|}{$EF (\sigma=10^{-3})$}   
%   & \multicolumn{2}{c}{$EF (\sigma=0)$}   
%   \tabularnewline
%   &    &  error & order &  error & order &  error & order       \tabularnewline
% \hline\hline
%   0.25 & 172.2 &   1.201E-02 &      $-$ &       2.276E-02 &      $-$ &       2.277E-02 &      $-$ \tabularnewline
%   0.10 & 63.7  &   1.648E-03 &    2.167 &       3.706E-03 &    1.981 &       3.708E-03 &    1.981 \tabularnewline
%   0.05 & 31.3  &   3.656E-04 &    2.173 &       8.786E-04 &    2.077 &       8.791E-04 &    2.076 \tabularnewline
%   0.02 & 12.4  &   5.358E-05 &    2.096 &       1.343E-04 &    2.050 &       1.358E-04 &    2.039 \tabularnewline
%   0.01 & 6.2   &   1.299E-05 &    2.045 &       3.875E-05 &    1.793 &       7.747E-05 &    0.809 \tabularnewline
%   %         Crd
%   % 0.25 & 107.3 &   1.201E-02 &      $-$ &       2.276E-02 &      $-$ &       2.277E-02 &      $-$ \tabularnewline
%   % 0.10 & 42.9  &   1.648E-03 &    2.167 &       3.706E-03 &    1.981 &       3.708E-03 &    1.981 \tabularnewline
%   % 0.05 & 21.5  &   3.656E-04 &    2.173 &       8.786E-04 &    2.077 &       8.791E-04 &    2.076 \tabularnewline
%   % 0.02 & 8.6   &   5.358E-05 &    2.096 &       1.343E-04 &    2.050 &       1.358E-04 &    2.039 \tabularnewline
%   % 0.01 & 4.3   &   1.299E-05 &    2.045 &       3.875E-05 &    1.793 &       7.747E-05 &    0.809 \tabularnewline
% % \multirow { 3}{*}{ $k=1$ }& 1/40 & 1.295E-02 &      $-$ &    x      &      $-$ &     x    &      $-$ \tabularnewline
% %                          & 1/80  & 5.558E-03 &    1.221 & 5.662E-03 &      $-$ &     x    &      $-$ \tabularnewline
% %                          & 1/160 & 2.001E-03 &    1.474 & 1.986E-03 &    1.512 &     x    &      $-$ \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% % \multirow { 3}{*}{ $k=2$ }& 1/40  & 4.223E-03 &      $-$ & 4.239E-03 &      $-$ &         x &      $-$ \tabularnewline
% %                          &  1/80  & 6.722E-04 &    2.651 & 6.698E-04 &    2.662 & 5.163E-03 &      $-$ \tabularnewline
% %                          &  1/160 & 9.852E-05 &    2.770 & 8.481E-05 &    2.981 & 2.705E-04 &    4.255 \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% % \multirow { 3}{*}{ $k=3$ }& 1/40  & 9.976E-04 &      $-$ & 1.014E-03 &      $-$ &     x     &      $-$ \tabularnewline
% %                           & 1/80  & 1.435E-04 &    2.797 & 1.326E-04 &    2.935 &     x     &      $-$ \tabularnewline
% %                           & 1/160 & 1.224E-05 &    3.551 & 1.079E-05 &    3.619 & 9.626E-05 &      $-$ \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% % \multirow { 3}{*}{ $k=4$ }& 1/40  & 3.606E-04 &      $-$ & 3.550E-04 &      $-$ & 1.335E-03 &      $-$ \tabularnewline
% %                           & 1/80  & 2.728E-05 &    3.724 & 2.471E-05 &    3.844 & 3.649E-04 &    1.871 \tabularnewline
% %                           & 1/160 & 8.084E-07 &    5.077 & 6.904E-07 &    5.162 & 1.613E-06 &    7.821 \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}



% \begin{table}[t]
% \caption{%A shock solution to the viscous Burgers equation with $\kappa=2\times 10^{-3}$:
% Same as Table \tabref{expo-burgers-sconv-shock-bigKappa} except $\kappa=2\times 10^{-3}$. }
% % a spatial convergence study using  $N_e=\LRc{40,80,160}$ elements is conducted with Lax-Friedrich (LF) flux and entropy flux (EF), and
% % EXPRB32 scheme with $dt=5\times 10^{-5}$ as the time integrator.
% % We take the RK4 solution (with $dt=5\times 10^{-7}$,  $k=10$, and
% % $N_e=160$) as a reference solution, and measure the $L^2$ error at $t=0.5$.}
% \tablab{expo-burgers-sconv-shock-smallKappa}
% \begin{center}
% \begin{tabular}{*{1}{c}|*{1}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
% \hline
% \multirow{2}{*}{} 
% % $\kappa$
%   & \multirow{2}{*}{$h$}  
%   & \multicolumn{2}{c|}{$LF$}   
%   & \multicolumn{2}{c|}{$EF (\sigma=10^{-3})$}   
%   & \multicolumn{2}{c}{$EF (\sigma=0)$}   
%   \tabularnewline
%   &    &  error & order &  error & order &  error & order       \tabularnewline
% \hline\hline
% \multirow { 3}{*}{  $k=2$ }&  1/40  & 1.286E-02 &      $-$ & 1.284E-02 &      $-$ & 1.210E-01 &      $-$ \tabularnewline
%                            &  1/80  & 3.980E-03 &    1.692 & 3.981E-03 &    1.689 & 7.875E-03 &    3.942 \tabularnewline
%                            &  1/160 & 5.505E-04 &    2.854 & 5.438E-04 &    2.872 & 1.096E-03 &    2.845 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=3$ }&  1/40  & 5.327E-03 &      $-$ & 5.332E-03 &      $-$ & 0.000E+00 &      $-$ \tabularnewline
%                            &  1/80  & 8.078E-04 &    2.721 & 8.264E-04 &    2.690 & 2.664E-03 &     -Inf \tabularnewline
%                            &  1/160 & 1.145E-04 &    2.819 & 1.042E-04 &    2.988 & 1.529E-04 &    4.123 \tabularnewline
% \multicolumn{8}{c}{} \tabularnewline
% \multirow { 3}{*}{  $k=4$ }&  1/40  & 1.873E-03 &      $-$ & 1.918E-03 &      $-$ & 2.560E-03 &      $-$ \tabularnewline
%                            &  1/80  & 3.135E-04 &    2.579 & 2.979E-04 &    2.687 & 4.700E-04 &    2.445 \tabularnewline
%                            &  1/160 & 1.389E-05 &    4.496 & 1.263E-05 &    4.559 & 2.646E-05 &    4.151 \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% % \multicolumn{8}{c}{} \tabularnewline
% \hline\hline
% \end{tabular}
% \end{center}
% \end{table}



% We %take $\kappa=0.001$ for regularizing solutions and 
%  perform the simulation for $t \in [0, 1]$ with $k = 4$ and $N_e = 40$.
%  We take the RK4 solution (with $dt=5\times 10^{-6}$,  $k=10$, and
% $N_e=40$) as a ground truth.
%  We measure the error at $t=1$.
%  In particular, for $\kappa=0.002$, we compute the error for $x=[0,1/4]\cup [3/4,1]$ to avoid shock region. 
%  Here, the shock (at $x=0.5$) is aligned with the mesh 
%  so that the DG methods effectively handle the discontinuity.
%  Also, we use positive $\kappa$ to regularize the shock solutions. 

% We conduct the temporal convergence with different $\kappa$ values 
% in Table \tabref{expo-burgers-tconv-shock}.
% For $\kappa=0.02$,
% both EPI2 solutions with LF and EF fluxes converge the reference RK4 solution with the second-order convergence rate.
% However, as solutions become less regular by reducing $\kappa$, 
% the convergence rate of EPI2 with EF flux and $dt=0.01$ decreases. 

% % Considering the small differences between two fluxes, %that these differences are not significant and 
Considering the simplicity and upwinding nature of Lax-Friedrich flux, 
we use Lax-Friedrich flux for Euler equations, which is hyperbolic equations,  
in the following examples.


 





==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
% \headers{A scalable exponential-DG approach for nonlinear conservation laws: with application to Burger and Euler equations}{Shinhoo Kang and Tan Bui-Thanh}
\headers{A scalable exponential-DG approach for nonlinear conservation laws}{S. Kang and T. Bui-Thanh}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A scalable exponential-DG approach for nonlinear conservation laws: with application to Burgers and Euler equations\thanks{Submitted to the editors DATE.
\funding{SK was partially supported by 
  the U.S. Department of Energy, Office of Science, Advanced Scientific Computing Research Program under contract DE-AC02-06CH11357. The work of TBT was funded in part by DOE grants DE-SC0010518 and DE-SC0011118, NSF Grant NSF-DMS1620352. We are grateful for the supports.}}}

% Authors: full names plus addresses.
\author{Shinhoo Kang\thanks{Mathematics and Computer Science Division, Argonne National Laboratory, Lemont, IL 60439, USA
  (\email{shinhoo.kang@anl.gov}).}
\and Tan Bui-Thanh\thanks{Department of Aerospace Engineering and Engineering Mechanics, Oden Institute for Computational Engineering And Sciences, The University of Texas at Austin, Austin, TX, USA
  (\email{tanbui@oden.utexas.edu}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> tbmacrosjcp.tex <==
% MY MACROs
\newcommand{\TODO}[1]{ \fbox{\parbox{3in}{\bf TODO: #1}}}

\newcommand{\grbf}[1] {\mbox{\boldmath${#1}$\unboldmath}}
%\renewcommand{\grbf}[1] {\mathbf{#1}}
\newcommand{\gbf}[1] {\mathbf{#1}}

%\renewcommand{\baselinestretch}{1.08}

\newcommand{\beq} {\begin{equation}}
\newcommand{\eeq} {\end{equation}}
\newcommand{\bdm} {\begin{displaymath}}
\newcommand{\edm} {\end{displaymath}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bde}{\begin{description}}
\newcommand{\ede}{\end{description}}
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
\newcommand{\ben} {\begin{enumerate}}
\newcommand{\een} {\end{enumerate}}
\newcommand{\bea} {\begin{eqnarray}}
\newcommand{\eea} {\end{eqnarray}}
\newcommand{\barr} {\begin{array}}
\newcommand{\earr} {\end{array}}
\newcommand{\bean} {\begin{eqnarray*}}
\newcommand{\eean} {\end{eqnarray*}}
\newcommand{\edoc} {\end{document}}
%\newcommand{\And}{\hspace{0.2cm} \mbox{and} \hspace{0.2cm}}
\newcommand{\On}{\hspace{0.2cm} \mbox{on} \hspace{0.2cm}}
%\newcommand{\Or}{\hspace{0.2cm} \mbox{or} \hspace{0.2cm}}
\newcommand{\In}{\hspace{0.2cm} \mbox{in} \hspace{0.2cm}}
%\newcommand{\For}{\hspace{0.2cm} \mbox{for} \hspace{0.2cm}}
\newcommand{\Minimize}{\hspace{0.2cm} \mbox{minimize} \hspace{0.2cm}}
\newcommand{\Maximize}{\hspace{0.2cm} \mbox{maximize} \hspace{0.2cm}}
\newcommand{\SubjectTo}{\hspace{0.2cm} \mbox{subject} \hspace{0.15cm}
            \mbox{to} \hspace{0.2cm}}

\def\etal{{\it et al.~}}

\newcommand{\point}[1] {\ensuremath{\boldsymbol{#1}}}
\newcommand{\vvec}[1] {\ensuremath{\boldsymbol{#1}}}
\renewcommand{\vec}[1] {\ensuremath{\boldsymbol{#1}}}
%\newcommand{\rvec}[1] {\ensuremath{\boldsymbol{\mathrm{#1}}}}
\newcommand{\cvec}[1] {\ensuremath{\boldsymbol{{#1}}}}
\newcommand{\ten}[1] {\ensuremath{\boldsymbol{#1}}}
\newcommand{\tenfour}[1] {\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\comp}[1]{\begin{pmatrix}{ #1 }\end{pmatrix}}
\newcommand{\vv}{\ensuremath{\vec{v}}}
\newcommand{\vr}{\left(\ensuremath{\vec{r}}\right)}
\newcommand{\att}{\left(t\right)}
\newcommand{\tvv}{\ensuremath{\tilde{\vec{v}}}}
\newcommand{\ww}{\ensuremath{\vec{w}}}
\newcommand{\GG}{\ensuremath{\ten{G}}}
\newcommand{\FF}{\ensuremath{\boldsymbol{\mathfrak{F}}}}
\newcommand{\tEE}{\ensuremath{\tilde{\vec{E}}}}
\newcommand{\nn}{\ensuremath{\vec{n}}}
\renewcommand{\SS}{\ensuremath{\ten{S}}}
\newcommand{\tSS}{\ensuremath{\tilde{\ten{S}}}}
\newcommand{\cp}{\ensuremath{{c_p}}}
\newcommand{\cs}{\ensuremath{{c_s}}}
%\newcommand{\tcp}{\ensuremath{{\tilde{c}_p}}}
\newcommand{\tcs}{\ensuremath{{\tilde{c}_s}}}
\newcommand{\Vp}{\ensuremath{{V^e_p}}}
\newcommand{\Vs}{\ensuremath{{V^e_s}}}
\newcommand{\Ss}{\ensuremath{{S^e_s}}}
\newcommand{\nxnx}[1] {\ensuremath{\nn\times\left(\nn\times{#1}\right)}}

\newcommand{\dd}[2] {\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\DD}[2] {\ensuremath{\frac{d {#1}}{d {#2}}}}
\newcommand{\Grad} {\ensuremath{\nabla}}
\newcommand{\Gradv}[1]{\ensuremath{\nabla_{#1}}}
\newcommand{\Div} {\ensuremath{\nabla\cdot}}
\newcommand{\Divv}[1] {\ensuremath{\nabla_{#1}\cdot}}
\newcommand{\Curl} {\ensuremath{\nabla\times}}
\newcommand{\Cten}{\ensuremath{\tenfour{C}}}

%    Notation for an expression evaluated at a particular condition. The
%    optional argument can be used to override automatic sizing of the
%    right vert bar, e.g. \eval[\biggr]{...}_{...}
\newcommand{\eval}[2][\right]{\relax
  \ifx#1\right\relax \left.\fi#2#1\rvert}

\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\Nel} {\ensuremath{{N_\text{el}}}}
\newcommand{\Ned} {\ensuremath{{N_\text{ed}}}}
\newcommand{\De} {\ensuremath{{\mathsf{D}^e}}}
\newcommand{\Dep} {\ensuremath{{\mathsf{D}^{e'}}}}
\newcommand{\Dhat} {\ensuremath{\hat{\mathsf{D}}}}
\newcommand{\Dehat} {\ensuremath{{\hat{\mathsf{D}}^e}}}
\newcommand{\half} {\ensuremath{\frac{1}{2}}}
\newcommand{\IN} {\ensuremath{{\mathcal{I}_N}}}
\newcommand{\INe} {\ensuremath{{\mathcal{I}_{N_e}}}}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mcC}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mi}[1]{\mathit{#1}}
% \newcommand{\mf}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\Oi}[1]{\int_{\mc{D}} #1 \, d\vec{x}}
\newcommand{\TOi}[1]{\int_{0}^T \int_{\mc{D}} #1 \, d\vec{x}dt}
\newcommand{\Ti}[1]{\int_{0}^T #1 \, dt}
\newcommand{\TDei}[1]{\int_{0}^T\int_{\De} #1 \, d\vec{x}dt}
\newcommand{\TDeid}[1]{\int_{0}^T\int_{\De,N} #1 \, d\vec{x}dt}
\newcommand{\Dei}[1]{\int_{\De} #1 \, d\vec{x}}
\newcommand{\DeI}[1]{\int_{D} #1 \, d\vec{x}}
\newcommand{\DeiM}[1]{\int_{\Dhat} #1 \, d\vec{r}}
\newcommand{\DeMd}[1]{\int_{\De,N_e} #1 \, d\vec{x}}
\newcommand{\DeiMd}[1]{\int_{\Dhat,N_e} #1 \, d\vec{r}}
\newcommand{\DeMdN}[1]{\int_{D,N} #1 \, d\vec{x}}
\newcommand{\DeiMdN}[1]{\int_{\Dhat,N} #1 \, d\vec{r}}
\newcommand{\DeiMdNC}[2]{\int_{\Dhat,N_{#2}} #1 \, d\vec{r}}
\newcommand{\pDei}[1]{\int_{\partial \De} #1 \, d\vec{x}}
\newcommand{\pDeiM}[1]{\int_{\partial \Dhat} #1 \, d\vec{r}}
\newcommand{\pDeiMd}[1]{\int_{\partial \Dhat,N_e} #1 \, d\vec{r}}
\newcommand{\pDeiMdN}[1]{\int_{\partial \Dhat,N} #1 \, d\vec{r}}
\newcommand{\pDeiMdNC}[2]{\int_{\partial \Dhat,N_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortar}[2]{\int_{\mc{M}_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortard}[2]{\int_{\mc{M}^{#2},N_{#2}} #1 \, d\vec{r}}
\newcommand{\pMortardd}[3]{\int_{\mc{M}^{#2},N_{#3}} #1 \, d\vec{r}}
\newcommand{\pMortardh}[3]{\int_{\mc{M}_{#2},N_{#3}} #1 \, d\vec{r}}
\newcommand{\pMortardhn}[4]{\int_{{#2}_{#3},N_{#4}} #1 \, d\vec{r}}
\newcommand{\TpDei}[1]{\int_{0}^T\int_{\partial \De} #1 \, d\vec{x}}
\newcommand{\TpDeid}[1]{\int_{0}^T\int_{\partial \De,N} #1 \, d\vec{x}}
\newcommand{\Deid}[1]{\int_{\De,N_e} #1 \, d\vec{x}}
\newcommand{\DeidN}[1]{\int_{\De,N} #1 \, d\vec{x}}
\newcommand{\pDeidN}[1]{\int_{\partial \De,N} #1 \, d\vec{x}}
\newcommand{\pDeid}[1]{\int_{\partial \De,N_e} #1 \, d\vec{x}}
\newcommand{\nor}[1]{\left\| #1 \right\|}
\newcommand{\snor}[1]{\left| #1 \right|}
\newcommand{\LRp}[1]{\left( #1 \right)}
\newcommand{\LRs}[1]{\left[ #1 \right]}
\newcommand{\LRa}[1]{\left< #1 \right>}
\newcommand{\LRc}[1]{\left\{ #1 \right\}}
\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppcp}[1]{\frac{\partial #1}{\partial \vec{c_p}}}
\newcommand{\ppcpj}[1]{\frac{\partial #1}{\partial c_p}}
\newcommand{\ppcpmf}[1]{\frac{\partial #1}{\partial \vec{\mf{c_p}}}}
\newcommand{\ppm}[1]{\frac{\partial #1}{\partial \vec{m}}}
\newcommand{\ppho}[3]{\frac{\partial^{#3} #1}{{\partial #2}^{#3}}}
\newcommand{\ppmi}[1]{\frac{\partial #1}{\partial m_i}}
\newcommand{\ppmj}[1]{\frac{\partial #1}{\partial m_j}}
\newcommand{\ppcpm}[1]{\frac{\partial #1}{\partial \vec{c_p}^-}}
\newcommand{\ppcpp}[1]{\frac{\partial #1}{\partial \vec{c_p}^+}}
\newcommand{\ppcs}[1]{\frac{\partial #1}{\partial \vec{c_s}}}
\newcommand{\ppcsm}[1]{\frac{\partial #1}{\partial \vec{c_s}^-}}
\newcommand{\ppcsp}[1]{\frac{\partial #1}{\partial \vec{c_s}^+}}
\newcommand{\td}[2]{\frac{d #1}{d #2}}
\newcommand{\Rvert}[1]{\left. #1 \right|}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\ipDed}[3]{\LRp{ #1, #2}_{\De,N}^{#3}}

\newcommand{\bigO}{\mathcal{O}}
%\newcommand{\supp}{\text{supp}}

\newcommand{\iOm}[1]{\int_{\Omega} #1 \, d\Omega}
\newcommand{\iGb}[1]{\int_{\Gamma_{b}} #1 \, ds}
\newcommand{\iGs}[1]{\int_{\Gamma_{s}} #1 \, ds}
\newcommand{\iGsy}[1]{\int_{\Gamma_{s}} #1 \, ds(\mb{y})}
\newcommand{\RE}{\mbox{{I}}\hspace{-0.5ex}\mbox{{R}}}
\newcommand{\iC}[1]{\int_{0}^{2\pi} #1 \, d\theta}
\newcommand{\iGr}[1]{\int_{\Gamma_{\infty}} #1 \, ds}

\newcommand{\jump}[1] {\ensuremath{\LRs{\!\!\LRs{#1}\!\!}}}
\newcommand{\diff}[1] {\ensuremath{\LRs{#1}}}
\newcommand{\average}[1] {\ensuremath{\LRc{\!\!\{#1\}\!\!}}}

\newcounter{tablecell}

\newcommand*{\numbercell}{%
  \stepcounter{tablecell}%
  \thetablecell. % **
}

\newtheorem{propo}{Proposition}
\newtheorem{coro}{Corollary}
\newtheorem{theo}{Theorem}
\newtheorem{lem}{Lemma}

%\theoremstyle{definition}
\newtheorem{defi}{definition}

%\theoremstyle{remark}
\newtheorem{rema}{remark}

\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\eqnlab}[1]{\label{eq:#1}}
\newcommand{\theolab}[1]{\label{theo:#1}}
\newcommand{\corolab}[1]{\label{coro:#1}}
\newcommand{\propolab}[1]{\label{propo:#1}}
\newcommand{\lemlab}[1]{\label{lem:#1}}
\newcommand{\defilab}[1]{\label{defi:#1}}
\newcommand{\remalab}[1]{\label{rema:#1}}
\newcommand{\tablab}[1]{\label{tab:#1}}

\newcommand{\figref}[1]{\ref{fig:#1}}
\newcommand{\theoref}[1]{\ref{theo:#1}}
\newcommand{\defiref}[1]{\ref{defi:#1}}
\newcommand{\remaref}[1]{\ref{rema:#1}}
\newcommand{\cororef}[1]{\ref{coro:#1}}
\newcommand{\proporef}[1]{\ref{propo:#1}}
\newcommand{\lemref}[1]{\ref{lem:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\alglab}[1]{\label{alg:#1}}
\newcommand{\algref}[1]{\ref{alg:#1}}
\newcommand{\seclab}[1]{\label{sect:#1}}
\newcommand{\secref}[1]{\ref{sect:#1}}
\newcommand{\tabref}[1]{\ref{tab:#1}}

\renewcommand{\u}{u}
\renewcommand{\v}{v}
\newcommand{\un}{\u_h}
\newcommand{\e}{e}
\newcommand{\w}{w}
\newcommand{\wb}{\mb{\w}}
\newcommand{\J}{J}
\newcommand{\Jb}{\mb{J}}
\newcommand{\q}{q}
\renewcommand{\r}{r}
\newcommand{\qh}{\hat{\q}}
\newcommand{\qs}{\q^*}
\newcommand{\qht}{\tilde{\qh}}
\newcommand{\qbar}{\overline{\q}}
\newcommand{\qb}{{\mb{\q}}}
\newcommand{\sig}{{\sigma}}
\newcommand{\thetah}{{\hat{\theta}}}
\newcommand{\thetas}{{\theta^*}}
\newcommand{\thetahn}{{\thetah_h}}
\newcommand{\sign}[1]{\text{ sgn}\!\LRp{#1}}
\newcommand{\sigh}{\hat{\sig}}
\newcommand{\sigs}{\sig^*}
\newcommand{\sigb}{{\bs{\sig}}}
\newcommand{\sigbn}{\sigb_h}
\newcommand{\sigbs}{\sigb^*}
\newcommand{\taub}{{\bs{\tau}}}
\newcommand{\kappab}{{\bs{\kappa}}}
\newcommand{\gamb}{{\bs{\gamma}}}
\newcommand{\ut}{\tilde{\u}}
\newcommand{\sigbt}{\tilde{\sigb}}
\newcommand{\vt}{\tilde{\v}}
\newcommand{\taubt}{\tilde{\taub}}
\newcommand{\ub}{\mb{\u}}
\newcommand{\ubp}{\mb{\u}^+}
\newcommand{\ubm}{\mb{\u}^-}
\newcommand{\vb}{\mb{\v}}
\newcommand{\um}{\u^-}
\newcommand{\up}{\u^+}


\newcommand{\m}{{m}}

\newcommand{\ud}{{\dot{\u}}}
\newcommand{\vd}{{\dot{\v}}}
\newcommand{\sigbd}{{\dot{\sigb}}}
\newcommand{\taubd}{\dot{\taub}}

\renewcommand{\d}{{d}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\kap}{\kappa}
\newcommand{\F}{\mb{F}}
\newcommand{\f}{f}
\newcommand{\g}{g}
\newcommand{\fb}{\mb{\f}}
\newcommand{\gb}{\mb{\g}}
\newcommand{\gD}{g_D}
\newcommand{\pOmega}{\partial \Omega}
\newcommand{\K}{K}
\newcommand{\Kp}{K^+}
\newcommand{\Km}{K^-}
\newcommand{\pK}{{\partial \K}}
\newcommand{\Kj}{{\K_j}}
\newcommand{\Gh}{{\mc{E}_h}}
\newcommand{\Gho}{{\mc{E}_h^o}}
\newcommand{\Ghb}{{\mc{E}_h^{\partial}}}
\newcommand{\Poly}{{\mc{P}}}
\newcommand{\D}{{D}}
\newcommand{\p}{{p}}
\newcommand{\Ts}{{\mb{T}}}
\newcommand{\Vb}{{\mb{V}}}
\newcommand{\V}{{V}}
\newcommand{\Lam}{{\Lambda}}
\newcommand{\Lamb}{\bs{\Lambda}}
\newcommand{\mub}{\bs{\mu}}
\newcommand{\lambdab}{\bs{\lambda}}
\newcommand{\Th}{{\Ts_h}}
\newcommand{\Vh}{{\V_h}}
\newcommand{\Vbh}{{\Vb_h}}
\newcommand{\Lamh}{{\Lam_h}}
\newcommand{\Lambh}{{\Lamb_h}}
\newcommand{\Lamho}{{\overline{\Lam}_h}}
\newcommand{\Lambht}{{\Lamb_h^t}}
\newcommand{\Ltwo}{{L^2\LRp{\Omega}}}
\newcommand{\Ltwoe}{{L^2\LRp{\e}}}
\newcommand{\Ltw}{{L^2\LRp{\K}}}
\newcommand{\VhK}{{\V_h\LRp{\K}}}
\newcommand{\ThK}{{\Ts_h\LRp{\K}}}
\newcommand{\VbhK}{{\Vb_h\LRp{\K}}}
\newcommand{\Lamhe}{{\Lam_h\LRp{\e}}}
\newcommand{\Lambhe}{{\Lamb_h\LRp{\e}}}
\renewcommand{\L}{\mc{L}}
\renewcommand{\D}{\mc{D}}
\newcommand{\T}{\mc{T}}
\newcommand{\Tt}{\tilde{\T}}
\newcommand{\A}{\mb{A}}
\newcommand{\B}{\mb{B}}
\renewcommand{\D}{\mb{D}}
\newcommand{\Am}{\A^-}
\newcommand{\Ap}{\A^+}
\newcommand{\Aa}{\snor{\A}}
\newcommand{\Rb}{\mb{R}}
\newcommand{\C}{\mb{C}}
\renewcommand{\S}{\mb{S}}
\newcommand{\Sm}{\S^{-}}
\newcommand{\Sp}{\S^{+}}
\newcommand{\Spm}{\S^{\pm}}
\newcommand{\Q}{\mb{Q}}

\newcommand{\Lte}{{L^2\LRp{\Gh}}}
\newcommand{\n}{\mb{n}}
\newcommand{\nm}{\n^-}
\newcommand{\np}{\n^+}
\newcommand{\uh}{{\hat{\u}}}
\newcommand{\us}{{\u^*}}
\newcommand{\uhn}{{\uh_h}}
\newcommand{\ubh}{{\hat{\ub}}}
\newcommand{\ubs}{{\ub^*}}
\newcommand{\ubht}{{\tilde{\ubh}}}
\newcommand{\uht}{{\tilde{\uh}}}
\newcommand{\uhtn}{{\uht_h}}
\newcommand{\uhd}{{\dot{\uh}}}
\newcommand{\sigbh}{{\hat{\sigb}}}
\newcommand{\Fh}{{\hat{\F}}}
\newcommand{\Fs}{\F^*}
\renewcommand{\c}{{c}}

\newcommand{\zb}{\mb{z}}
\renewcommand{\sb}{\mb{s}}
\newcommand{\rb}{\mb{r}}
\newcommand{\betab}{\bs{\beta}}
\newcommand{\veps}{{\varepsilon}}
\newcommand{\vepsb}{\bs{\veps}}
\newcommand{\Hb}{\mb{H}}
\newcommand{\Hbt}{\Hb^t}
\newcommand{\Eb}{\mb{E}}
\newcommand{\Ebt}{\Eb^t}
\newcommand{\hb}{\mb{h}}
\newcommand{\eb}{\mb{e}}
\newcommand{\Hbh}{\hat{\mb{H}}}
\newcommand{\Ebh}{\hat{\mb{E}}}
\newcommand{\Hbs}{{\mb{H}^*}}
\newcommand{\Ebs}{{\mb{E}^*}}
\newcommand{\Ebht}{\Ebh^t}
\newcommand{\Hbht}{\Hbh^t}
\newcommand{\Lb}{\mb{L}}
\newcommand{\Gb}{\mb{G}}
\newcommand{\Lbh}{\hat{\Lb}}
\newcommand{\Lbs}{\Lb^*}
\newcommand{\Ib}{\mb{I}}
\newcommand{\Sigb}{\bs{\Sigma}}
\newcommand{\Piu}{\Pi_\u}
\newcommand{\Pisigb}{\Pi_\sigb}
\newcommand{\Z}{Z}
\newcommand{\Y}{Y}
%\newcommand{\m}{m}
\newcommand{\rhou}{\rho\u}
\newcommand{\rhov}{\rho\v}
\newcommand{\E}{E}
\renewcommand{\P}{P}
\newcommand{\h}{H}
\newcommand{\diag}{\text{diag}}

\newcommand{\phie}{\phi^e}
\newcommand{\vel}{\Ub}
\newcommand{\ephih}{{\veps^h_\phi}}
\newcommand{\ephiI}{{\veps^I_\phi}}
\newcommand{\ephihh}{{\veps^h_{\phih}}}
\newcommand{\ephihI}{{\veps^I_{\phih}}}
\newcommand{\evelh}{{\bs{\veps}^h_{\vel}}}
\newcommand{\evelhh}{{\bs{\veps}^h_{\Ubh}}}
\newcommand{\evelI}{{\bs{\veps}^I_{\vel}}}
\newcommand{\evelhI}{{\bs{\veps}^I_{\Ubh}}}
\newcommand{\Proj}{{\mathbb{P}}}
\newcommand{\Ic}{\Proj}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\tanbui}[2]{\textcolor{blue}{#1} \textcolor{red}{#2}}
%\newcommand{\myblue}[1]{\textcolor{blue}{#1}}

% color
\newcommand{\mygreen}[1]{{\color[rgb]{0,.65,0} #1}}
\newcommand{\mywhite}[1]{{\color[rgb]{1.0,1.0,1.0} #1}}
\newcommand{\myred}[1]{{\color[rgb]{0.65,0.0,0.0} #1}}
\newcommand{\myblue}[1]{{\color[rgb]{0.0,0.0,1.0} #1}}
\newcommand{\mygray}[1]{{\color[rgb]{.15,.35,.60} #1}}
\newcommand{\mythemec}[1]{{\color[RGB]{51,108,121} #1}}
\newcommand{\mydarkred}[1]{{\color[rgb]{.6,.1,.1} #1}}
\newcommand{\mydarkblue}[1]{{\color[rgb]{.1,.1,.9} #1}}
\newcommand{\mygreenback}[1]{{\color[rgb]{.75,1,.75} #1}}
\newcommand{\myorange}[1]{{\color[rgb]{.76,.39,.13} #1}}
\newcommand{\mygrass}[1]{{\color[rgb]{.19,.64,.13} #1}}
\newcommand{\mysierp}[1]{{\color[RGB]{209,28,209} #1}}

